Secrecy Energy Efficiency of MIMOME Wiretap Channels with Full-Duplex Jamming

Full-duplex (FD) jamming transceivers are recently shown to enhance the information security of wireless communication systems by simultaneously transmitting artificial noise (AN) while receiving information. In this work, we investigate if FD jamming can also improve the systems secrecy energy efficiency (SEE) in terms of securely communicated bits-per- Joule, when considering the additional power used for jamming and self-interference (SI) cancellation. Moreover, the degrading effect of the residual SI is also taken into account. In this regard, we formulate a set of SEE maximization problems for a FD multiple-input-multiple-output multiple-antenna eavesdropper (MIMOME) wiretap channel, considering both cases where exact or statistical channel state information (CSI) is available. Due to the intractable problem structure, we propose iterative solutions in each case with a proven convergence to a stationary point. Numerical simulations indicate only a marginal SEE gain, through the utilization of FD jamming, for a wide range of system conditions. However, when SI can efficiently be mitigated, the observed gain is considerable for scenarios with a small distance between the FD node and the eavesdropper, a high Signal-to-noise ratio (SNR), or for a bidirectional FD communication setup.

==> Contributions_Overview.tex <==
 sssssssssssssssss

==> Sections/sec_WMMSE.tex <==

%Due to the intractable mathematical structure of (\ref{eq:model_optimization}), in this part we propose an iterative optimization solution following WMMSE method, see \cite{CACC:08,JPKR:11,7422719}. 
Via the application of $\ma{V}_i^k$ and $\ma{U}_i^k$, as the linear transmit precoder and receive filters, the mean-squared-error (MSE) matrix of the defined system is calculated as
\begin{align} \label{MSE_Matrix}
\ma{E}_i^k :&= \mathbb{E} \left\{ \left( \tilde{\ma{s}}_i^k - {\ma{s}}_i^k \right) \left( \tilde{\ma{s}}_i^k - {\ma{s}}_i^k \right)^H \right\} \nonumber \\  &= \left( {\ma{U}_i^k}^H \ma{H}_{ii}^k \ma{V}_i^k - \ma{I}_{d_i} \right)\left( {\ma{U}_i^k}^H \ma{H}_{ii}^k \ma{V}_i^k - \ma{I}_{d_{i}} \right)^H  \nonumber  \\ & \;\;\;\; + {\ma{U}_i^k}^H  \ma{\Sigma}_i^k {\ma{U}_i^k},  
\end{align}
where $\ma{\Sigma}_i^k$ is given in (\ref{eq_model_aggregate_interference_covariance_CSI_Perfect}). In the following we propose two design strategies for the defined system, proposing an alternating QCP framework. 
 
\subsection{Weighted MSE minimization via Alternating QCP (AltQCP)} \label{sec:MWMSE}
An optimization problem for minimizing the weighted sum MSE is written as 
\begin{subequations}  \label{eq:global_opt_problem_MWMSE}
\begin{align}
\underset{\mathbb{V},\mathbb{U}}{ \text{min}} \;\;   & \sum_{i \in \mathbb{I}}\sum_{k \in \mathbb{F}_K}  \text{tr} \left({\ma{S}_i^k} \ma{E}_i^k\right)  \label{eq:global_opt_problem_MWMSE_a} \\
{\text{s.t.}} \;\; & \text{tr}\bigg( \left( \ma{I}_{N_i} + \ma{\Theta}_{\text{tx},i}\right) \sum_{l\in \mathbb{F}_K} \ma{V}_i^l{\ma{V}_i^l}^H \bigg) \leq P_i, \;\; \forall i \in \mathbb{I},  \label{eq:global_opt_problem_MWMSE_b}
\end{align} 
\end{subequations}
where $\mathbb{X}:= \{\ma{X}_{i}^k, \; \forall i \in \mathbb{I}, \; \forall k \in \mathbb{F}_K\}$, with $\mathbb{X} \in \{\mathbb{U}, \mathbb{V}\}$, and (\ref{eq:global_opt_problem_MWMSE_b}) represents the transmit power constraint. It is worth mentioning that the application of ${\ma{S}_i^k} \succ 0$, as a weight matrix associated with $\ma{E}_i^k$ is two-folded. Firstly, it may appear as a diagonal matrix, emphasizing the importance of different data streams and different users. Secondly, it can be applied as an auxiliary variable which later relates the defined weighted MSE minimization to a sum-rate maximization problem, see Subsection~\ref{sec:perf_CSI_Rate}. \par 
It is observed that (\ref{eq:global_opt_problem_MWMSE}) is not a jointly convex problem. Nevertheless, it holds a QCP structure separately over the sets $\mathbb{V}$ and $\mathbb{U}$, in each case when other variables are fixed. In this regard, the objective (\ref{eq:global_opt_problem_MWMSE_a}) can be decomposed over $\mathbb{U}$ for different communication directions, and for different subcarriers. The optimal minimum MSE (MMSE) receive filter can be hence calculated in closed form as 
\begin{align} \label{wmmse_U_mmse}
\ma{U}_{i,\text{mmse}}^k = \left( \ma{\Sigma}_i^k + \ma{H}_{ii}^k\ma{V}_i^k{\ma{V}_i^k}^H{\ma{H}_{ii}^k}^H \right)^{-1} {\ma{H}_{ii}^k} {\ma{V}_i^k}.
\end{align} 
Nevertheless, the defined problem is coupled over $\ma{V}_{i}^k$, due to the impact of inter-carrier leakage, as well as the power constraint (\ref{eq:global_opt_problem_MWMSE_b}). The Lagrangian function, corresponding to the optimization (\ref{eq:global_opt_problem_MWMSE}) over $\mathbb{V}$ is expressed as 
\begin{align} \label{Lagrangian_WMMSE}     
\mathcal{L} & \left( \mathbb{V}, \boldsymbol{\iota}\right)  :  = \sum_{i \in \mathbb{I}} \bigg( \iota_i { \mathcal{P}_i }\left( \mathbb{V} \right) + \sum_{k \in \mathbb{F}_K}  \text{tr} \left({\ma{S}_i^k} \ma{E}_i^k\right)     \bigg), \\ &  \mathcal{P}_i \left( \mathbb{V} \right):=  - P_i +   \text{tr}\bigg( \left( \ma{I}_{N_i} + \ma{\Theta}_{\text{tx},i}\right) \sum_{l\in \mathbb{F}_K} \ma{V}_i^l{\ma{V}_i^l}^H \bigg),   
\end{align}
where $ \boldsymbol{\iota}:= \{\iota_i,\; i\in\mathbb{I}\}$ is the set of dual variables. The dual function, corresponding to the above Lagrangian is defined as 
\begin{align} 
\mathcal{F}\left( \boldsymbol{\iota} \right)  : & = \underset{\mathbb{V}}{\text{min}} \;\;   \mathcal{L} \left( \mathbb{V}, \boldsymbol{\iota}\right) \label{WMMSE_dualfunction} 
\end{align} 
where the optimal ${\ma{V}_i^k}$ is obtained as
\begin{align} \label{WMMSE_ClosedForm_V}
& {\ma{V}_i^k}^\star = \left( {\ma{J}_i^k} + \iota_i \left( \ma{I}_{N_i} + \ma{\Theta}_{\text{tx},i}\right) + {\ma{H}_{ii}^k}^H {\ma{U}_i^k} {\ma{S}_i^k} {\ma{U}_i^k}^H {\ma{H}_{ii}^k }  \right)^{-1} \nonumber \\ & \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;  \times {\ma{H}_{ii}^k}^H {\ma{U}_i^k}{\ma{S}_i^k},
\end{align} 
and
\begin{align} 
{\ma{J}_i^k} :&= \sum_{l \in \mathbb{F}_K} \sum_{j \in \mathbb{I}} \bigg( {\ma{H}_{ji}^k}^H \text{diag} \left( {\ma{U}_j^l} {\ma{S}_j^l} {\ma{U}_j^l}^H  {\ma{\Theta}_{\text{rx},j}^l}  \right) {\ma{H}_{ji}^k}  \nonumber \\  &  \;\;\;\;  +   \text{diag} \left({\ma{H}_{ji}^l}^H  {\ma{U}_j^l}  {\ma{S}_j^l} {\ma{U}_j^l}^H  {\ma{H}_{ji}^l}  {\ma{\Theta}_{\text{tx},i}^l}  \right)  
\bigg).   
\end{align}
Due to the convexity of the original problem (\ref{eq:global_opt_problem_MWMSE}) over $\mathbb{V}$, the defined dual problem is a concave function over $\boldsymbol{\iota}$, with $\mathcal{P}_i(\mathbb{V})$ as a subgradient, see \cite[Eq.~(6.1)]{bertesekas1999nonlinear}. As a result, the optimal $\boldsymbol{\iota}$ is obtained from the maximization 
\begin{align} 
\boldsymbol{\iota}^\star = \underset{\boldsymbol{\iota} \geq 0}{\text{argmax}} \; \mathcal{F}\left( \boldsymbol{\iota} \right),
\end{align} 
following a standard subgradient update,~\cite[Subsection~6.3.1]{bertesekas1999nonlinear}. \par
 %\cite[Subsections~6.1,~6.3.1]{bertesekas1999nonlinear}.   The optimal  and can be obtained using an iterative subgradiant update, see \cite[Subsections~6.1,~6.3.1]{bertesekas1999nonlinear}. 

 %
%In order to cast the objective into a quadratic norm minimization\footnote{The minimization over $\mathbb{V}$ can be alternatively formulated as a quadratic-constraint quadratic program (QCQP). Nevertheless, the proposed SOCP structure is preferable since it can be later extended for the scenario with CSI error, see Subsection~\ref{WMMSE_CSI_Error} for more details.} we calculate   
%\begin{align}
%& \sum_{k\in \mathbb{F}_K} \text{tr} \left({\ma{W}_i^k}^H \ma{E}_i^k\ma{W}_i^k\right) \nonumber \\ & {=}  \sum_{k\in \mathbb{F}_K} \Bigg{(}
%\left\| {\ma{W}_i^k}^H \left( {\ma{U}_i^k}^H \ma{H}_{ii}^k \ma{V}_i^k - \ma{I}_{d_i} \right) \right\|_{{F}}^2  + \sigma_{i,k}^2 \left\|  {\ma{W}_i^k}^H {\ma{U}_i^k}^H\right\|_{{F}}^2 \nonumber   \\
 %& \;\;\;\; + \sum_{l\in \mathbb{F}_{N_i}}  \sum_{m\in \mathbb{F}_K }   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \ma{H}_{ii}^k \left(\ma{\Theta}_{\text{tx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{N_i}^l  \ma{V}_i^m   \right\|_{{F}}^2  \nonumber   \\
 %& \;\;\;\; + \sum_{l\in \mathbb{F}_{N_j}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \ma{H}_{ij}^k \left(\ma{\Theta}_{\text{tx},j}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^l  \ma{V}_j^m   \right\|_{{F}}^2  \nonumber \\
 %& \;\;\;\; + \sum_{l\in \mathbb{F}_{M_i}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \left(\ma{\Theta}_{\text{rx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l  \ma{H}_{ii}^m\ma{V}_i^m   \right\|_{{F}}^2  \nonumber \\
 %& \;\;\;\; + \sum_{l\in \mathbb{F}_{M_i}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \left(\ma{\Theta}_{\text{rx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l  \ma{H}_{ij}^m\ma{V}_j^m   \right\|_{{F}}^2  \nonumber \\
 %& \;\;\;\;+ \left\|  {\ma{W}_i^k}^H {\ma{U}_i^k}^H   \left(\ma{\Theta}_{\text{rx},i}^k  \sum_{k\in\mathbb{F}_K}  \sigma_{i,k}^2  \right)^{\frac{1}{2}}  \right\|_{{F}}^2 \Bigg{)} \label{error_representation_fro_norm} \\
%& = {\sum_{j \in \mathbb{I} }  \sum_{k \in \mathbb{F}_K } \big\| \ma{c}_{ij}^k \big\|_{2}^2 } ,  \label{quadratic_error_representation_final}
%%
 %%& + \sum_{l\in \mathbb{F}_{N_i}}  \kappa_i  \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{H}_{ii}   \ma{\Gamma}_l \ma{V}_i   \right{\|}_{{F}}^2 \hspace{-0mm} +  \sum_{l\in \mathbb{F}_{M_i}}  \beta_i   \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{\Gamma}_l \ma{H}_{ii}   \ma{V}_i   \right{\|}_{{F}}^2 \nonumber  \\ 
 %%& + \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{\Delta}_{ij} \ma{V}_j   \right{\|}_{{F}}^2 + \sigma_{\text{n},i}^2 \left{\|}  \ma{W}_i^H \ma{U}_i^H\right{\|}_{{F}}^2,  \\
%%& = \boxed{\sum_{j \in \mathcal{D} } \left{\|} \ma{c}_{ij} + \ma{C}_{ij} \text{vec}\left( \ma{\Delta}_{ij} \right) \right{\|}_{2}^2 } ,  \label{quadratic_error_representation_final}
%\end{align}  
%%\end{subequations}
%where (\ref{error_representation_fro_norm}) and (\ref{quadratic_error_representation_final}) are obtained by recalling (\ref{MSE_Matrix}) and (\ref{eq_model_aggregate_interference_covariance_CSI_Perfect}), and following the known matrix equalities \cite[Eq.~(496),~(516)]{MCB:08}. In the above expressions $\ma{\Gamma}_{M}^l$ represents a square matrix with dimension $M$, with all zero elements except of the $l$-th diagonal element equal to $1$, and 
%\begin{align} \label{calculate_c_ii}
%& \ma{c}_{ii}^k :=  \nonumber \\   & \left[ \begin{array}{c} \text{vec} \left( {\ma{W}_i^k}^H \left( {\ma{U}_i^k}^H {\ma{H}}_{ii}^k\ma{V}_i^k  - \ma{I}_{d_i}   \right) \right) \\ \left\lfloor \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H {\ma{H}}_{ii}^k  \left( \ma{\Theta}_{\text{tx},i}^k \right)^{\frac{1}{2}}     \ma{\Gamma}_{N_i}^l \ma{V}_i^m \right) \right\rfloor_{l \in \mathbb{F}_{N_i}, m \in \mathbb{F}_K  } \\  \left\lfloor \text{vec} \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^m \right)^{\frac{1}{2}}     \ma{\Gamma}_{M_i}^l {\ma{H}}_{ii}^k \ma{V}_i^k \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K }    \\  \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H  \left( \sigma_{i,k}^2 \ma{I}_{M_i} + \ma{\Theta}_{\text{rx},i}^k \sum_{m \in \mathbb{F}_K} \sigma_{i,m}^2   \right)^{\frac{1}{2}}  \right)  \\   
%\end{array} \right], 
%\end{align}
%%\begin{align}\label{calculate_C_ii}
%%&\ma{C}_{ii}^k := \nonumber \\ & \left[ \begin{array}{c} {\ma{V}_i^k}^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \\ \left\lfloor  \left(  \left( \ma{\Theta}_{\text{tx},i}^k  \right)^{\frac{1}{2}} \ma{\Gamma}_{N_i}^l \ma{V}_i^m \right)^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \right\rfloor_{l \in \mathbb{F}_{N_i}, m \in \mathbb{F}_K} \\  \left\lfloor  {\ma{V}_i^k}^T \otimes \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^m  \right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m\in \mathbb{F}_K} \\ \ma{0}_{M_i d_i \times M_i N_i}  \end{array} \right],
%%\end{align}
%\begin{align}\label{calculate_c_ij}
%& \ma{c}_{ij}^k \stackrel{i \neq j}{:=}  \nonumber \\   &\left[ \begin{array}{c} \left\lfloor \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H {\ma{H}}_{ij} \left( \ma{\Theta}_{\text{tx},j}^k  \right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^l   \ma{V}_j^m \right) \right\rfloor_{l \in \mathbb{F}_{N_j} , m \in \mathbb{F}_K}   \\ \left\lfloor \text{vec} \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H  \left( \ma{\Theta}_{\text{rx},i}^m  \right)^{\frac{1}{2}} \ma{\Gamma}_{M_{i}}^l {\ma{H}}_{ij}^k  \ma{V}_j^k \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K } \\  \ma{0}_{d_i d_j \times 1 }  \end{array} \right], 
%\end{align}
%%\begin{align}\label{calculate_C_ij}
%%& \ma{C}_{ij}^k \stackrel{i \neq j}{:=}  \nonumber \\ &\left[ \begin{array}{c} \left\lfloor   \left(  \left( \ma{\Theta}_{\text{tx},j}^k  \right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^{l} \ma{V}_j^m \right)^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \right\rfloor_{l \in \mathbb{F}_{N_j} , m\in \mathbb{F}_K}  \\ \left\lfloor {\ma{V}_j^k}^T \otimes \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^k   \right)^{\frac{1}{2}} \ma{\Gamma}_{M_i}^l \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K }  \\    {\ma{V}_j^k}^T \otimes  \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H  \right)  \end{array} \right],
%%\end{align}
%where $\ma{c}_{ij}^k \in \compl^{ \tilde{d}_{ij} \times 1}$ such that  
%\begin{align}\label{length_d}
%& \tilde{d}_{ii} := d_i^2 \left( 1 + K \left( N_i + M_i \right) \right) + d_iM_i,  \\
%& \tilde{d}_{ij} :=  d_id_j \left( 1 + K \left( N_j + M_i \right) \right), \; i,j \in \mathbb{I}, \; i\neq j.
%\end{align}
%Via the introduction of slack variables $\tau_{ij}^k$, the optimization problem (\ref{eq:global_opt_problem_MWMSE}) can be formulated in epigraph form as
 %\begin{subequations}  \label{eq:global_opt_problem_MWMSE_2}
%\begin{align}
%\underset{\mathbb{V},\mathbb{U}, \mathbb{T} }{\text{min}} \;\;  & \sum_{i,j \in \mathbb{I}} \sum_{k \in \mathbb{F}_K}  \tau_{ij}^k  \label{eq:global_opt_problem_MWMSE_2_a} \\
%{\text{s.t.}} \;\;\;     & \big\| \tilde{\ma{v}}_i \big\|_{2}^2  \leq P_i, \; \forall i \in \mathbb{I},  \label{eq:global_opt_problem_MWMSE_2_b}   \\
%&  \big\| \ma{c}_{ij}^k \big\|_{2}^2  \leq  \tau_{ij}^k ,  \; \forall i,j \in \mathbb{I}, \; k \in \mathbb{F}_K,  \label{eq:global_opt_problem_MWMSE_2_c}
%\end{align} 
%\end{subequations}  
%where $\mathbb{T}:= \{\tau_{ij}^k, \; \forall i,j \in \mathbb{I}, \; \forall k \in \mathbb{F}_K\}$, and $\tilde{\ma{v}}_i  := \left\lfloor \text{vec}\left( \ma{V}_{i}^k \right) \right\rfloor_{k\in \mathbb{F}_K}$. It can be observed that (\ref{eq:global_opt_problem_MWMSE_2}) holds an SOCP structure over $\mathbb{V}, \mathbb{T}$ for a fixed $\mathbb{U}$. This facilitates an alternating optimization over the sets $\mathbb{V},\mathbb{T}$ and $\mathbb{U}$, where in each step the corresponding problem is solved to the optimality. 
Utilizing the proposed optimization framework, the alternating optimization over $\mathbb{V}$ and $\mathbb{U}$ is continued until a stable point is obtained. Note that due to the monotonic decrease of the objective in each step, and the fact that (\ref{eq:global_opt_problem_MWMSE_a}) is non-negative and hence bounded from below, the defined procedure leads to a necessary convergence. Algorithm~\ref{alg:MWMSE} defines the necessary optimization steps.
\begin{algorithm}[H] 
 \small{	\begin{algorithmic}[1] 
  %\SetAlgoLined
\State{$\ell \leftarrow  {0}  ;  \;\;\;\; \text{(set iteration number to zero)}$}
\State{$\mathbb{V} \leftarrow \text{right~singular~matrix~initialization,~see~\cite[Appendix~A]{5585631}}$ }
\State{$\mathbb{U} \leftarrow \text{solve~(\ref{wmmse_U_mmse})}$ }
\Repeat 
\State{$\ell \leftarrow  \ell + 1 $}
\State{$\mathbb{V} \leftarrow \text{solve (\ref{WMMSE_ClosedForm_V}) or QCP (\ref{eq:global_opt_problem_MWMSE}), with fixed} \; \mathbb{U}$}

\State{$\mathbb{U} \leftarrow \text{solve (\ref{wmmse_U_mmse}) or QCP (\ref{eq:global_opt_problem_MWMSE}) with fixed} \; \mathbb{V}$}

\Until{$\text{a stable point, or maximum number of $\ell$ reached}$}

\State{\Return$\left\{\mathbb{U},\mathbb{V}\right\}$}
  \end{algorithmic} } 
 \caption{\small{Alternating QCP (AltQCP) for weighted MSE minimization} } \label{alg:MWMSE}
\end{algorithm}   	

\subsection{Weighted MMSE (WMMSE) design for sum rate maximization} \label{sec:perf_CSI_Rate}
Via the utilization of $\ma{V}_{i}^k$ as the transmit precoders, the resulting communication rate for the $k$-th subcarrier and for the $i$-th communication direction is written as 
\begin{align} \label{model:rate_formulation}
I_i^k = B \text{log}_2 \left| \ma{I}_{d_i} + {{\ma{V}}_{i}^k}^H{{\ma{H}}_{ii}^k}^H \big({\ma{\Sigma}}_{i}^k\big)^{-1} {\ma{H}}_{ii}^k{\ma{V}}_{i}^k  \right|, 
\end{align}
where $B$ and ${\ma{\Sigma}}_{i}^k$ are defined in (\ref{eq_model_distortion_stat_res_tx}) and (\ref{eq_model_aggregate_interference_covariance_CSI_Perfect}). The sum rate maximization problem can be hence presented as
%\begin{subequations} 
\begin{align} \label{eq:model_optimization}
\underset{\mathbb{V}}{ \text{max}} \;\; & \;\;\sum_{i \in \mathbb{I}}\sum_{k \in \mathbb{F}_K} I_i^k , \;\; {\text{s.t.}} \;\; \text{(\ref{eq:global_opt_problem_MWMSE_b})}. 
\end{align} 
%\end{subequations} 
The optimization problem (\ref{eq:model_optimization}) is intractable in the current form. In the following we propose an iterative optimization solution, following the WMMSE method \cite{CACC:08}. \\

Via the application of the MMSE receive linear filters from (\ref{wmmse_U_mmse}), the resulting MSE matrix is obtained as 
\begin{align} \label{wmmse_E_mmse}
{\ma{E}_{ i,{\text{mmse}} }^k} = \left(  \ma{I}_{d_i} + {\ma{V}_i^k}^H {\ma{H}_{ii}^k}^H \left({\ma{\Sigma}_i^k}\right)^{-1} \ma{H}_{ii}^k \ma{V}_i^k \right)^{-1}.
\end{align}
By recalling (\ref{model:rate_formulation}), and upon utilization of $\ma{U}_{i,\text{mmse}}^k$, we observe the following useful connection to the rate function 
\begin{align} \label{wmmse_wmmseEquivalent}
I_i^k = - B \text{log}_2 \left| \ma{E}_{i,\text{mmse}}^k \right|,
\end{align}
which facilitates the decomposition of rate function via the following lemma, see also \cite[Eq.~(9)]{CACC:08}.   

\begin{lemma} \label{lemma_logdetE}
Let $\ma{E} \in \compl^{d \times d}$ be a positive definite matrix. The maximization of the term $-\text{log} \left|\ma{E} \right|$ is equivalent to the maximization
\begin{align}
\underset{\ma{E}, \ma{S}}{ \text{max}} - \text{tr}\left( \ma{S} \ma{E} \right) +  \text{log} \left|\ma{S} \right| + d,
\end{align} 
where $\ma{S} \in \compl^{d \times d}$ is a positive definite matrix, and we have 
\begin{align} \label{W_opt_perfectCSI}
\ma{S} = \ma{E}^{-1} ,
\end{align}
at the optimality.
\end{lemma}
\begin{proof}
See \cite[Lemma~2]{JPKR:11}.
\end{proof}
By recalling (\ref{wmmse_wmmseEquivalent}), and utilizing Lemma~\ref{lemma_logdetE}, the original optimization problem over $\mathbb{V}$ can be equivalently formulated as
%\begin{subequations}  
\begin{align} \label{eq:global_opt_problem_rate}
\underset{\mathbb{V},\mathbb{U},\mathbb{S}}{ \text{max}} \;\; & \sum_{k \in \mathbb{F}_K} B \sum_{i \in \mathbb{I}} \bigg(\text{log}\left|\ma{S}_i^k\right|  + d_i  - \text{tr} \left({\ma{S}_i^k} \ma{E}_i^k\right)\bigg) \;\; {\text{s.t.}} \;\; \text{(\ref{eq:global_opt_problem_MWMSE_b})}, 
\end{align} 
%\end{subequations}
where $\mathbb{S}:= \{\ma{S}_{i}^k \succ 0, \; \forall i \in \mathbb{I}, \; \forall k \in \mathbb{F}_K\}$.  
%\begin{align}
%\ma{F}_{ij}^k := \left[\hspace{-0mm}\begin{array}{cc} \tau_{ij}^k &\hspace{-0mm}  {{\ma{c}}_{ij}^k}^H  \\ {\ma{c}}_{ij}^k  & \hspace{-0mm}\ma{I}_{} \end{array} \hspace{-0mm}\right], \;\; \ma{G}_{i} := \left[\hspace{-0mm}\begin{array}{cc} P_i &\hspace{-0mm}  \tilde{\ma{v}}_i^H  \\ \tilde{\ma{v}}_i  & \hspace{-0mm}\ma{I}_{} \end{array} \hspace{-0mm}\right], \label{G_F_definition}
%\end{align}
%where $\ma{G}_i $ and $\ma{F}_{ij}^k$ are obtained by applying the Schur's complement lemma on the quadratic norm constraints (\ref{eq:global_opt_problem_MWMSE_2_b}), (\ref{eq:global_opt_problem_MWMSE_2_c}), respectively. 
The obtained optimization problem (\ref{eq:global_opt_problem_rate}) is not a jointly convex problem. Nevertheless, it is a QCP over $\mathbb{V}$ when other variables are fixed, and can be obtained with a similar structure as for (\ref{eq:global_opt_problem_MWMSE}). Moreover, the optimization over $\mathbb{U}$ and $\mathbb{S}$ is respectively obtained from (\ref{wmmse_U_mmse}), and (\ref{W_opt_perfectCSI}) as $\ma{S}_i^k = {\ma{E}_i^k}^{-1}$. This facilitates an alternating optimization where in each step the corresponding problem is solved to optimality, see Algorithm~\ref{alg:WMMSE_rate}. The defined alternating optimization steps results in a necessary convergence due to the monotonic increase of the objective in each step, and the fact that the eventual system sum rate is bounded from above. 
\begin{algorithm}[H] 
 \small{	\begin{algorithmic}[1] 
  %\SetAlgoLined
\State{$\ell \leftarrow  {0}  ;  \;\;\;\; \text{(set iteration number to zero)}$}
\State{$\mathbb{V} \leftarrow  \text{right~singular~matrix~initialization~\cite[Appendix~A]{5585631}} $} 
\Repeat 
\State{$\ell \leftarrow  \ell + 1$}
\State{$\mathbb{U} \leftarrow \text{solve~(\ref{wmmse_U_mmse})}$}
\State{$\mathbb{V} \leftarrow \text{solve QCP (\ref{eq:global_opt_problem_rate}), with fixed} \; \mathbb{U},\mathbb{S}$}
%\State{$\mathbb{W}, \mathbb{T}, \leftarrow \text{solve SDP (\ref{eq:global_opt_problem_rate}), with fixed} \; \mathbb{V},\mathbb{W}$}
%\State{$\mathbb{U},  \leftarrow \text{solve~(\ref{wmmse_U_mmse})}$}
\State{$\mathbb{S} \leftarrow \ma{S}_i^k = \left( {\ma{E}_i^k} \right)^{-1}$ }
\Until{$\text{a stable point, or maximum number of $\ell$ reached}$}

\State{\Return$\left\{\mathbb{V} \right\}$}
  \end{algorithmic} } 
 \caption{\small{AltQCP-WMMSE design for sum rate maximization} } \label{alg:WMMSE_rate}
\end{algorithm} 

%\begin{subequations}  \label{eq:}
%\begin{align}
%\underset{\mathcal{V}, \mathcal{U}, \mathcal{W}, \mathcal{\tau}, \mathcal{\lambda}, p_{\text{tot}}}{\text{min}} \;\; & p_{\text{tot}} \\
%{\rm s.t.} \;\;     &   \ma{\Theta}_{ij} \succeq 0, \;\; \forall i,j \in \mathcal{I}, \label{Theta_semidefinite_const}\\
%&  \left[\begin{array}{cc} p_{\text{tot}} &   \ma{b}^H\\  \ma{b}  & \ma{I} \end{array} \right] \succeq 0, \label{eq_powerconstraint}
%\end{align} 
%\end{subequations}

%\begin{align}
%\left[\hspace{-0mm}\begin{array}{cc} 0 &\hspace{-0mm}  {{\ma{b}}_{ij}^k}^H {\tilde{\ma{D}}_{ij}^k}^{H} {\ma{C}_{ij}^k}^H  \\   {\ma{C}_{ij}^k}{\tilde{\ma{D}}_{ij}}^k {\ma{b}}_{ij}^k  & \hspace{-0mm}\ma{0}_{\tilde{d}_{ij} \times \tilde{d}_{ij}} \end{array} \hspace{-0mm}\right] \hspace{-0mm}+\hspace{-0mm} \left[\begin{array}{cc} \tau_{ij}^k & {\ma{c}_{ij}^k}^H \\   \ma{c}_{ij}^k &  \ma{I}_{\tilde{d}_{ij}} \end{array} \right] \succeq 0. 
%\end{align}

%The MMSE receive filter can be then calculated as 

%\begin{align} \label{wmmse_U_mmse}
%\ma{U}_{i,\text{mmse}}^k = \left( \ma{\Sigma}_i^k + \ma{H}_{ii}^k\ma{V}_i^k{\ma{V}_i^k}^H{\ma{H}_{ii}^k}^H \right)^{-1} {\ma{H}_{ii}^k} {\ma{V}_i^k} ,
%\end{align}    
%and the resulting MSE matrix is obtained as 
%\begin{align} \label{wmmse_E_mmse}
%{\ma{E}_{ i,{\text{mmse}} }^k} = \left(  \ma{I}_{d_i} + {\ma{V}_i^k}^H {\ma{H}_{ii}^k}^H \left({\ma{\Sigma}_i^k}\right)^{-1} \ma{H}_{ii}^k \ma{V}_i^k \right)^{-1}.
%\end{align}
%By recalling (\ref{model:rate_formulation}), and upon utilization of $\ma{U}_{i,\text{mmse}}^k$, we observe the following useful connection to the rate function 
%\begin{align} \label{wmmse_wmmseEquivalent}
%I_i^k = - B_i^k \text{log}_2 \left| \ma{E}_{i,\text{mmse}}^k \right|,
%\end{align}
%which facilitates the decomposition of rate function via the following lemma, see also \cite[Eq.~(9)]{CACC:08}.   
%
%\begin{lemma} \label{lemma_logdetE}
%Let $\ma{E} \in \compl^{d \times d}$ be a positive definite matrix. The maximization of the term $-\text{log} \left|\ma{E} \right|$ is equivalent to the maximization
%\begin{align}
%\underset{\ma{E}, \ma{W}}{ \text{max}} - \text{tr}\left( \ma{W}^H \ma{E} \ma{W} \right) +  \text{log} \left|\ma{W}\ma{W}^H \right| + d,
%\end{align} 
%where $\ma{W} \in \compl^{d \times d}$ is a positive definite matrix.
%\end{lemma}
%\begin{proof}
%The proof is obtained following \cite[Lemma~2]{JPKR:11}, and decomposing $\ma{S}\in \compl^{d \times d}$ as $\ma{S}=\ma{W}\ma{W}^H$.
%\end{proof}
%By recalling (\ref{wmmse_wmmseEquivalent}), and utilizing Lemma~\ref{lemma_logdetE}, the original optimization problem can be equivalently formulated as
%\begin{subequations}  \label{eq:global_opt_problem_2}
%\begin{align}
%\underset{\mathbb{V}}{ \text{max}} \;\; \underset{\mathbbl{\Delta}}{ \text{min}}  \;\; \underset{\mathbb{U}, \mathbb{W}}{ \text{max}}  &\;\; \sum_{i \in \mathbb{I}} \gamma_i \sum_{k \in \mathbb{F}_K}  \bigg( \text{log} \left|\ma{W}_i^k{\ma{W}_i^k}^H\right|  \nonumber \\ & + d_i - \text{tr} \left({\ma{W}_i^k}^H \ma{E}_i^k\ma{W}_i^k\right) \bigg) \\
%{\rm s.t.} \;\;     & \text{(\ref{eq:global_opt_problem_1_power_contraint}),~(\ref{eq:global_opt_problem_1_normbounded_contraint})} \label{eq:global_opt_problem_2_constraints}
%\end{align} 
%\end{subequations}
%where $\mathbb{U}$ is defined similar to that of $\mathbb{V}$, and $\mathbb{W}$ is a set containing $\ma{W}_{i}^k \succ 0,\; i,\in \mathbb{I}, \; k,\in \mathbb{F}_K$. In order to cast the objective into a simpler form we calculate  
%\begin{align}
%& \sum_{k\in \mathbb{F}_K} \text{tr} \left({\ma{W}_i^k}^H \ma{E}_i^k\ma{W}_i^k\right) \nonumber \\ & =  \sum_{k\in \mathbb{F}_K} \Bigg{(}
%\left\| {\ma{W}_i^k}^H \left( {\ma{U}_i^k}^H \ma{H}_{ii}^k \ma{V}_i^k - \ma{I}_{d_i} \right) \right\|_{{F}}^2 \nonumber \\
 %& \;\;\;\; + \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \ma{\Delta}_{ij}^k \ma{V}_j^k   \right\|_{{F}}^2 + \sigma_{i,k}^2 \left\|  {\ma{W}_i^k}^H {\ma{U}_i^k}^H\right\|_{{F}}^2, \nonumber   \\
 %& \;\;\;\; + \sum_{l\in \mathbb{F}_{N_i}}  \sum_{m\in \mathbb{F}_K }   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \ma{H}_{ii}^k \left(\ma{\Theta}_{\text{tx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{N_i}^l  \ma{V}_i^m   \right\|_{{F}}^2  \nonumber   \\
 %& \;\;\;\; + \sum_{l\in \mathbb{F}_{N_j}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \ma{H}_{ij}^k \left(\ma{\Theta}_{\text{tx},j}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^l  \ma{V}_j^m   \right\|_{{F}}^2  \nonumber \\
 %& \;\;\;\; + \sum_{l\in \mathbb{F}_{M_i}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \left(\ma{\Theta}_{\text{rx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l  \ma{H}_{ii}^m\ma{V}_i^m   \right\|_{{F}}^2  \nonumber \\
 %& \;\;\;\; + \sum_{l\in \mathbb{F}_{M_i}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \left(\ma{\Theta}_{\text{rx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l  \ma{H}_{ij}^m\ma{V}_j^m   \right\|_{{F}}^2  \nonumber \\
 %& \;\;\;\;+ \left\|  {\ma{W}_i^k}^H {\ma{U}_i^k}^H   \left(\ma{\Theta}_{\text{rx},i}^k  \sum_{k\in\mathbb{F}_K}  \sigma_{i,k}^2  \right)^{\frac{1}{2}}  \right\|_{{F}}^2 \Bigg{)} \label{error_representation_fro_norm} \\
%& = \boxed{\sum_{j \in \mathbb{I} }  \sum_{k \in \mathbb{F}_K } \left\| \ma{c}_{ij}^k + \ma{C}_{ij}^k \text{vec}\left( \ma{\Delta}_{ij}^k \right) \right\|_{2}^2 } .  \label{quadratic_error_representation_final}
%%
%%
 %%& + \sum_{l\in \mathbb{F}_{N_i}}  \kappa_i  \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{H}_{ii}   \ma{\Gamma}_l \ma{V}_i   \right{\|}_{{F}}^2 \hspace{-0mm} +  \sum_{l\in \mathbb{F}_{M_i}}  \beta_i   \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{\Gamma}_l \ma{H}_{ii}   \ma{V}_i   \right{\|}_{{F}}^2 \nonumber  \\ 
 %%& + \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{\Delta}_{ij} \ma{V}_j   \right{\|}_{{F}}^2 + \sigma_{\text{n},i}^2 \left{\|}  \ma{W}_i^H \ma{U}_i^H\right{\|}_{{F}}^2,  \\
%%& = \boxed{\sum_{j \in \mathcal{D} } \left{\|} \ma{c}_{ij} + \ma{C}_{ij} \text{vec}\left( \ma{\Delta}_{ij} \right) \right{\|}_{2}^2 } ,  \label{quadratic_error_representation_final}
%\end{align}  
%%\end{subequations}
%In the above expressions $\ma{\Gamma}_{K}^l$ represents a square matrix with dimension $K$, with all zero elements except of the $l$-th diagonal element equal to $1$, and 
%\begin{align} \label{calculate_c_ii}
%& \ma{c}_{ii}^k :=  \nonumber \\   & \left[ \begin{array}{c} \text{vec} \left( {\ma{W}_i^k}^H \left( {\ma{U}_i^k}^H \tilde{\ma{H}}_{ii}^k\ma{V}_i^k  - \ma{I}_{d_i}   \right) \right) \\ \left\lfloor \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \tilde{\ma{H}}_{ii}^k  \left( \ma{\Theta}_{\text{tx},i}^k \right)^{\frac{1}{2}}     \ma{\Gamma}_{N_i}^l \ma{V}_i^m \right) \right\rfloor_{l \in \mathbb{F}_{N_i}, m \in \mathbb{F}_K  } \\  \left\lfloor \text{vec} \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^m \right)^{\frac{1}{2}}     \ma{\Gamma}_{M_i}^l \tilde{\ma{H}}_{ii}^k \ma{V}_i^k \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K }    \\  \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H  \left( \sigma_{i,k}^2 \ma{I}_{M_i} + \ma{\Theta}_{\text{rx},i}^k \sum_{m \in \mathbb{F}_K} \sigma_{i,m}^2   \right)^{\frac{1}{2}}  \right)  \\   
%\end{array} \right], 
%\end{align}
%\begin{align}\label{calculate_C_ii}
%&\ma{C}_{ii}^k := \nonumber \\ & \left[ \begin{array}{c} {\ma{V}_i^k}^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \\ \left\lfloor  \left(  \left( \ma{\Theta}_{\text{tx},i}^k  \right)^{\frac{1}{2}} \ma{\Gamma}_{N_i}^l \ma{V}_i^m \right)^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \right\rfloor_{l \in \mathbb{F}_{N_i}, m \in \mathbb{F}_K} \\  \left\lfloor  {\ma{V}_i^k}^T \otimes \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^m  \right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m\in \mathbb{F}_K} \\ \ma{0}_{M_i d_i \times M_i N_i}  \end{array} \right],
%\end{align}
%\begin{align}\label{calculate_c_ij}
%& \ma{c}_{ij}^k \stackrel{i \neq j}{:=}  \nonumber \\   &\left[ \begin{array}{c} \left\lfloor \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \tilde{\ma{H}}_{ij} \left( \ma{\Theta}_{\text{tx},j}^k  \right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^l   \ma{V}_j^m \right) \right\rfloor_{l \in \mathbb{F}_{N_j} , m \in \mathbb{F}_K}   \\ \left\lfloor \text{vec} \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H  \left( \ma{\Theta}_{\text{rx},i}^m  \right)^{\frac{1}{2}} \ma{\Gamma}_{M_{i}}^l \tilde{\ma{H}}_{ij}^k  \ma{V}_j^k \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K } \\  \ma{0}_{d_i d_j \times 1 }  \end{array} \right], 
%\end{align}
%\begin{align}\label{calculate_C_ij}
%& \ma{C}_{ij}^k \stackrel{i \neq j}{:=}  \nonumber \\ &\left[ \begin{array}{c} \left\lfloor   \left(  \left( \ma{\Theta}_{\text{tx},j}^k  \right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^{l} \ma{V}_j^m \right)^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \right\rfloor_{l \in \mathbb{F}_{N_j} , m\in \mathbb{F}_K}  \\ \left\lfloor {\ma{V}_j^k}^T \otimes \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^k   \right)^{\frac{1}{2}} \ma{\Gamma}_{M_i}^l \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K }  \\    {\ma{V}_j^k}^T \otimes  \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H  \right)  \end{array} \right],
%\end{align}
%where $\ma{c}_{ij}^k \in \compl^{ \tilde{d}_{ij} \times 1}$, $\ma{C}_{ij}^k \in \compl^{ \tilde{d}_{ij} \times {M_i N_j}}$ such that  
%\begin{align}\label{length_d}
%& \tilde{d}_{ii} := d_i^2 \left( 1 + K \left( N_i + M_i \right) \right) + d_iM_i,  \\
%& \tilde{d}_{ij} :=  d_id_j \left( 1 + K \left( N_j + M_i \right) \right), \; i,j \in \mathbb{I}, \; i\neq j.
%\end{align}
%Please note that (\ref{error_representation_fro_norm}) is obtained by recalling (\ref{MSE_Matrix}) and (\ref{eq_model_aggregate_interference_covariance}) and the known matrix equality \cite[Eq.~(516)]{MCB:08}, and (\ref{calculate_c_ii})-(\ref{calculate_C_ij}) are calculated via the application of \cite[Eq.~(496),~(497)]{MCB:08}. \par
%Unfortunately, the problem (\ref{eq:global_opt_problem_2}) is still intractable, due to the the joint inner and outer maximization. Hence, we focus on maximizing the lower bound of the objective following the max-min inequality, see \cite[Eq.~(12)]{JPKR:11}. This is written using the epigraph form as 
%\begin{subequations}  \label{eq:global_opt_problem_3}
%%\begin{subequations}  \label{eq:global_opt_problem}
%\begin{align}
%\underset{\mathbb{V}, \mathbb{U}, \mathbb{W}, \mathcal{T}}{ \text{max}} \;\; \underset{\mathbbl{\Delta}}{ \text{min}} & \; \sum_{i \in \mathbb{I}} \gamma_i \sum_{k \in \mathbb{F}_K}  \bigg( \text{log} \left|\ma{W}_i^k{\ma{W}_i^k}^H\right|  + d_i - \sum_{j \in \mathbb{I}} \tau_{ij}^k \bigg)  \\
%{\rm s.t.} \;     &  \| \ma{c}_{ij}^k + \ma{C}_{ij}^k\text{vec}\left( \ma{\Delta}_{ij}^k \right)  \|_2^2 \leq \tau_{ij}^k, \; \forall i,j \in \mathbb{I}, k \in \mathbb{F}_K, \label{eq:global_opt_problem_3_normbounded_contraint}\\ & \text{(\ref{eq:global_opt_problem_1_normbounded_contraint}),~(\ref{eq:global_opt_problem_1_power_contraint})}, \;\; \label{Opt_problem_3_normconstraint}
%\end{align} 
%\end{subequations}
%where $\mathcal{T} :=\{\tau_{ij}^k, \; \forall i,j \in \mathbb{I}, k \in \mathbb{F}_K\}$. In order to simplicity the formulations we define 
%\begin{align}
%\tilde{\ma{\Delta}}_{ij}^k & := \ma{D}_{ij}^k {\ma{\Delta}}_{ij}^k, \\
%\tilde{\ma{D}}_{ij}^k & := \ma{I}_{N_j} \otimes \left({\ma{D}_{ij}^k}\right)^{-1}, \\
%\ma{b}_{ij}^k & := \text{vec}\left(\tilde{\ma{\Delta}}_{ij}^k \right). 
%\end{align}
%By applying the Schur complement lemma, the constraint (\ref{eq:global_opt_problem_3_normbounded_contraint}) is equivalently written as 
%\begin{align}
%\left[\hspace{-0mm}\begin{array}{cc} 0 &\hspace{-0mm}  {{\ma{b}}_{ij}^k}^H {\tilde{\ma{D}}_{ij}^k}^{H} {\ma{C}_{ij}^k}^H  \\   {\ma{C}_{ij}^k}{\tilde{\ma{D}}_{ij}}^k {\ma{b}}_{ij}^k  & \hspace{-0mm}\ma{0}_{\tilde{d}_{ij} \times \tilde{d}_{ij}} \end{array} \hspace{-0mm}\right] \hspace{-0mm}+\hspace{-0mm} \left[\begin{array}{cc} \tau_{ij}^k & {\ma{c}_{ij}^k}^H \\   \ma{c}_{ij}^k &  \ma{I}_{\tilde{d}_{ij}} \end{array} \right] \succeq 0. 
%\end{align} 
%Moreover, the constraint (\ref{eq:global_opt_problem_1_normbounded_contraint}) can be equivalently written as $ \| {\ma{b}}_{ij}^k\|_2 \leq \zeta_{ij}^k$.  
%
%\begin{lemma} \label{petersen}
%Generalized Petersen's sign-definiteness lemma: Let $\ma{Y} = \ma{Y}^H$, and $\ma{X},\ma{P},\ma{Q}$ are arbitrary matrices with complex valued elements. Then we have
%\begin{align}
%\ma{Y} \succeq \ma{P}^H \ma{X} \ma{Q} + \ma{Q}^H \ma{X}^H \ma{P}, \;\; \forall \ma{X} \; : \; \| \ma{X}\|_F \leq \zeta, 
%\end{align} 
%if and only if 
%\begin{align}
%\exists \lambda \geq 0, \; \left[\begin{array}{cc} \ma{Y} - \lambda \ma{Q}^H\ma{Q} & - \zeta \ma{P}^H \\   - \zeta \ma{P} & \lambda \ma{I} \end{array} \right] \succeq 0.
%\end{align} 
%\end{lemma}
%\begin{proof}
%See~\cite[Proposition~2]{EM:04}, \cite{khlebnikov2008petersen}.
%\end{proof}
%By choosing the matrices in Lemma~\ref{petersen} such that $\ma{X} = {\ma{b}}_{ij}^k$, $\ma{Q} = \left[ -1, \; \ma{0}_{1 \times \tilde{d}_{ij} }  \right]$ and  
%\begin{align}
%\ma{Y} =  \left[\begin{array}{cc} \tau_{ij}^k & {\ma{c}_{ij}^k}^H \\   \ma{c}_{ij}^k & \ma{I}_{\tilde{d}_{ij}} \end{array} \right], \ma{P} = \left[\begin{array}{cc} \ma{0}_{{M_i N_j} \times 1 }, \;\; {\tilde{\ma{D}}_{ij}^k}^H {{\ma{C}}_{ij}^k}^H \end{array} \right],
%\end{align} 
%the optimization problem in (\ref{eq:global_opt_problem_3}) is equivalently written as  
%\begin{subequations}  \label{eq:global_opt_problem_4}
%\begin{align}
%\underset{\mathbb{V},\mathbb{U}, \mathbb{W}, \mathcal{T}, \mathcal{C}}{ \text{max}}  \;\;\; & \sum_{i \in \mathbb{I}} \gamma_i \sum_{k \in \mathbb{F}_K}  \bigg( 2\text{log}\left|\ma{W}_i^k\right|  + d_i - \sum_{j \in \mathbb{I}} \tau_{ij}^k \bigg) \\
%{\rm s.t.} \;\;     & \ma{\Lambda}_{i,j}^k \succeq 0,  \;\; \forall i,j \in \mathbb{I}, k \in \mathbb{F}_K, \label{eq:p4_lambda_tau} \\
%&  \ma{\Omega}_i \succeq 0 , \;\;  \forall i \in \mathbb{I}, \label{eq:p4_power}
%\end{align} 
%\end{subequations}
%where 
%\begin{align}
%\ma{\Lambda}_{i,j}^k := \left[\begin{array}{ccc} \tau_{ij}^k - \lambda_{ij}^k & {\ma{c}_{ij}^k}^H &  \ma{0}_{1 \times M_i N_j }\\  \ma{c}_{ij}^k & \ma{I}_{\tilde{d}_{ij}}  &  - \zeta_{ij}^k {\ma{C}}_{ij}^k\tilde{\ma{D}}_{ij}^k \\  \ma{0}_{{M_i N_j \times 1 }} & - \zeta_{ij}^k {\tilde{\ma{D}}_{ij}^k}^H {{\ma{C}}_{ij}^k}^H  &   \lambda_{ij}^k \ma{I}_{M_i N_j} \end{array} \right]
%\end{align} 
%and
%\begin{align}
%\ma{\Omega}_{i} := \left[\begin{array}{cc}  P_i & \ma{d}_i^H\\ \ma{d}_i & \ma{I}_{KN_id_i}    \end{array} \right], \;\; \ma{d}_i :=  \left\lfloor \text{vec}\left( \ma{V}_i^k \right) \right\rfloor_{k\in\mathbb{F}_K}.
%\end{align} 
%In the formulation of the optimization problem (\ref{eq:global_opt_problem_4}) the semi-definite constraints (\ref{eq:p4_lambda_tau}) and (\ref{eq:p4_power}) are respectively equivalent to (\ref{eq:global_opt_problem_3_normbounded_contraint}) and (\ref{eq:global_opt_problem_1_power_contraint}), and $\mathcal{C}$ is the set containing the auxiliary variables $\lambda_{ij}^k$, i.e., $\mathcal{C} :=\{\lambda_{ij}^k, \; \forall i,j \in \mathbb{I}, k \in \mathbb{F}_K \}$. \par 
%%Note that (\ref{eq:global_opt_problem_4}) is not a jointly convex optimization problem. Nevertheless, it is separately convex over the optimization variables, see (\ref{calculate_c_ii})-(\ref{calculate_C_ij}). This facilitates an iterative optimization over separated variable sets, where in each iteration a convex sub-problem is solved, see Algorithm~\ref{alg_1}. In this regard, the maximization over $\ma{V},\ma{U}$ can be separately cast as a general SDP, where the optimization over $\ma{W}$ can be efficiently implemented using MAX-DET algorithm \cite{vandenberghe1998determinant}. Moreover, due to the monotonic increase of the objective in each optimization iteration, and since the objective is bounded from above, the algorithm necessarily convergences to a stationary point.
%Note that (\ref{eq:global_opt_problem_4}) is not a jointly convex optimization problem. Nevertheless, it is separately convex over the optimization variables, see (\ref{calculate_c_ii})-(\ref{calculate_C_ij}). This facilitates an iterative optimization over separated variable sets, where in each iteration a convex sub-problem is solved, see Algorithm~\ref{alg_1}. In this regard, the maximization over ${\mathbb{V}},{\mathbb{U}}$ can be separately cast as a general semi-definite program (SDP), where the optimization over ${\mathbb{W}}$ can be efficiently implemented using MAX-DET algorithm \cite{vandenberghe1998determinant}. Moreover, due to the monotonic increase of the objective in each optimization iteration the algorithm convergences to a stationary point. See \cite[Section~III]{JPKR:11} for detailed arguments regarding convergence and optimization steps for a problem with similar variable separation.  
%
%
%\subsection{Worst-Case Channel Error Matrices}
%The obtained design from (\ref{eq:global_opt_problem_4}) is intended to maximize the worst-case weighted system sum rate, over the feasible error region. On the other hand it is beneficial to obtain the least favorable channel error matrices, as it provides guidelines for the future channel estimation strategies. For instance, this helps us to choose a channel training sequence that reduces the radius of the CSI error feasible regions in the most destructive directions. Moreover, such knowledge is a necessary step for cutting-set-based methods \cite{mutapcic2009cutting} that aim to reduce the design complexity by iteratively identifying the most destructive error matrices and incorporating them into the future design steps. In the current setup, the worst-case channel error matrices are identified by minimizing the rate function (\ref{eq:model_optimization}) within their feasible region. Due to the intractable structure of such a rate minimization problem, we focus on the modified objective in (\ref{eq:global_opt_problem_3}) where the worst case error matrices can be obtained via the inner minimization as 
%\begin{subequations}  \label{wmmse_}
%\begin{align}
%\underset{\mathbbl{{\Delta}}}{ \text{min}} \;\;  &- \sum_{i \in \mathbb{I}} \gamma_i  \sum_{k\in\mathbb{F}_K}\text{tr}\left({\ma{W}_{i}^k}^H \ma{E}_i^k \ma{W}_{i}^k\right), \;\; \\
%{\rm s.t.} \;\;     &  \| \ma{D}_{ij}^k  \ma{\Delta}_{ij}^k \| \leq \zeta_{ij}^k, \;\; \forall i,j \in \mathbb{I},\; k \in \mathbb{F}_K,
%\end{align} 
%\end{subequations}
%Note that the above formulation also defines the worst-case CSI error matrices in the MMSE sense, by setting $\ma{W}_i^k = \ma{I}_{d_i}$, and considering $\gamma_i$ as the price of the estimation MSE in the direction $i$, see Subsection~\ref{subsec_MMSE}. Due to the uncoupled nature of the error feasible set, and the value of the objective function over $\ma{\Delta}_{ij}^k, \; i,j \in \mathbb{I}$, following (\ref{quadratic_error_representation_final}), the above minimization can be decomposed as 
%%\begin{align}
%%\underset{ {\ma{b}}_{ij} }{ \text{max}} \;\;  \left{\|} \ma{c}_{ij} + \ma{C}_{ij} \tilde{\ma{D}}_{ij} {\ma{b}}_{ij} \right{\|}_{2}^2, \;\;\;\; {\rm s.t.} \;\;       \| {\ma{b}}_{ij} \|_2^2 \leq \zeta_{ij}^2, 
%%\end{align} 
%\begin{subequations} \label{find_worst_delta_3}
%\begin{align} 
%\underset{ {\ma{b}}_{ij}^k }{ \text{min}} \;\;  & - \left\| \ma{C}_{ij}^k \tilde{\ma{D}}_{ij}^k {\ma{b}}_{ij}^k \right\|_2^2 - 2 \text{Re}\left\{ {{\ma{b}}_{ij}^k}^H   {{\tilde{\ma{D}}_{ij}^k}}^H {\ma{C}_{ij}^k}^H  \ma{c}_{ij}^k \right\} -  {\ma{c}_{ij}^k}^H\ma{c}_{ij}^k \label{wwmse_worstcaseerror_nonconvexquadraticobjective}\\ {\rm s.t.} \;\;      & {{\ma{b}}_{ij}^k}^H {\ma{b}}_{ij}^k  \leq {\zeta_{ij}^k}^2, 
%\end{align} 
%\end{subequations}
%where $\text{Re}\{\cdot\}$ represents the real part of a complex value. Note that the objective in (\ref{wwmse_worstcaseerror_nonconvexquadraticobjective}) is a non convex function and can not be minimized using the usual numerical solvers in the current form. Following the zero duality gap results for the non-convex quadratic problems \cite{zheng2012zero, BV:04}, we focus on the dual function of (\ref{find_worst_delta_3}). The corresponding Lagrangian function to (\ref{find_worst_delta_3}) is hence constructed as 
%\begin{align}  \label{find_worst_delta_Lagrangian}
%& \mathcal{L}\left({\ma{b}}_{ij}^k , \rho_{ij}^k \right)  =  \nonumber  \\  &  {{\ma{b}}_{ij}^k}^H  \ma{A}_{ij}^k {\ma{b}}_{ij}^k  - 2 \text{Re}\left\{ {{\ma{b}}_{ij}^k}^H   {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  \ma{c}_{ij}^k \right\} -  {\ma{c}_{ij}^k}^H \ma{c}_{ij}^k - \rho_{ij}^k  {\zeta_{ij}^k}^2, 
%\end{align} 
%where $\rho_{ij}^k$ is the dual variable and 
%\begin{align} 
%\ma{A}_{ij}^k := \rho_{ij}^k \ma{I}_{N_jM_i} - {\tilde{\ma{D}}_{ij}^k}^H{{\ma{C}}_{ij}^k}^H{\ma{C}}_{ij}^k\tilde{\ma{D}}_{ij}^k.
%\end{align} 
%Consequently, the value of the dual function is obtained as 
%\begin{align}
%& \ma{g} \left( \rho_{ij}^k \right) = \nonumber \\ & - {{\ma{c}}_{ij}^k}^H  \ma{C}_{ij}^k  \tilde{\ma{D}}_{ij}^k \left(\ma{A}_{ij}^k\right)^{-1} {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {\ma{c}}_{ij}^k  - {\ma{c}_{ij}^k}^H\ma{c}_{ij}^k - \rho_{ij}^k {\zeta_{ij}^k}^2, 
%%\left\{\begin{array}{cc} \tau_{ij} & \ma{c}_{ij}^H \\   \ma{c}_{ij} & \ma{I}_{\tilde{d}_{ij}} \end{array} \right\
%\end{align}
%if $ \ma{A}_{ij}^k \succeq 0$, and ${\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {\ma{c}}_{ij}^k \in \mathcal{R}\{\ma{A}_{ij}^k\}$, and otherwise is unbounded from below\footnote{If one of the aforementioned conditions is not satisfied, an infinitely large value of $\ma{b}_{ij}$ can be chosen in the negative direction of $\ma{A}_{ij}$, if $\ma{A}_{ij}^k$ is not positive semi-definite, or in the direction ${\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  \ma{c}_{ij}^k$ within the null-space of $\ma{A}_{ij}^k$.}. By applying the Schur complement lemma, the maximization of the dual function is written using the epigraph form as
%\begin{subequations} \label{eq:dual_channelerrormatrices}
%\begin{align}
%\underset{ {\rho}_{ij}^k \geq 0 , \; \phi_{ij}^k} { \text{max} } \;\;  & - \phi_{ij}^k \\  
%{\rm s.t.} \;\; & \left[\begin{array}{cc} \phi_{ij}^k - {\ma{c}_{ij}^k}^H\ma{c}_{ij}^k  - {\rho}_{ij}^k {\zeta_{ij}^k}^2   & {{\ma{c}}_{ij}^k}^H  \ma{C}_{ij}^k  \tilde{\ma{D}}_{ij}^k  \\ {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {\ma{c}}_{ij}^k   & \ma{A}_{ij}^k  \end{array} \right] \succeq 0,  \label{eq:dual_channelerrormatrices_schur_semidefiniteconstraint}
%\end{align} 
%\end{subequations}
%where $\phi_{ij}^k \in \real $ is an auxiliary variable\footnote{Note that the semi-definite presentation in (\ref{eq:dual_channelerrormatrices_schur_semidefiniteconstraint}) automatically satisfies  $ \ma{A}_{ij}^k \succeq 0$, and ${\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {\ma{c}}_{ij}^k \in \mathcal{R}\{\ma{A}_{ij}^k\}$.}. By plugging the obtained dual variable ${\rho}_{ij}^k$ into (\ref{find_worst_delta_Lagrangian}), and considering the fact that $- {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H \ma{C}_{ij}^k \tilde{\ma{D}}_{ij}^k + {\rho_{ij}^k}^\star \ma{I}_{N_jM_i} \succeq 0$ as a result of (\ref{eq:dual_channelerrormatrices}), the optimal value of $\ma{b}_{ij}^k$ is obtained from (\ref{find_worst_delta_Lagrangian}) as 
%\begin{align}
%{\ma{b}_{ij}^k}^\star = \left( - {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H \ma{C}_{ij}^k \tilde{\ma{D}}_{ij}^k + {\rho_{ij}^k}^\star \ma{I}_{N_jM_i} \right)^{-1} {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {\ma{c}}_{ij}^k,
%\end{align} 
%where $(\cdot)^\star$ represents the optimality and the worst case $\ma{\Delta}_{ij}^k$ is consequently calculated via $\text{vec}(\ma{\Delta}_{ij}^k) = \tilde{\ma{D}}_{ij}^k {\ma{b}_{ij}^k}^\star$.
%
%
%%\subsection{Worst-Case MMSE Optimization}
%%%The design of an MMSE-based FD transceiver is addressed in \cite{}, assu under channel knowledge ubncertainty is been addressed in \cite{}, where the statistics of the CSI errors are known.
%%By setting a The design procedure can be directly obtained from the  
%\subsection{Computational Complexity}
%As mentioned, the optimization over $\mathbb{V}, \mathbb{U}$ are cast as variations of SDP, where the optimization over $\mathbb{W}$, is performed using MAX-DET algorithm. A general SDP problem is defined as 
%\begin{align}
%\underset{\ma{z}}{\text{min}} \;\; \ma{p}^T \ma{z}, \;\; {\rm{s.t.}} \;\;  \ma{z}\in \real^n, \; \ma{Y}_0 + \sum_{i=1}^n z_i \ma{Y}_i \succeq 0, \; \|\ma{z}\|_2 \leq q,  
%\end{align}
%where the fixed matrices $\ma{Y}_i$ are symmetric block-diagonal, with $M$ diagonal blocks of the sizes $l_m \times l_m,\; m \in \{1,\ldots,M\}$, and define the specific problem structure, see \cite[Subsection~4.6.3]{ben2001lectures}, and \cite{7422719} for a similar discussion. The arithmetic complexity of obtaining an $\epsilon$-solution to the defined problem, i.e., the convergence to the $\epsilon$-distance vicinity of the optimum is upper-bounded by 
%\begin{align}
%\mathcal{O}(1) \left(1 + \sum_{m=1}^{M} l_m  \right)^{\frac{1}{2}} \left( n^3 + n^2 \sum_{m=1}^{M} l_m^2 + n \sum_{m=1}^M l_m^3\right) \text{digit}\left( \epsilon\right), 
%\end{align}
%where $\text{digit}(\epsilon)$, is obtained from \cite[Subsection~4.1.2]{ben2001lectures}, and affected by the required solution precision. The required computation of each step is hence determined by size of the variable space, and the corresponding block diagonal matrix structure.   
%
%\subsubsection{Optimization over $\mathbb{V},\mathcal{T},\mathcal{C}$}
%The size of the variable space is given as $n= 2K \left( 4 + \sum_{i\in\mathbb{I}} d_iN_i  \right)$. Moreover, the block sizes are calculated as $l_m = 2 + 2 K d_i N_i, \; \forall i \in \mathbb{I}$, corresponding to the (\ref{eq:p4_power}), and as $l_m = 2+ 2\tilde{d}_{ij} + 2M_iN_j, \; \forall i,j \in \mathbb{I},k\in\mathbb{F}_K$, corresponding to (\ref{eq:p4_lambda_tau}). The overall number of the blocks is calculated as $M=2+4K$.
%\subsubsection{Optimization over $\mathbb{U},\mathcal{T},\mathcal{C}$}
%The size of the variable space is given as $n= 2K \left( 4 + \sum_{i\in\mathbb{I}} d_i M_i  \right)$. Block sizes are calculated similar to the previous case (optimization over $\mathbb{V}$). The block sizes are calculated as $l_m = 2+ 2\tilde{d}_{ij} + 2M_iN_j, \; \forall i,j \in \mathbb{I},k\in\mathbb{F}_K$, corresponding to (\ref{eq:p4_lambda_tau}). The overall number of the blocks is calculated as $M=4K$.
%
%
%\subsubsection{Optimization over $\mathbb{W},\mathcal{T},\mathcal{C}$}
%A general form of a MAX-DET problem is defined as 
%\begin{align}
%\underset{\ma{z}}{\text{min}} \;\; \ma{p}^T \ma{z} + \text{log}\left|{\ma{Y}(\ma{z})}^{-1}\right|, \;\; {\rm{s.t.}} \;\; {\ma{Y}(\ma{x})} \succ 0,\; {\ma{F}(\ma{x})} \succeq 0, 
%\end{align}  
%where $\ma{z}\in \real^n$, and 
%\begin{align}
%& {\ma{Y}(\ma{z})} \in \real^{n_Y \times n_Y} := \ma{Y}_0 + \sum_{i=1}^{n} {z_i \ma{Y}_i}, \nonumber \\
%& {\ma{F}(\ma{z})} \in \real^{n_F \times n_F} := \ma{F}_0 + \sum_{i=1}^{n} {z_i \ma{F}_i}. \nonumber
%\end{align}
%an upper bound to the computational complexity of the above problem is given as
%\begin{align}
%\mathcal{O}\Big( \sqrt{n} \big(n^2 + n_Y^2 \big) n_F^2 \Big),
%\end{align}
%see \cite[Section~10]{vandenberghe1998determinant}. In the current optimization problem, the variable dimentions are obtained as $n = 2K \left( 4 + \sum_{i\in\mathbb{I}} d_i^2\right) $, $n_F = 8K\left(1+ 1\tilde{d}_{ij} + 1M_iN_j\right)$, and $n_Y = 2Kd_i$. 
%\subsubsection{Remarks}
%The above analysis intends to show how the bounds on computational complexity are related to different dimensions in the problem structure. Nevertheless, the computational load may vary in practice, and depending on the used numerical solver. Furthermore, the overall algorithm complexity also depends on the number of optimization iterations required to obtain convergence. Please see Subsection~\ref{sim_numericalcomplexityanalysis} for the convergence behavior, as well as a numerical evaluation of the algorithm computational complexity.
  %
%%\subsubsection{Calculation of $\ma{U}$}
%%The size of the variable space is given as $n=  1 + 4|\mathcal{I}| + 2T \sum_{i\in \mathcal{I}} M_i d_i$, $K = 2|\mathcal{I}|$, $a_k = 1 + \tilde{d}_{ij} + M_iN_j,\;\forall i,j$.
%%\subsubsection{Calculation of $\ma{W}$}
%%Similar to the last parts we calculate $n=  1 + 4|\mathcal{I}| + 2T \sum_{i\in \mathcal{I}} d_i^2$, $K = 2|\mathcal{I}|$, $a_k = 1 + \tilde{d}_{ij} + M_iN_j,\;\forall i,j$.
%%
%%Note that the discussed complexity measure refers to the required arithmetic operations of each optimization step. The overall arithmetic complexity is also impacted by the number of necessary optimization iterations, which is numerically studied in Section~\ref{sec:simulations}.  
%
%
  %
%%\begin{lemma}
%%The inner optimization part in (\ref{}) 
%%\begin{align}
%%\underset{ {\tau} }{ \text{max}} \;\; \underset{ {\Delta} }{ \text{min}}   \;\; -  \sum_{i,j \in \mathcal{D}} \tau_{ij} \;\;
%%{\rm s.t.} \;\; \text{(12), (13)}
%%\end{align} 
%%can be equivalently written as 
%
%\begin{algorithm}[H] 
 %\small{	\begin{algorithmic}[1] 
  %%\SetAlgoLined
%\State{$\ell \leftarrow  {0}  ;  \;\;\;\; \text{(set iteration number to zero)}$}
%\State{$\ma{V}_i,\ma{U}_i \leftarrow  \ma{0}, \; \ma{W}_i \leftarrow  \ma{I}_{d_i} ; \;\;\;\; \text{(initialization)}$}
%\Repeat 
%\State{$\ell \leftarrow  \ell + 1;$}
%\State{$\mathbb{V}, \mathcal{T}, \mathcal{C} \leftarrow \text{solve SDP (\ref{eq:global_opt_problem_4}), with fixed} \; \mathbb{U},\mathbb{W};$}
%
%\State{$\mathbb{U}, \mathcal{T}, \mathcal{C} \leftarrow \text{solve SDP (\ref{eq:global_opt_problem_4}), with fixed} \; \mathbb{V},\mathbb{W};$}
%
%\State{$\mathbb{W}, \mathcal{T}, \mathcal{C} \leftarrow \text{solve MAX-DET (\ref{eq:global_opt_problem_4}), with fixed} \; \mathbb{U},\mathbb{V};$}
%
%\Until{$\text{a stable point, or maximum number of $\ell$ reached}$}
%
%\State{\Return$\left\{\mathbb{W},\mathbb{U},\mathbb{V}\right\}$}
%
  %\end{algorithmic} } 
 %\caption{\small{Iterative semi-definite-programming (SDP) framework for worst-case sum rate maximization in a Bidirectional FD system} } \label{alg_1}
%\end{algorithm}   	




==> Sections/sec_WMMSE_CSI_Error.tex <==
In many realistic scenarios the CSI matrices can not be estimated or communicated accurately due to the limited channel coherence time as a result of, e.g., reflections from a moving object, or due to dedicating limited resource on the training/feedback process. This issue becomes more significant in a FD system, due to the strong self-interference channel which calls for dedicated silent times for tuning and training process, see~\cite[Subsection~III.A]{DMBS:12}. In particular, the impact of CSI error on the defined MC FD system is three-fold. Firstly, similar to the usual HD scenarios, it results in the erroneous equalization in the receiver, as the communication channels are not accurately known. Secondly, it results in an inaccurate estimation of the received signal from the self-interference path, and thereby degrades the SIC quality. Finally, due to the CSI error, the impact of the distortion signals may not be accurately known, as the statistics of the distortion signals directly depend on the channel situation. In this part we extend the proposed designs in Section~\ref{sec:WMMSE} where the aforementioned uncertainties, resulting from CSI error, are also taken into account. 

\subsection{Norm-bounded CSI error}
In this part we update the defined system model in Section~\ref{sec:model} to the scenario where the CSI is known erroneously. In this respect we follow the so-called deterministic model \cite{WP:09}, where the error matrices are not known but located, with a sufficiently high probability, within a known feasible error region. This is expressed as 
\begin{align} \label{eq:model_channel_eror}
\ma{H}_{ij}^{k} =  \tilde{\ma{H}}_{ij}^{k} + {\ma{\Delta}}_{ij}^{k}, \;\; {\ma{\Delta}}_{ij}^{k} \in \mathbb{D}_{ij}^{k}, \;\; i,j\in\mathbb{I},
\end{align}
and
\begin{align} \label{eq:model_channel_eror}
\mathbb{D}_{ij}^{k} :=  \left\{ {\ma{\Delta}}_{ij}^{k} \; \big{\vert} \;  \| {\ma{D}}_{ij}^{k} {\ma{\Delta}}_{ij}^{k} \|_F \leq \zeta_{ij}^{k} \right\}, \;\; \forall i,j \in\mathbb{I}, \; k \in \mathbb{F}_{K},
\end{align}
where $\tilde{\ma{H}}_{ij}^{k}$ is the estimated channel matrix and ${\ma{\Delta}}_{ij}^{k}$ represents the channel estimation error. Moreover, ${\ma{D}}_{ij}^{k}\succeq 0$ and $\zeta_{ij}^{k} \geq 0$ jointly define a feasible ellipsoid region for ${\ma{\Delta}}_{ij}^{k}$ which generally depends on the noise and interference statistics, and the used channel estimation method. For further elaboration on the used error model see \cite{WP:09,LB:05,PPNL:06} and the references therein.  \\
The aggregate interference-plus-noise signal at the receiver is hence updated as  
\begin{align} \label{model:ri_signal_CSIError}
{\boldsymbol{\nu}}_{i}^k & = \ma{H}_{ij}^k \ma{e}_{\text{t},j}^k + \ma{H}_{ii}^k \ma{e}_{\text{t},i}^k + \ma{e}_{\text{r},i}^k + \ma{\Delta}_{ij}^k \ma{V}_{j}^k \ma{s}_{j}^k + \ma{n}_{i}^k, \;\; j \neq i \in \mathbb{I},
\end{align}
where $\ma{\Sigma}_i^k$, representing the covariance of ${\boldsymbol{\nu}}_{i}^k$, is expressed in (\ref{eq_model_aggregate_interference_covariance_CSIError}).  

\begin{figure*}[!ht]
\normalsize
\begin{align} \label{eq_model_aggregate_interference_covariance_CSIError}
\ma{\Sigma}_{i}^k & = \ma{\Delta}_{ij}^k \ma{V}_j^k{\ma{V}_j^k}^H {\ma{\Delta}_{ij}^k}^H \nonumber \\
%%%%%+ \ma{H}_{ii}^k \ma{\Theta}_{\text{tx},i}^k \text{diag} \left( \sum_{k \in \mathbb{F}_K } \ma{V}_i^k{\ma{V}_i^k}^H \right)  {\ma{H}_{ii}^k}^H 
%%%%%+ \ma{H}_{ij}^k \ma{\Theta}_{\text{tx},j}^k \text{diag} \left( \sum_{k \in \mathbb{F}_K } \ma{V}_j^k{\ma{V}_j^k}^H \right) {\ma{H}_{ij}^k}^H  \nonumber \\
%%%%%& + \ma{\Theta}_{\text{rx},i}^k   \text{diag} \left( \sum_{k\in\mathbb{F}_K}  \sigma_{i,k}^2 \ma{I}_{M_i} + \ma{H}_{ii}^k \ma{V}_i^k{\ma{V}_i^k}^H {\ma{H}_{ii}^k}^H + \ma{H}_{ij}^k \ma{V}_j^k{\ma{V}_j^k}^H {\ma{H}_{ij}^k}^H   \right)  + \sigma_{i,k}^2 \ma{I}_{M_i} . 
&  +  \sum_{ j \in \mathbb{I} } \ma{H}_{ij}^k \ma{\Theta}_{\text{tx},j}^k \text{diag} \left( \sum_{l \in \mathbb{F}_K } \ma{V}_j^l{\ma{V}_j^l}^H \right) {\ma{H}_{ij}^k}^H + \ma{\Theta}_{\text{rx},i}^k   \text{diag} \bigg( \sum_{l\in\mathbb{F}_K}  \bigg(   \sigma_{i,l}^2 \ma{I}_{M_i}  + \sum_{ j \in \mathbb{I} } \ma{H}_{ij}^l \ma{V}_j^l{\ma{V}_j^l}^H {\ma{H}_{ij}^l}^H   \bigg) \bigg)  + \sigma_{i,k}^2 \ma{I}_{M_i}.
\end{align}
\hrulefill
\vspace*{-0mm}
\end{figure*}

%\subsection{Impact of CSI error}
%The impact of CSI error on the defined FD system is three-fold. Firstly, it degrades the self-interference cancellation, as the self-interference channel is not accurately known. In this regard, the signal passing through the error part of the self-interference channel may not be correctly estimated/cancelled. Secondly, due to the CSI inaccuracy, the impact of the distortion signals may not be correctly known, as the CSI error directly modifies the statistics of the distortion signals.   Finally, similar to the usual HD scenarios the CSI uncertainty results in the uncertain beamforming/equalization of the transmitted symbols, as the communication channels are not known. 
%In the following, we propose a minimum worst-case MSE design, taking into account all of the aforementioned uncertainties.       

\subsection{Alternating SDP (AltSDP) for worst-case MSE minimization} \label{WMMSE_CSI_Error}
An optimization problem for minimizing the worst-case MSE under the defined norm-bounded CSI error is written as 
%\begin{subequations}  
\begin{align}
\underset{\mathbb{V},\mathbb{U}}{ \text{min}} \;\; \underset{\mathbb{C}}{\text{max}} \;\;  & \sum_{i \in \mathbb{I}}\sum_{k \in \mathbb{F}_K}  \text{tr} \left({\ma{S}_i^k} \ma{E}_i^k\right),   \nonumber \\ 
 {\text{s.t.}} \;\;\; &  \text{(\ref{eq:global_opt_problem_MWMSE_b})}, \;\; \ma{\Delta}_{ij}^{k} \in \mathbb{D}_{ij}^{k}, \;\;  \forall i,j \in \mathbb{I}, \;\;  k \in \mathbb{F}_K,   \label{eq:global_opt_problem_MWMSE_CSIError}
\end{align}  
%\end{subequations}
where $\mathbb{C} := \{\ma{\Delta}_{ij}^k, \; \forall i,j \in \mathbb{I} , \;\forall k \in \mathbb{F}_K\}$, and $\ma{E}_{i}^k$ is obtained from (\ref{MSE_Matrix}) and (\ref{eq_model_aggregate_interference_covariance_CSIError}). Note that the above problem is intractable, due to the inner maximization of quadratic convex objective over $\mathbb{C}$, which also invalidates the observed convex QCP structure in (\ref{eq:global_opt_problem_MWMSE}). In order to formulate the objective into a tractable form, we calculate
%%%%\begin{align} 
%%%%\sum_{k\in \mathbb{F}_K} \text{tr} \left({\ma{W}_i^k}^H \ma{E}_i^k\ma{W}_i^k\right) \; {=} \; {\sum_{j \in \mathbb{I} }  \sum_{k \in \mathbb{F}_K } \big\| \tilde{\ma{c}}_{ij}^k + \ma{C}_{ij}^k  \ma{\Delta}_{ij}^k \big\|_{2}^2} , \label{quadratic_error_representation_final_CSIError}
%%%%\end{align}
%%%%where $\tilde{\ma{c}}_{ij}^k$ are obtained similar to that of (\ref{calculate_c_ii}) and (\ref{calculate_c_ij}) by replacing the channel values $\ma{H}_{ij}^k$ by the estimated ones, i.e, $\tilde{\ma{H}}_{ij}^k$, and 
%%%%\begin{align}\label{calculate_C_ii}
%%%%&\ma{C}_{ii}^k := \nonumber \\ & \left[ \begin{array}{c} {\ma{V}_i^k}^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \\ \left\lfloor  \left(  \left( \ma{\Theta}_{\text{tx},i}^k  \right)^{\frac{1}{2}} \ma{\Gamma}_{N_i}^l \ma{V}_i^m \right)^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \right\rfloor_{l \in \mathbb{F}_{N_i}, m \in \mathbb{F}_K} \\  \left\lfloor  {\ma{V}_i^k}^T \otimes \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^m  \right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m\in \mathbb{F}_K} \\ \ma{0}_{M_i d_i \times M_i N_i}  \end{array} \right],
%%%%\end{align}
%%%%\begin{align}\label{calculate_C_ij}
%%%%& \ma{C}_{ij}^k \stackrel{i \neq j}{:=}  \nonumber \\ &\left[ \begin{array}{c} \left\lfloor   \left(  \left( \ma{\Theta}_{\text{tx},j}^k  \right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^{l} \ma{V}_j^m \right)^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \right\rfloor_{l \in \mathbb{F}_{N_j} , m\in \mathbb{F}_K}  \\ \left\lfloor {\ma{V}_j^k}^T \otimes \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^k   \right)^{\frac{1}{2}} \ma{\Gamma}_{M_i}^l \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K }  \\    {\ma{V}_j^k}^T \otimes  \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H  \right)  \end{array} \right],
%%%%\end{align}    
%%%%where $\ma{C}_{ij}^k \in \compl^{ \tilde{d}_{ij} \times {M_i N_j}}$. 
\begin{align}
& \sum_{k\in \mathbb{F}_K} \text{tr} \left({\ma{S}_i^k} \ma{E}_i^k \right) \nonumber \\ & =  \sum_{k\in \mathbb{F}_K} \Bigg{(}
\left\| {\ma{W}_i^k}^H \left( {\ma{U}_i^k}^H \ma{H}_{ii}^k \ma{V}_i^k - \ma{I}_{d_i} \right) \right\|_{{F}}^2 \nonumber \\
 & \;\;\;\; + \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \ma{\Delta}_{i3-i}^k \ma{V}_{3-i}^k   \right\|_{{F}}^2 + \sigma_{i,k}^2 \left\|  {\ma{W}_i^k}^H {\ma{U}_i^k}^H\right\|_{{F}}^2 \nonumber   \\
 %%%& \;\;\;\; + \sum_{l\in \mathbb{F}_{N_i}}  \sum_{m\in \mathbb{F}_K }   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \ma{H}_{ii}^k \left(\ma{\Theta}_{\text{tx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{N_i}^l  \ma{V}_i^m   \right\|_{{F}}^2  \nonumber   \\
 & \;\;\;\; + \sum_{j \in \mathbb{I} } \sum_{l\in \mathbb{F}_{N_j}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \ma{H}_{ij}^k \left(\ma{\Theta}_{\text{tx},j}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^l  \ma{V}_j^m   \right\|_{{F}}^2  \nonumber \\
 %%%& \;\;\;\; + \sum_{l\in \mathbb{F}_{M_i}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \left(\ma{\Theta}_{\text{rx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l  \ma{H}_{ii}^m\ma{V}_i^m   \right\|_{{F}}^2  \nonumber \\
 & \;\;\;\; + \sum_{j \in \mathbb{I} } \sum_{l\in \mathbb{F}_{M_i}}  \sum_{m\in \mathbb{F}_K}   \left\| {\ma{W}_i^k}^H {\ma{U}_i^k}^H \left(\ma{\Theta}_{\text{rx},i}^k\right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l  \ma{H}_{ij}^m\ma{V}_j^m   \right\|_{{F}}^2  \nonumber \\
 & \;\;\;\;+ \left\|  {\ma{W}_i^k}^H {\ma{U}_i^k}^H   \left( \ma{\Theta}_{\text{rx},i}^k  \sum_{q\in\mathbb{F}_K} \sigma_{i,q}^2  \right)^{\frac{1}{2}}  \right\|_{F}^2 \Bigg{)}  \label{error_representation_fro_norm} \\
& = {\sum_{j \in \mathbb{I} }  \sum_{k \in \mathbb{F}_K } \Big\| \ma{c}_{ij}^k + \ma{C}_{ij}^k \text{vec}\left( \ma{\Delta}_{ij}^k \right) \Big\|_{2}^2 } ,  \label{quadratic_error_representation_final}
 %& + \sum_{l\in \mathbb{F}_{N_i}}  \kappa_i  \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{H}_{ii}   \ma{\Gamma}_l \ma{V}_i   \right{\|}_{{F}}^2 \hspace{-0mm} +  \sum_{l\in \mathbb{F}_{M_i}}  \beta_i   \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{\Gamma}_l \ma{H}_{ii}   \ma{V}_i   \right{\|}_{{F}}^2 \nonumber  \\ 
 %& + \left{\|} \ma{W}_i^H \ma{U}_i^H \ma{\Delta}_{ij} \ma{V}_j   \right{\|}_{{F}}^2 + \sigma_{\text{n},i}^2 \left{\|}  \ma{W}_i^H \ma{U}_i^H\right{\|}_{{F}}^2,  \\
%& = \boxed{\sum_{j \in \mathcal{D} } \left{\|} \ma{c}_{ij} + \ma{C}_{ij} \text{vec}\left( \ma{\Delta}_{ij} \right) \right{\|}_{2}^2 } ,  \label{quadratic_error_representation_final}
\end{align}  
%\end{subequations}
where $\ma{\Gamma}_{M}^l$ is an $M \times M$ zero matrix except for the $l$-th diagonal element equal to $1$. In the above expressions $\ma{W}_{i}^k = \left( \ma{S}_{i}^k \right)^{\frac{1}{2}}$, and 
%%%\begin{align} \label{calculate_c_ii}
%%%& \ma{c}_{ij}^k :=  \nonumber \\   & \left[ \begin{array}{c} \text{vec} \left( {\ma{W}_i^k}^H \left( {\ma{U}_i^k}^H \tilde{\ma{H}}_{ii}^k\ma{V}_i^k  - \ma{I}_{d_i}   \right) \right) \\ \left\lfloor \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \tilde{\ma{H}}_{ii}^k  \left( \ma{\Theta}_{\text{tx},i}^k \right)^{\frac{1}{2}}     \ma{\Gamma}_{N_i}^l \ma{V}_i^m \right) \right\rfloor_{l \in \mathbb{F}_{N_i}, m \in \mathbb{K}  } \\  \left\lfloor \text{vec} \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^m \right)^{\frac{1}{2}}     \ma{\Gamma}_{M_i}^l \tilde{\ma{H}}_{ii}^k \ma{V}_i^k \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{K} }    \\  \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H  \left( \sigma_{i,k}^2 \ma{I}_{M_i} + \ma{\Theta}_{\text{rx},i}^k \sum_{m \in \mathbb{K}} \sigma_{i,m}^2   \right)^{\frac{1}{2}}  \right)  \\   
%%%\end{array} \right], 
%%%\end{align}
%%%\begin{align}\label{calculate_C_ii}
%%%&\ma{C}_{ii}^k := \nonumber \\ & \left[ \begin{array}{c} {\ma{V}_i^k}^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \\ \left\lfloor  \left(  \left( \ma{\Theta}_{\text{tx},i}^k  \right)^{\frac{1}{2}} \ma{\Gamma}_{N_i}^l \ma{V}_i^m \right)^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \right\rfloor_{l \in \mathbb{F}_{N_i}, m \in \mathbb{K}} \\  \left\lfloor  {\ma{V}_i^k}^T \otimes \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^m  \right)^{\frac{1}{2}}  \ma{\Gamma}_{M_i}^l \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m\in \mathbb{K}} \\ \ma{0}_{M_i d_i \times M_i N_i}  \end{array} \right],
%%%\end{align}
\begin{align}\label{calculate_c_ij}
& \ma{c}_{ij}^k {:=}  \nonumber \\   &\left[ \begin{array}{c} \delta_{ij} \text{vec} \left( {\ma{W}_i^k}^H \left( {\ma{U}_i^k}^H \tilde{\ma{H}}_{ij}^k\ma{V}_j^k  -  \ma{I}_{d_j \delta_{ij}}   \right) \right)  \\   \left\lfloor \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \tilde{\ma{H}}_{ij} \left( \ma{\Theta}_{\text{tx},j}^k  \right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^l   \ma{V}_j^m \right) \right\rfloor_{l \in \mathbb{F}_{N_j} , m \in \mathbb{F}_K}   \\ \left\lfloor \text{vec} \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H  \left( \ma{\Theta}_{\text{rx},i}^m  \right)^{\frac{1}{2}} \ma{\Gamma}_{M_{i}}^l \tilde{\ma{H}}_{ij}^k  \ma{V}_j^k \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K } \\   \delta_{ij} \text{vec} \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H  \left( \sigma_{i,k}^2 \ma{I}_{M_i} + \ma{\Theta}_{\text{rx},i}^k \sum_{m \in \mathbb{F}_K} \sigma_{i,m}^2 \right)^{\frac{1}{2}} \right) \end{array} \right], 
\end{align}
\begin{align}\label{calculate_C_ij}
& \ma{C}_{ij}^k {:=}  \nonumber \\ &\left[ \begin{array}{c}  {\ma{V}_j^k}^T \otimes  \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H  \right)  \\
\left\lfloor  \left(  \left( \ma{\Theta}_{\text{tx},j}^k  \right)^{\frac{1}{2}}  \ma{\Gamma}_{N_j}^{l} \ma{V}_j^m \right)^T \otimes \left( {\ma{W}_i^k}^H {\ma{U}_i^k}^H \right) \right\rfloor_{l \in \mathbb{F}_{N_j} , m\in \mathbb{F}_K}  \\ \left\lfloor {\ma{V}_j^k}^T \otimes \left( {\ma{W}_i^m}^H {\ma{U}_i^m}^H \left( \ma{\Theta}_{\text{rx},i}^k   \right)^{\frac{1}{2}} \ma{\Gamma}_{M_i}^l \right) \right\rfloor_{l \in \mathbb{F}_{M_i}, m \in \mathbb{F}_K } \\ \ma{0}_{M_i d_i \times M_i N_i}  \end{array} \right],
\end{align}
where $\delta_{ij}$ is the Kronecker delta where $\delta_{ij}=1$ for $i=j$ and zero otherwise. Moreover we have $\ma{c}_{ij}^k \in \compl^{ \tilde{d}_{ij} \times 1}$, $\ma{C}_{ij}^k \in \compl^{ \tilde{d}_{ij} \times {M_i N_j}}$ such that  
\begin{align}\label{length_d}
%& \tilde{d}_{ii} := d_i^2 \left( 1 + K \left( N_i + M_i \right) \right) + d_iM_i,  \\
& \tilde{d}_{ij} :=  d_id_j \left( 1 + K \left( N_j + M_i \right) \right) + d_i M_i .
\end{align}
Please note that (\ref{error_representation_fro_norm}) is obtained by recalling (\ref{MSE_Matrix}) and (\ref{eq_model_aggregate_interference_covariance_CSIError}) and the known matrix equality \cite[Eq.~(516)]{MCB:08}, and (\ref{calculate_c_ij})-(\ref{calculate_C_ij}) are calculated via the application of \cite[Eq.~(496),~(497)]{MCB:08}. \par

By applying the Schur's complement lemma on the epigraph form of the quadratic norm (\ref{quadratic_error_representation_final}), i.e., $ \big\| \ma{c}_{ij}^k + \ma{C}_{ij}^k \text{vec}\left( \ma{\Delta}_{ij}^k \right) \big\|_{2}^2 \leq \tau_{ij}^k$, the optimization problem (\ref{eq:global_opt_problem_MWMSE_CSIError}) is equivalently written as    
\begin{subequations} \label{global_opt_problem_MWMSE_CSIError}
\begin{align}
& \underset{\mathbb{V},\mathbb{U}, \mathbb{T}} {\text{min}} \;\; \underset{\mathbb{C}}{\text{max}} \;\;   \sum_{i \in \mathbb{I}}\sum_{k \in \mathbb{F}_K}  \tau_{ij}^k,  \;\;\; {\text{s.t.}} \;\;\; \text{(\ref{eq:global_opt_problem_MWMSE_b})}, \;\; \| \ma{b}_{ij}^k \|_{F} \leq \zeta_{ij}^k,    \\    
&  \left[\hspace{-0mm}\begin{array}{cc} 0 &\hspace{-0mm}  {{{\ma{b}}_{ij}^k}}^H {{\tilde{\ma{D}}_{ij}^k}}^{H} {{\ma{C}_{ij}^k}}^H  \\   {\ma{C}_{ij}^k}{\tilde{\ma{D}}_{ij}}^k {\ma{b}}_{ij}^k  & \hspace{-0mm}\ma{0}_{\tilde{d}_{ij} \times \tilde{d}_{ij}} \end{array} \hspace{-0mm}\right] \hspace{-0mm}+\hspace{-0mm} \left[\begin{array}{cc} \tau_{ij}^k & {{{\ma{c}}_{ij}^k}}^H \\   {\ma{c}}_{ij}^k &  \ma{I}_{\tilde{d}_{ij}} \end{array} \right] \succeq 0, 
 %\\ & \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \forall i,j \in \mathbb{I}, \;\; k \in \mathbb{F}_K, \nonumber 
\end{align}
\end{subequations} 
where $\mathbb{T}:= \{\tau_{ij}^k, \; \forall i,j \in \mathbb{I}, \; \forall k \in \mathbb{F}_K\}$ and 
\begin{align}
\tilde{\ma{D}}_{ij}^k & := \ma{I}_{N_j} \otimes \left({\ma{D}_{ij}^k}\right)^{-1}, \\
\tilde{\ma{\Delta}}_{ij}^k & := \ma{D}_{ij}^k {\ma{\Delta}}_{ij}^k, \;\; \ma{b}_{ij}^k  := \text{vec}\left(\tilde{\ma{\Delta}}_{ij}^k \right), 
\end{align}
are defined for notational simplicity. The problem (\ref{global_opt_problem_MWMSE_CSIError}) is still intractable, due to the impact of the inner maximization. The following lemma translates the given structure into a tractable form. 

%By applying the Schur complement lemma, the constraint (\ref{eq:global_opt_problem_3_normbounded_contraint}) is equivalently written as 
%\begin{align}
%\left[\hspace{-0mm}\begin{array}{cc} 0 &\hspace{-0mm}  {{\ma{b}}_{ij}^k}^H {\tilde{\ma{D}}_{ij}^k}^{H} {\ma{C}_{ij}^k}^H  \\   {\ma{C}_{ij}^k}{\tilde{\ma{D}}_{ij}}^k {\ma{b}}_{ij}^k  & \hspace{-0mm}\ma{0}_{\tilde{d}_{ij} \times \tilde{d}_{ij}} \end{array} \hspace{-0mm}\right] \hspace{-0mm}+\hspace{-0mm} \left[\begin{array}{cc} \tau_{ij}^k & {\tilde{\ma{c}}_{ij}^k}^H \\   \tilde{\ma{c}}_{ij}^k &  \ma{I}_{\tilde{d}_{ij}} \end{array} \right] \succeq 0. 
%\end{align} 
%Moreover, the constraint (\ref{eq:global_opt_problem_1_normbounded_contraint}) can be equivalently written as $ \| {\ma{b}}_{ij}^k\|_2 \leq \zeta_{ij}^k$.  
%
\begin{lemma} \label{petersen}
Generalized Petersen's sign-definiteness lemma: Let $\ma{Y} = \ma{Y}^H$, and $\ma{X},\ma{P},\ma{Q}$ are arbitrary matrices with complex valued elements. Then we have
\begin{align}
\ma{Y} \succeq \ma{P}^H \ma{X} \ma{Q} + \ma{Q}^H \ma{X}^H \ma{P}, \;\; \forall \ma{X} \; : \; \| \ma{X}\|_F \leq \zeta, 
\end{align} 
if and only if 
\begin{align}
\exists \lambda \geq 0, \; \left[\begin{array}{cc} \ma{Y} - \lambda \ma{Q}^H\ma{Q} & - \zeta \ma{P}^H \\   - \zeta \ma{P} & \lambda \ma{I} \end{array} \right] \succeq 0.
\end{align} 
\end{lemma}
\begin{proof}
See~\cite[Proposition~2]{EM:04}, \cite{khlebnikov2008petersen}.
\end{proof}
By choosing the matrices in Lemma~\ref{petersen} such that $\ma{X} = {\ma{b}}_{ij}^k$, $\ma{Q} = \left[ -1, \; \ma{0}_{1 \times \tilde{d}_{ij} }  \right]$ and  
\begin{align} \label{CSI_Error_ChoosingMatrices_Lemma_Peterson}
\ma{Y} =  \left[\begin{array}{cc} \tau_{ij}^k & {{\ma{c}}_{ij}^k}^H \\   {\ma{c}}_{ij}^k & \ma{I}_{\tilde{d}_{ij}} \end{array} \right], \ma{P} = \left[\begin{array}{cc} \ma{0}_{{M_i N_j} \times 1 }, \;\; {\tilde{\ma{D}}_{ij}^k}^H {{\ma{C}}_{ij}^k}^H \end{array} \right],
\end{align} 
the optimization problem in (\ref{global_opt_problem_MWMSE_CSIError}) is equivalently written as  
\begin{subequations}  \label{Prob:MMSE_CSI_Error_final}
\begin{align}
\underset{\mathbb{V},\mathbb{U}, \mathbb{T}, \mathbb{M}}{ \text{min}}  \;\;\; & \sum_{i,j \in \mathbb{I}} \sum_{k \in \mathbb{F}_K} \tau_{ij}^k  \\
{\text{s.t.}} \;\;     &  {\ma{F}}_{i,j}^k \succeq 0,  \; \ma{G}_i \succeq 0 , \;\;  \forall i,j \in \mathbb{I},\;k \in \mathbb{F}_K, 
\end{align} 
\end{subequations}
where $\mathbb{M} :=\{\lambda_{ij}^k, \; \forall i,j \in \mathbb{I}, k \in \mathbb{F}_K \}$, and
\begin{align} 
\ma{G}_{i} :&= \left[\hspace{-0mm}\begin{array}{cc} P_i &\hspace{-0mm}  \tilde{\ma{v}}_i^H  \\ \tilde{\ma{v}}_i  & \hspace{-0mm}\ma{I}_{} \end{array} \hspace{-0mm}\right], \; \tilde{\ma{v}}_i  := \left\lfloor \text{vec} \left( \left( \ma{I} + \ma{\Theta}_{\text{tx},i} \right)^{\frac{1}{2}} \ma{V}_{i}^k \right) \right\rfloor_{k\in \mathbb{F}_K} ,\\
%\end{align}
{\ma{F}}_{i,j}^k :&= \left[\begin{array}{ccc} \tau_{ij}^k - \lambda_{ij}^k & {{\ma{c}}_{ij}^k}^H &  \ma{0}_{1 \times M_i N_j }\\  {\ma{c}}_{ij}^k & \ma{I}_{\tilde{d}_{ij}}  &  - \zeta_{ij}^k {\ma{C}}_{ij}^k\tilde{\ma{D}}_{ij}^k \\  \ma{0}_{{M_i N_j \times 1 }} & - \zeta_{ij}^k {\tilde{\ma{D}}_{ij}^k}^H {{\ma{C}}_{ij}^k}^H  &   \lambda_{ij}^k \ma{I}_{M_i N_j} \end{array} \right].
\end{align} 
Similar to (\ref{eq:global_opt_problem_rate}), the obtained problem in (\ref{Prob:MMSE_CSI_Error_final}) is not a jointly, but a separately convex problem over $\mathbb{V}$ and $\mathbb{U}$, in each case when the other variables are fixed. In particular, the optimization over $\mathbb{V},\mathbb{T}, \mathbb{M}$ is cast as an SDP, assuming a fixed $\mathbb{U}$. Afterwards, the optimization over $\mathbb{U}, \mathbb{T}, \mathbb{M}$ is solved as an SDP, assuming a fixed $\mathbb{V}$. The described alternating steps are continued until a stable point is achieved, see Algorithm~\ref{alg:WMMSECSIError} for a detailed explanation. 


\begin{algorithm}[H] 
 \small{	\begin{algorithmic}[1] 
  %\SetAlgoLined
\State{$\ell \leftarrow  {0}  ;  \;\;\;\; \text{(set iteration number to zero)}$}
\State{$\mathbb{V},\mathbb{U} \leftarrow  \text{similar~initialization~as~Algorithm~$1$}$}
%\State{$\mathbb{U} \leftarrow \text{solve~(\ref{wmmse_U_mmse})}$}
\Repeat 
\State{$\ell \leftarrow  \ell + 1$}
\State{$\mathbb{V}, \mathbb{T}, \mathbb{M} \leftarrow \text{solve SDP (\ref{Prob:MMSE_CSI_Error_final}), with fixed} \; \mathbb{U}$}
\State{$\mathbb{U}, \mathbb{T}, \mathbb{M} \leftarrow \text{solve SDP (\ref{Prob:MMSE_CSI_Error_final}), with fixed} \; \mathbb{V}$}
%\State{$\mathbb{W}, \mathbb{T}, \leftarrow \text{solve SDP (\ref{eq:global_opt_problem_rate}), with fixed} \; \mathbb{V},\mathbb{W}$}
%\State{$\mathbb{U},  \leftarrow \text{solve~(\ref{wmmse_U_mmse})}$}
\Until{$\text{a stable point, or maximum number of $\ell$ reached}$}

\State{\Return$\left\{ \mathbb{U},\mathbb{V} \right\}$}
  \end{algorithmic} } 
 \caption{\small{Alternating SDP (AltSDP) for worst-case MMSE design under CSI error.} } \label{alg:WMMSECSIError}
\end{algorithm}

\subsection{WMMSE for sum rate maximization} \label{sec:Error_CSI_Rate}
Under the impact of CSI error, the worst-case rate maximization problem is written as 
\begin{subequations} \label{eq:model_optimization_Error_CSI_Rate}
\begin{align}
\underset{\mathbb{V}}{ \text{max}} \;\; \underset{\mathbb{C} }{ \text{min}} \;\; & \;\;\sum_{i \in \mathbb{I}} \sum_{k \in \mathbb{F}_K}  I_i^k   \\
{\text{s.t.}} \;\;\; &  \text{(\ref{eq:global_opt_problem_MWMSE_b})}, \;\; \ma{\Delta}_{ij}^{k} \in \mathbb{D}_{ij}^{k}, \;\;  \forall i,j \in \mathbb{I}, \;\;  k \in \mathbb{F}_K.  \label{eq:global_opt_problem_1_normbounded_contraint_Error_CSI_Rate}
\end{align} 
\end{subequations}
Via the application of Lemma~\ref{lemma_logdetE}, and (\ref{wmmse_wmmseEquivalent}) the rate maximization problem is equivalently written as 
\begin{subequations}  \label{eq:global_opt_problem_2_Error_CSI_Rate}
\begin{align}
\underset{\mathbb{V}}{ \text{max}} \;\; \underset{\mathbb{C}}{ \text{min}}  \;\; \underset{\mathbb{U}, \mathbb{W}}{ \text{max}} \;\;  & \sum_{i \in \mathbb{I}} \sum_{k \in \mathbb{F}_K}  B \bigg( \text{log} \left|\ma{W}_i^k{\ma{W}_i^k}^H\right|  \nonumber \\ & + d_i - \text{tr} \left({\ma{W}_i^k}^H \ma{E}_i^k\ma{W}_i^k\right) \bigg) \\
{\text{s.t.}} \;\;\;\;     & \text{(\ref{eq:global_opt_problem_1_normbounded_contraint_Error_CSI_Rate})}, \label{eq:global_opt_problem_2_constraints}
\end{align} 
\end{subequations}
where $\mathbb{W}:= \{\ma{W}_{i}^k, \; \forall i \in \mathbb{I}, \; \forall k \in \mathbb{F}_K\}$. The above problem is not tractable in the current form, due to the inner min-max structure. Following the max-min exchange introduced in \cite[Section~III]{JPKR:11}, and undertaking similar steps as in (\ref{quadratic_error_representation_final})-(\ref{CSI_Error_ChoosingMatrices_Lemma_Peterson}) the problem (\ref{eq:global_opt_problem_2_Error_CSI_Rate}) is turned into 
\begin{subequations}  \label{Prob:RATE_CSI_Error_final}
\begin{align}
\underset{\mathbb{V},\mathbb{U}, \mathbb{W}, \mathbb{T}, \mathbb{M} }{ \text{max}}  \;\;\; & \sum_{i \in \mathbb{I}} \sum_{k \in \mathbb{F}_K}   B \bigg( 2 \text{log}\left|\ma{W}_i^k\right|  + d_i - \sum_{j \in \mathbb{I}} \tau_{ij}^k \bigg)  \\
{\text{s.t.}} \;\;     &  {\ma{F}}_{i,j}^k \succeq 0,  \; \ma{G}_i \succeq 0 , \;\;  \forall i,j \in \mathbb{I},\;k \in \mathbb{F}_K, 
\end{align} 
\end{subequations}
where ${\ma{F}}_{i,j}^k, \ma{G}_i$ are defined in (\ref{Prob:MMSE_CSI_Error_final}). It is observable that the transformed problem holds a separately, but not a jointly, convex structure over the optimization variable sets. In particular, the optimization over $\mathbb{V},\mathbb{T}, \mathbb{M}$ and $\mathbb{U},\mathbb{T}, \mathbb{M}$ are cast as SDP in each case when other variables are fixed. Moreover, the optimization over $\mathbb{W}$ can be efficiently implemented using the MAX-DET algorithm \cite{vandenberghe1998determinant}, see Algorithm~\ref{alg:WMMSECSIError_Rate}. Similar to Algorithm~\ref{alg:WMMSECSIError}, due to the monotonic increase of the objective in each optimization iteration the algorithm convergences to a stationary point. See \cite[Section~III]{JPKR:11} for arguments regarding convergence and optimization steps for a problem with a similar variable separation.   
\begin{algorithm}[H] 
 \small{	\begin{algorithmic}[1] 
  %\SetAlgoLined
\State{$\ell \leftarrow  {0}  ;  \;\;\;\; \text{(set iteration number to zero)}$}
\State{$\mathbb{V},\mathbb{U} \leftarrow  \text{similar~initialization~as~Algorithm~$1$}$}
\State{$\mathbb{W}, \leftarrow  \text{identity~matrix~initialization}$}

%\State{$\mathbb{U} \leftarrow \text{solve~(\ref{wmmse_U_mmse})}$}
\Repeat 
\State{$\ell \leftarrow  \ell + 1$}
\State{$\mathbb{V}, \mathbb{T}, \mathbb{M} \leftarrow \text{solve SDP (\ref{Prob:MMSE_CSI_Error_final}), with fixed} \; \mathbb{U},\mathbb{W}$}
\State{$\mathbb{U}, \mathbb{T}, \mathbb{M} \leftarrow \text{solve SDP (\ref{Prob:MMSE_CSI_Error_final}), with fixed} \; \mathbb{V},\mathbb{W}$}
\State{$\mathbb{W}, \mathbb{T}, \mathbb{M} \leftarrow \text{solve MAT-DET (\ref{Prob:MMSE_CSI_Error_final}), with fixed} \; \mathbb{V},\mathbb{U}$}
%\State{$\mathbb{W}, \mathbb{T}, \leftarrow \text{solve SDP (\ref{eq:global_opt_problem_rate}), with fixed} \; \mathbb{V},\mathbb{W}$}
%\State{$\mathbb{U},  \leftarrow \text{solve~(\ref{wmmse_U_mmse})}$}
\Until{$\text{a stable point, or maximum number of $\ell$ reached}$}

\State{\Return$\left\{ \mathbb{U},\mathbb{V} \right\}$}
  \end{algorithmic} } 
 \caption{\small{AltSDP-WMMSE algorithm for worst-case rate maximization under CSI error} } \label{alg:WMMSECSIError_Rate}
\end{algorithm}

 
  
%\subsubsection{Calculation of $\ma{U}$}
%The size of the variable space is given as $n=  1 + 4|\mathcal{I}| + 2T \sum_{i\in \mathcal{I}} M_i d_i$, $K = 2|\mathcal{I}|$, $a_k = 1 + \tilde{d}_{ij} + M_iN_j,\;\forall i,j$.
%\subsubsection{Calculation of $\ma{W}$}
%Similar to the last parts we calculate $n=  1 + 4|\mathcal{I}| + 2T \sum_{i\in \mathcal{I}} d_i^2$, $K = 2|\mathcal{I}|$, $a_k = 1 + \tilde{d}_{ij} + M_iN_j,\;\forall i,j$.
%
%Note that the discussed complexity measure refers to the required arithmetic operations of each optimization step. The overall arithmetic complexity is also impacted by the number of necessary optimization iterations, which is numerically studied in Section~\ref{sec:simulations}.  







==> Sections/sec_abstract.tex <==
 In this paper we address a worst-case weighted sum rate maximization problem for a full-duplex (FD) and multi-carrier point-to-point (P2P) system. The effects of channel-state information (CSI) error, as well as the signal distortion due to hardware impairments are jointly taken into account. This also includes the inter-carrier destruction due to the non-linear distortions in a FD transceiver. Due to the non-tractable structure of the resulting problem, a weighted minimum mean squared error (WMMSE) method is applied to cast the rate maximization problem into a separately convex optimization problem, which can be iteratively solved with a guaranteed convergence to a local optimum. Moreover, a methodology to obtain the least favorable error matrices is proposed by casting the resulting non-convex quadratic optimization into a convex optimization problem. The achievable guaranteed (worst-case) rate is then numerically studied, over different levels of CSI error and transceiver accuracy.


==> Sections/sec_discussions.tex <==
In this section we provide useful insights regarding the proposed designs in Section~\ref{sec:WMMSE} and \ref{sec:WMMSE_CSI_Error}, from the aspects of the required computational complexity, as well as the worst-case CSI error matrices. 

\subsection{Worst case CSI error} \label{WC_CSI}
It is beneficial to obtain the least favorable CSI error matrices, as they provide guidelines for the future channel estimation strategies. For instance, this helps us to choose a channel training sequence that reduces the radius of the CSI error feasible regions in the most destructive directions. Moreover, such knowledge is a necessary step for cutting-set-based methods \cite{mutapcic2009cutting} which aim to reduce the design complexity by iteratively identifying the most destructive error matrices and explicitly incorporating them into the future design steps. In the current setup, the worst-case channel error matrices are identified by maximizing the weighted MSE objective in (\ref{eq:global_opt_problem_MWMSE_CSIError}) within their defined feasible region. This is expressd as
\begin{subequations}  \label{wmmse_}
\begin{align}
\underset{{{\mathbb{C}}}}{ \text{max}} \;\;  & \sum_{i \in \mathbb{I}} \sum_{k\in\mathbb{F}_K}\text{tr}\left({\ma{W}_{i}^k}^H \ma{E}_i^k \ma{W}_{i}^k\right), \;\; \\
{\text{s.t.}} \;\;     &  \left\| \ma{D}_{ij}^k  \ma{\Delta}_{ij}^k \right\|_F \leq \zeta_{ij}^k, \;\; \forall i,j \in \mathbb{I},\; k \in \mathbb{F}_K.
\end{align} 
\end{subequations}
Due to the uncoupled nature of the error feasible set, and the value of the objective function over $\ma{\Delta}_{ij}^k$, following (\ref{quadratic_error_representation_final}), the above problem is decomposed as 
%\begin{align}
%\underset{ {\ma{b}}_{ij} }{ \text{max}} \;\;  \left{\|} \tilde{\ma{c}}_{ij} + \ma{C}_{ij} \tilde{\ma{D}}_{ij} {\ma{b}}_{ij} \right{\|}_{2}^2, \;\;\;\; {\rm s.t.} \;\;       \| {\ma{b}}_{ij} \|_2^2 \leq \zeta_{ij}^2, 
%\end{align} 
\begin{subequations} \label{find_worst_delta_3}
\begin{align} 
\underset{ {\ma{b}}_{ij}^k }{ \text{min}} \;\;  & - \left\| \ma{C}_{ij}^k \tilde{\ma{D}}_{ij}^k {\ma{b}}_{ij}^k \right\|_2^2 - 2 \text{Re}\left\{ {{\ma{b}}_{ij}^k}^H   {{\tilde{\ma{D}}_{ij}^k}}^H {\ma{C}_{ij}^k}^H  {\ma{c}}_{ij}^k \right\} -  {{\ma{c}}_{ij}^k}^H {\ma{c}}_{ij}^k \label{wwmse_worstcaseerror_nonconvexquadraticobjective}\\ {\text{ s.t.}} \;\;      & {{\ma{b}}_{ij}^k}^H {\ma{b}}_{ij}^k  \leq {\zeta_{ij}^k}^2, 
\end{align} 
\end{subequations}
where $\text{Re}\{\cdot\}$ represents the real part of a complex value. Note that the objective in (\ref{wwmse_worstcaseerror_nonconvexquadraticobjective}) is a non convex function and can not be minimized using the usual numerical solvers in the current form. Following the zero duality gap results for the non-convex quadratic problems \cite{zheng2012zero, BV:04}, we focus on the dual function of (\ref{find_worst_delta_3}). The corresponding Lagrangian function to (\ref{find_worst_delta_3}) is constructed as 
\begin{align}  \label{find_worst_delta_Lagrangian}
& \mathcal{L}\left({\ma{b}}_{ij}^k , \rho_{ij}^k \right)  =  \nonumber  \\  &  {{\ma{b}}_{ij}^k}^H  \ma{A}_{ij}^k {\ma{b}}_{ij}^k  - 2 \text{Re}\left\{ {{\ma{b}}_{ij}^k}^H   {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {\ma{c}}_{ij}^k \right\} -  {{\ma{c}}_{ij}^k}^H {\ma{c}}_{ij}^k - \rho_{ij}^k  {\zeta_{ij}^k}^2, 
\end{align} 
where $\rho_{ij}^k$ is the dual variable and 
\begin{align} 
\ma{A}_{ij}^k := \rho_{ij}^k \ma{I}_{N_jM_i} - {\tilde{\ma{D}}_{ij}^k}^H{{\ma{C}}_{ij}^k}^H{\ma{C}}_{ij}^k\tilde{\ma{D}}_{ij}^k.
\end{align} 
Consequently, the value of the dual function is obtained as 
\begin{align}
& \ma{g} \left( \rho_{ij}^k \right) = \nonumber \\ & - {{{\ma{c}}}_{ij}^k}^H  \ma{C}_{ij}^k  \tilde{\ma{D}}_{ij}^k \left(\ma{A}_{ij}^k\right)^{-1} {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {{\ma{c}}}_{ij}^k  - {{\ma{c}}_{ij}^k}^H{\ma{c}}_{ij}^k - \rho_{ij}^k {\zeta_{ij}^k}^2, 
%\left\{\begin{array}{cc} \tau_{ij} & \tilde{\ma{c}}_{ij}^H \\   \tilde{\ma{c}}_{ij} & \ma{I}_{\tilde{d}_{ij}} \end{array} \right\
\end{align}
if $ \ma{A}_{ij}^k \succeq 0$, and ${\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {{\ma{c}}}_{ij}^k \in \mathcal{R}\{\ma{A}_{ij}^k\}$, and otherwise is unbounded from below\footnote{If one of the aforementioned conditions is not satisfied, an infinitely large value of $\ma{b}_{ij}$ can be chosen in the negative direction of $\ma{A}_{ij}$, if $\ma{A}_{ij}^k$ is not positive semi-definite, or in the direction ${\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {\ma{c}}_{ij}^k$ within the null-space of $\ma{A}_{ij}^k$.}. By applying the Schur complement lemma, the maximization of the dual function is written using the epigraph form as
\begin{subequations} \label{eq:dual_channelerrormatrices}
\begin{align}
\underset{ {\rho}_{ij}^k \geq 0 , \; \phi_{ij}^k} { \text{max} } \;\;  & - \phi_{ij}^k \\  
{\rm s.t.} \;\; & \left[\begin{array}{cc} \phi_{ij}^k - {{\ma{c}}_{ij}^k}^H{\ma{c}}_{ij}^k  - {\rho}_{ij}^k {\zeta_{ij}^k}^2   & {{{\ma{c}}}_{ij}^k}^H  \ma{C}_{ij}^k  \tilde{\ma{D}}_{ij}^k  \\ {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {{\ma{c}}}_{ij}^k   & \ma{A}_{ij}^k  \end{array} \right] \succeq 0,  \label{eq:dual_channelerrormatrices_schur_semidefiniteconstraint}
\end{align} 
\end{subequations}
where $\phi_{ij}^k \in \real $ is an auxiliary variable\footnote{Note that the semi-definite presentation in (\ref{eq:dual_channelerrormatrices_schur_semidefiniteconstraint}) automatically satisfies  $ \ma{A}_{ij}^k \succeq 0$, and ${\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {{\ma{c}}}_{ij}^k \in \mathcal{R}\{\ma{A}_{ij}^k\}$.}. By plugging the obtained dual variable ${\rho}_{ij}^k$ into (\ref{find_worst_delta_Lagrangian}), and considering the fact that $- {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H \ma{C}_{ij}^k \tilde{\ma{D}}_{ij}^k + {\rho_{ij}^k}^\star \ma{I}_{N_jM_i} \succeq 0$ as a result of (\ref{eq:dual_channelerrormatrices}), the optimal value of $\ma{b}_{ij}^k$ is obtained from (\ref{find_worst_delta_Lagrangian}) as 
\begin{align}
{\ma{b}_{ij}^k}^\star = \left( - {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H \ma{C}_{ij}^k \tilde{\ma{D}}_{ij}^k + {\rho_{ij}^k}^\star \ma{I}_{N_jM_i} \right)^{-1} {\tilde{\ma{D}}_{ij}^k}^H {\ma{C}_{ij}^k}^H  {{\ma{c}}}_{ij}^k,
\end{align} 
where $(\cdot)^\star$ represents the optimality and the worst case $\ma{\Delta}_{ij}^k$ is consequently calculated via $\text{vec}(\ma{\Delta}_{ij}^k) = \tilde{\ma{D}}_{ij}^k {\ma{b}_{ij}^k}^\star$.



\subsection{Computational complexity} \label{alg_complexity}
The proposed designs in Section~\ref{sec:WMMSE} and \ref{sec:WMMSE_CSI_Error} are based on the alternative design of the optimization variables. Furthermore, it is observed that the consideration of non-linear hardware distortions, leading to inter-carrier leakage, as well as the impact of CSI error, result in a higher problem dimension and thereby complicate the structure of the resulting optimization problem. In this part, we analyze the arithmetic complexity associated with the Algorithm~\ref{sec:WMMSE_CSI_Error}. Note that Algorithm~\ref{sec:WMMSE_CSI_Error} is considered as a general framework, containing Algorithm~\ref{sec:WMMSE} as a special case, since it takes into account the impacts of hardware distortion jointly with CSI error. \par
The optimization over $\mathbb{V}, \mathbb{U}$ are separately cast as SDP. A general SDP problem is defined as 
\begin{align}
\underset{\ma{z}}{\text{min}} \;\; \ma{p}^T \ma{z}, \;\; {\text{s.t.}} \;\;  \ma{z}\in \real^n, \; \ma{Y}_0 + \sum_{i=1}^n z_i \ma{Y}_i \succeq 0, \; \|\ma{z}\|_2 \leq q,  
\end{align}
where the fixed matrices $\ma{Y}_i$ are symmetric block-diagonal, with $M$ diagonal blocks of the sizes $l_m \times l_m,\; m \in \mathbb{F}_M$, and define the specific problem structure, see \cite[Subsection~4.6.3]{ben2001lectures}. The arithmetic complexity of obtaining an $\epsilon$-solution to the defined problem, i.e., the convergence to the $\epsilon$-distance vicinity of the optimum is upper-bounded by 
\begin{align}
\mathcal{O}(1) \left(1 + \sum_{m=1}^{M} l_m  \right)^{\frac{1}{2}} \left( n^3 + n^2 \sum_{m=1}^{M} l_m^2 + n \sum_{m=1}^M l_m^3\right) \text{digit}\left( \epsilon\right), 
\end{align}
where $\text{digit}(\epsilon)$, is obtained from \cite[Subsection~4.1.2]{ben2001lectures}, and affected by the required solution precision. The required computation of each step is hence determined by size of the variable space and the corresponding block diagonal matrix structure, which is obtained in the following:   

\subsubsection{Optimization over $\mathbb{V},\mathbb{T},\mathbb{M}$}
The size of the variable space is given as $n= 2K \left( 4 + \sum_{i\in\mathbb{I}} d_iN_i  \right)$. Moreover, the block sizes are calculated as $l_m = 2 + 2 K d_i N_i, \; \forall i \in \mathbb{I}$, corresponding to the semi-definite constraint on $\ma{G}_i$, and as $l_m = 2+ 2\tilde{d}_{ij} + 2M_iN_j, \; \forall i,j \in \mathbb{I},k\in\mathbb{F}_K$, corresponding to the semidefinite constraint on $\ma{F}_{i,j}^k$ from (\ref{Prob:MMSE_CSI_Error_final}). The overall number of the blocks is calculated as $M=2+4K$.

\subsubsection{Optimization over $\mathbb{U},\mathbb{T},\mathbb{M}$}
The size of the variable space is given as $n= 2K \left( 4 + \sum_{i\in\mathbb{I}} d_i M_i  \right)$. The block sizes are calculated as $l_m = 2+ 2\tilde{d}_{ij} + 2M_iN_j, \; \forall i,j \in \mathbb{I},k\in\mathbb{F}_K$, corresponding to the semidefinite constraint on $\ma{F}_{i,j}^k$ from (\ref{Prob:MMSE_CSI_Error_final}). The overall number of the blocks is calculated as $M=4K$.
%
%
%\subsubsection{Optimization over $\mathbb{W},\mathcal{T},\mathcal{C}$}
%A general form of a MAX-DET problem is defined as 
%\begin{align}
%\underset{\ma{z}}{\text{min}} \;\; \ma{p}^T \ma{z} + \text{log}\left|{\ma{Y}(\ma{z})}^{-1}\right|, \;\; {\rm{s.t.}} \;\; {\ma{Y}(\ma{x})} \succ 0,\; {\ma{F}(\ma{x})} \succeq 0, 
%\end{align}  
%where $\ma{z}\in \real^n$, and 
%\begin{align}
%& {\ma{Y}(\ma{z})} \in \real^{n_Y \times n_Y} := \ma{Y}_0 + \sum_{i=1}^{n} {z_i \ma{Y}_i}, \nonumber \\
%& {\ma{F}(\ma{z})} \in \real^{n_F \times n_F} := \ma{F}_0 + \sum_{i=1}^{n} {z_i \ma{F}_i}. \nonumber
%\end{align}
%an upper bound to the computational complexity of the above problem is given as
%\begin{align}
%\mathcal{O}\Big( \sqrt{n} \big(n^2 + n_Y^2 \big) n_F^2 \Big),
%\end{align}
%see \cite[Section~10]{vandenberghe1998determinant}. In the current optimization problem, the variable dimentions are obtained as $n = 2K \left( 4 + \sum_{i\in\mathbb{I}} d_i^2\right) $, $n_F = 8K\left(1+ 1\tilde{d}_{ij} + 1M_iN_j\right)$, and $n_Y = 2Kd_i$. 
\subsubsection{Remarks}
The above analysis intends to show how the bounds on computational complexity are related to different dimensions in the problem structure. Nevertheless, the actual computational load may vary in practice, due to the structure simplifications and depending on the used numerical solver. Furthermore, the overall algorithm complexity also depends on the number of optimization iterations required for convergence. See Subsection~\ref{sec_AlgorithmAnalysis} for a study on the convergence behavior, as well as a numerical evaluation of the algorithm computational complexity.
  
%\subsubsection{Calculation of $\ma{U}$}
%The size of the variable space is given as $n=  1 + 4|\mathcal{I}| + 2T \sum_{i\in \mathcal{I}} M_i d_i$, $K = 2|\mathcal{I}|$, $a_k = 1 + \tilde{d}_{ij} + M_iN_j,\;\forall i,j$.
%\subsubsection{Calculation of $\ma{W}$}
%Similar to the last parts we calculate $n=  1 + 4|\mathcal{I}| + 2T \sum_{i\in \mathcal{I}} d_i^2$, $K = 2|\mathcal{I}|$, $a_k = 1 + \tilde{d}_{ij} + M_iN_j,\;\forall i,j$.
%
%Note that the discussed complexity measure refers to the required arithmetic operations of each optimization step. The overall arithmetic complexity is also impacted by the number of necessary optimization iterations, which is numerically studied in Section~\ref{sec:simulations}. 




==> Sections/sec_extensions.tex <==

In Section~\ref{sec:WMMSE} we have provided a robust rate maximization framework for a FD-P2P system, which benefits from spatial, and frequency diversity, i.e., a MIMO-MC system. On the other hand, the same framework can be extended to support further algorithm or system concepts which may become relevant in a wider range of applications. In the following we discuss some of the useful extensions which can be implemented with a minimal effort.
   
\subsection{Robust MMSE Transceiver Design} \label{subsec_MMSE}
The optimization in (\ref{eq:global_opt_problem_4}) provides a design for maximizing the system sum rate, where the rate functions are re-structured using the WMMSE method. Alternatively, an optimization problem for obtaining the optimal MMSE system operation can be formulated as
%\begin{subequations} 
\begin{align}  
\underset{{\mathbb{V}}, {\mathbb{U}}}{ \text{min}} \;\; \underset{{\mathbbl{\Delta}}}{\text{max}}  \;\; &\;\; \sum_{i \in \mathbb{I}} \mu_i \sum_{k \in \mathbb{K}} \text{tr} \left( \ma{E}_i^k\right) ,\;\; {\rm s.t.} \;\; \text{(\ref{eq:global_opt_problem_1_power_contraint}),~(\ref{eq:global_opt_problem_1_normbounded_contraint})} \label{eq:global_opt_problem_2_constraints}, \label{MMSE_global_opt_problem}
\end{align} 
%\end{subequations}
where the maximization over ${\mathbbl{\Delta}}$ represents the worst-case channel estimation error in the MMSE sense, and $\mu_i \in \real$ represents the significance of the estimation MSE at communication direction $i$. As it can be observed from (\ref{eq:global_opt_problem_3}), the defined MMSE optimization (\ref{MMSE_global_opt_problem}) can be interpreted as the special case of (\ref{eq:global_opt_problem_3}) by choosing $\nu_i = \mu_i$, and setting $\ma{W}_i^k = \ma{I}_{d_i}$ in the objective and in the definitions of $\ma{c}_{ij}^k$ and $\ma{C}_{ij}^k, \forall i,j \in \mathcal{D}, k \in \mathbb{K}$. As a result, a similar iterative optimization can be employed where at each step a convex sub-problem is solved over ${\mathbb{U}}$ and ${\mathbb{V}}$. Note that unlike the rate maximization case, where the max-min inequality is employed to construct a lower bound of the rate function, the provided framework acts on the exact sum-MSE value as the objective. Moreover, the utilization of the MAX-DET algorithm is not necessary and all sub-problems are presented as a standard SDP, due to the elimination of ${\mathbb{W}}$ from the optimization variables set. 

\subsection{Extended Power Constraints}
System power constraints usually reflect the limitations of battery, or device energy storage. Nevertheless, multiple considerations of power may become relevant for the systems with distributed antennas \cite{5963593}\footnote{In a distributed antenna system a centralized core performs joint transmit/receive processing tasks for all chains. Nevertheless, each antenna unit, or each sub-set of antennas, can be connected to a separate power sources.} or for the transceivers where an accurate operation of the chain elements are crucial. In this respect, a FD transceiver, in particular is sensitive to the operational accuracy of the hardware elements, which may become saturated or inaccurate outside of a given functional range. In this respect the consideration of per transmit antenna power constraint \cite{CZHH:14,7478064}, total or per receive antenna self-interference power constraint as may become relevant \cite{HL:14, Huberman2014, JTLH:12}. 

In order to incorporate this, we generalize the defined power constraint in (\ref{p4_power}) as
\begin{subequations}
\begin{align}  
& \ma{s}_{\text{tx},l}^T \left\lceil \text{diag}\left( \sum_{k \in \mathbb{K} }  \tilde{\ma{V}}_{i}^k \right) \right\rceil_{i \in \mathbb{I} } \leq p_{\text{tx},l},\; l \in \mathbb{C}_{\text{tx}}, \\
&\ma{s}_{\text{rx},l}^T \left\lceil \text{diag}\left( \sum_{k \in \mathbb{K} } \ma{H}_{ij} \tilde{\ma{V}}_{j}^k \ma{H}_{ij}^H \right) \right\rceil_{i \in \mathbb{I}} \leq p_{\text{rx},l}, \; \forall i \neq j \in \mathbb{I},\; l \in \mathbb{C}_{\text{rx}}, \\ 
& \left[\begin{array}{cc} \tilde{\ma{V}}_{i}^k & {{\ma{V}}_{i}^k} \\ {{\ma{V}}_{i}^k}^H & \ma{I}_{d_i}    \end{array} \right] \succeq 0, \; \forall i \in \mathbb{I}, \; k \in \mathbb{K},
\end{align}     
\end{subequations}
where $\tilde{\ma{V}}_{i}^k$ is the transmit covariance in the direction $i$ and subcarrier $k$, and $\ma{s}_{\text{tx},l}$ ($\ma{s}_{\text{rx},l}$) is a selection vector with zero and one elements, and $\mathbb{C}_{\text{tx}}$ ($\mathbb{C}_{\text{rx}}$) are the set of transmit (receive) power constraints\footnote{As an example, the choice $\ma{s}_{\text{tx},l} = [ 1 \ldots 1 ] $ represents a total transmit power from all antennas.}.   

%\subsection{Power Minimization Approach}
%In many applications it is favorable to satisfy a required quality of service, rather than to maximize the system performance. Such consideration results in the minimal resource expenditure, without compromising the required service quality by the user. In order to satisfy a required information rate for the communication direction $i$, namely $I_{\text{req,i}}$, we follow the penalty approach, see \cite[Subsection~3.1.1]{bertsekas1999nonlinear}, by introducing a price term in the objective proportional to the rate deficiency 
%\begin{subequations} \label{eq:sumpower_minimization}
%\begin{align}
%\underset{\mathbb{V}, \mathbb{U}}{ \text{max}} \;\; \underset{\mathbbl{\Delta} }{ \text{min}} \;\; &  \sum_{i \in \mathbb{I}} P_i  + \eta_i \left ( -I_{\text{req},i} + \sum_{k\in \mathbb{K} }  I_i^k \right)  \\
%{\rm s.t.} \;\;     & \text{(\ref{eq:global_opt_problem_1_power_contraint}),~(\ref{eq:global_opt_problem_1_normbounded_contraint})} \label{eq:global_opt_problem_2_constraints},
%\end{align}
%\end{subequations}
%where $\eta_i \in \real$ is the penalty weight and will be adjusted to enforce the satisfaction of the rate constraint. Following the same procedure as in (\ref{eq:model_optimization})-(\ref{eq:global_opt_problem_4}) we restructure the power minimization problem (\ref{eq:sumpower_minimization}) as 
%\begin{subequations}  \label{eq:global_opt_problem_reformulated_sumpowermin}
%\begin{align}
%\underset{\mathbb{V}, \mathbb{U}, \mathbb{W}, \mathcal{T}, \mathcal{C}} {\text{max}} \;\;\; & \sum_{i \in \mathbb{I}} P_i + \eta_i   \bigg(-I_{\text{req},i} + \sum_{k \in \mathbb{K}} 2\text{log} \left|\ma{W}_i^k\right|  + d_i - \sum_{j \in \mathbb{I}} \tau_{ij}^k \bigg) \\
%{\rm s.t.} \;\;     & \ma{\Lambda}_{i,j}^k \succeq 0,  \;\; \forall i,j \in \mathbb{I}, k \in \mathbb{K}, \label{p4_lambda_tau}\\
%&  \ma{\Omega}_i \succeq 0 , \;\;  \forall i \in \mathbb{I}, \label{p4_power}
%\end{align} 
%\end{subequations}
%where the optimization over $\mathbb{V}, \mathbb{U}, \mathbb{W}$ are performed iteratively, similar to that of (\ref{eq:global_opt_problem_4}), where a convex sub-problem for each case. Moreover, the value of $\eta_i$ is updated in the direction of the subgradient $ -I_{\text{req},i} + \sum_{k\in \mathbb{K}}  I_i^k$ after each optimization iteration. Nevertheless, the convergence of the defined algorithm is not necessarily obtained since the satisfaction of the rate constraints may not be feasible for a high value of the rate demand in both communication direction, if the transceiver accuracy is not sufficiently high.        
  
\subsection{Extension to the Multi-User Interference Channel Setup}
The proposed optimization framework in (\ref{}) consideres a multi-carrier FD communication in a P2P setup. Nevertheless, the proposed formulation can be easily extended to a scenario with multiple simultaneously active communication pairs, i.e., a FD interference channel. Such a setup gains high practical relevance, considering the trend of wireless systems towards frequency reuse and network densification, which results in the coexistence of multiple wireless communication links on the same area. In particular, while the proposed design simultaneously accounts for the inherent inaccuracies of a FD system regarding inaccurate CSI and the impacts of hardware impairments, it benefits the performance of an interference channel by simultaneously taking advantage of the additional design freedom. This includes the application of possible duplexing modes\footnote{This is since each communicating pair may now operate as a HD link in two directions, or to act as a FD link where both directions are active.}, as well as spatial (due to multiple antenna setup), and multi-carrier diversities. The two latter cases are in particular beneficial in controlling the additional interference terms in a dense communication setup, by properly assigning different beams/subchannels to the coexisting communication links. 

%In this part we extend the proposed optimization framework for a multi-carrier FD P2P setup, to serve for a more general system with multiple active FD nodes, communicating to a centralized node, i.e., a star topology. This setup in particular presents a multi-user FD cellular topology in the related literature, where all nodes may operate in FD mode, see Subsection~\ref{intro_MUMIMO} for detailed discussion of the related studies. In particular, the proposed approach, while simultaneously accounting for the inherent inaccuracies of a FD system regarding inaccurate CSI and the impacts of hardware impairments, benefits the design of a cellular system by taking advantage of the additional duplexing mode\footenote{This is since each individual link may now operate as a HD link in UL or DL directions, or to act as a FD link where both UL and DL directions are active.}, multi-user, spatial (due to multiple antenna setup), and multi-carrier diversities. The aforementioned factors are particularly effective in combating the usual challenge of FD cellular systems, regarding the co-channel interference (CCI), where the first three factors are most effective in controlling the impacts of the residual self-interference. 
%
In order to extend our design framework, we generalize the definition of the set $\mathbb{I}$ to include all communication links. In this way, each pair includes two communication links which are operating at the opposite directions. Similar to Section~\ref{sec:model}, the channel $\ma{H}_{ii}$ represents the desired channel for the link $i$, where $\ma{H}_{ij}, i \neq j$, represents the interference channel from link $j$ to link $i$. As a result, a similar signal definition is obtained via (\ref{model:transmitsignal}), (\ref{model:rx_signal}), and (\ref{model:ri_estimatedsignal}) where the aggregate interference-plus-noise on the link $i$, and in the subcarrier $k$ is redefined as 
\begin{align}
{\boldsymbol{\nu}}_{i}^k  =\ma{n}_{i}^k +  \ma{e}_{\text{r},i}^k + \ma{\Delta}_{i\bar{i}}^k \ma{V}_{\bar{i}}^k \ma{s}_{\bar{i}}^k + \hspace{-3mm} {\sum_{j \in \{\mathbb{I}\setminus \{i,\bar{i}\}\}}} \hspace{-3mm} \ma{H}_{ij}^k  \ma{x}_{j}^k  +  \hspace{-1mm} \sum_{ j\in \{i,\bar{i}\} } \hspace{-1mm} \ma{H}_{ij}^k \ma{e}_{\text{t},j}^k ,
\end{align}
where $\bar{i}\in\mathbb{I}$ is the index of the communication link at the opposite direction of the link $i$, but among the same pair of nodes. Consequently, the aggregate interference-plus-noise covariance is obtained as (\ref{eq_extension_multiplelinks_aggregate_interference_covariance}). Moreover, following the same procedure as in (\ref{MSE_Matrix})-(\ref{eq:global_opt_problem_4}), a similar optimization structure is obtained where $\ma{c}_{ij}^k$ and $\ma{C}_{ij}^k$ are redefined with the consideration of the new interference terms, see Appendix. 
\begin{figure*}[!hb]
\normalsize
\begin{align} \label{eq_extension_multiplelinks_aggregate_interference_covariance}
\ma{\Sigma}_{i}^k  & = \ma{\Delta}_{i\bar{i}}^k \ma{V}_{\bar{i}}^k{\ma{V}_{\bar{i}}^k}^H {\ma{\Delta}_{i{\bar{i}}}^k}^H +
% \sum_{j \in \mathbb{I}} \ma{\Delta}_{ij}^k \ma{V}_j^k{\ma{V}_j^k}^H {\ma{\Delta}_{ij}^k}^H 
\nonumber \\ & {\sum_{j \in \mathbb{I} }}  \ma{H}_{ij}^k \ma{\Theta}_{\text{tx},j}^k \text{diag} \left( \sum_{k \in \mathbb{K} } \ma{V}_j^k{\ma{V}_j^k}^H \right)  {\ma{H}_{ij}^k}^H  
+ \ma{\Theta}_{\text{rx},i}^k   \text{diag} \left( \sum_{k\in\mathbb{K}}  \left( \sigma_{i,k}^2 \ma{I}_{M_i} + {\sum_{j \in \mathbb{I}}}  \ma{H}_{ij}^k  \ma{V}_j^k{\ma{V}_j^k}^H {\ma{H}_{ij}^k}^H \right)    \right)  \nonumber \\ & \;\;\;\; + {\sum_{j \in \{\mathbb{I}\setminus \{i,\bar{i}\}\}}} \ma{H}_{ij}^k  \ma{V}_j^k{\ma{V}_j^k}^H   {\ma{H}_{ij}^k}^H  + \sigma_{i,k}^2 \ma{I}_{M_i}.
\end{align}
\hrulefill
\vspace*{-0mm}
\end{figure*}


%define the set \mathbb{N} representing the communication nodes. Moreover, the set $\mathbb{I}$ is extended to include all active communication links. In this regard, the link $l_i, \; i \in \mathbb{I}$ corresponds to a pair $(n_i,m_i),\; n_i \neq m_i\in \mathbb{N}$ where $n_i$ is the source and $m_i$ is the destination of the communication link $i$. The signal flow in the communication link $i\in\mathbb{I}$ is defined similar to  




==> Sections/sec_intro.tex <==

\IEEEPARstart{F}{ULL}-Duplex (FD) transceivers are known for their capability to transmit and receive at the same time and frequency, and hence have the potential to enhance the spectral efficiency~\cite{HBCJMKL:14}. Nevertheless, such systems suffer from the inherent self-interference from their own transmitter. Recently, specialized self-interference cancellation (SIC) techniques, e.g., \cite{Bharadia:14,YLMAC:11,BMK:13,JCKB:11,lee2016analog}, have demonstrated an adequate level of isolation between transmit (Tx) and receive (Rx) directions to facilitate a FD communication and motivated a wide range of related studies, see, e.g., \cite{KLH:15,HBCJMKL:14,SSDBRW:14}. A common idea of such SIC techniques is to subtract the dominant part of the self-interference signal, e.g., a line-of-sight (LOS) self-interference path or near-end reflections, in the radio frequency (RF) analog domain so that the remaining signal can be further processed in the baseband, i.e., digital domain. Nevertheless, such methods are still far from perfect in a realistic environment mainly due to \emph{i)} aging and inherent inaccuracy of the hardware (analog) elements, as well as \emph{ii)} inaccurate channel state information (CSI) in the self-interference path, due to noise and limited channel coherence time. In this regard, inaccuracy of the analog hardware elements used in subtracting the dominant self-interference path in RF domain may result in severe degradation of SIC quality. This issue becomes more relevant in a realistic scenario, where unlike the demonstrated setups in the lab environment, analog components are prone to aging, temperature fluctuations, and occasional physical damage. Moreover, a FD link is vulnerable to CSI inaccuracy at the self-interference path in environments with a small channel coherence time, see~\cite[Subsection~3.4.1]{JCKB:11}. A good example of such challenge is a high-speed vehicle that passes close to a FD device, and results in additional reflective self-interference paths\footnote{Since the object is moving rapidly, the reflective paths are more difficult to be accurately estimated.}.            
%This may render the self-interference cancellation module out of tune, and result in degradation of link quality as a result of the increased residual error.
                      
In order to combat the aforementioned issues, a FD transceiver may adapt its transmit/receive strategy to the expected nature of CSI inaccuracy, e.g., by directing the transmit beams away from the moving objects or operating in the directions with smaller impact of CSI error. Moreover, the accuracy of the transmit/receiver chain elements can be considered, e.g., by dedicating less task to the chains with noisier elements. In this regard, a widely used model for the operation of a multiple-antenna FD transceiver is proposed in \cite{DMBS:12}, assuming a single carrier communication system, where CSI inaccuracy as well as the impact of hardware impairments are taken into account. A gradient-projection-based method is then proposed in the same work for maximizing the sum rate in a FD bidirectional setup. Building upon the proposed benchmark, a convex optimization design framework is introduced in \cite{HL:14, Huberman2014, JTLH:12} by defining a price/threshold for the self-interference power, assuming the availability of perfect CSI and accurate transceiver operation. While this approach reduces the design computational complexity, it does not provide a reliable performance for a scenario with erroneous CSI, particularly regarding the self-interference path \cite{ZTH:132}. Consequently, the consideration of CSI and transceiver error in a FD bidirectional system is further studied in \cite{CWH:13, CZHH:14, CRYL:15} by maximizing the system sum rate, in \cite{6941786} by minimizing the sum mean-squared-error (MSE), and in \cite{CTLMH:16, 7562572} for minimizing the system power consumption under a required quality of service. \par 

The aforementioned works focus on modeling and design methodologies for single-carrier FD bidirectional systems, under frequency-flat channel assumptions.
In this regard, the importance of extending the previous designs for a multi-carrier (MC) system with a frequency selective channel is threefold.
Firstly, due to the increasing rate demand of the wireless services, and following the same rationale for the promotion of FD systems, the usage of larger bandwidths becomes necessary. This, in turn, invalidates the usual frequency-flat assumption and calls for updated design methodologies. 
Secondly, unlike the half-duplex (HD) systems where the operation of different subcarriers can be safely separated in the digital domain, an FD system is highly prone to the inter-carrier leakage due to the impact of hardware distortions on the strong self-interference channel\footnote{For instance, a high-power transmission in one of the subcarriers will result in a higher residual self-interference in all of the sub-channels due to, e.g., a higher quantization and power amplifier noise levels.}. This, in particular, calls for a proper modeling of the inter-carrier leakage as a result of non-linear hardware distortions for FD transceivers. And finally, the frequency diversity on the frequency selective channels shall be properly exploited to enhance the system performance.   

%  This, in particular, calls for the consideration of frequency selective channels, in a multi subchannel communication
%  System      In this work we aim at expanding the current literature on the design of FD bi-directional systems, to a multi-carrier FD communication over a frequency selective channel.  
%
%  Firstly, we consider that while the previous studies consider a single carrier communication scenario over a flat fading channel, such assumption reduces the applicability of the proposed designs to the low-rate, short-bandwidth scenarios. In this regard, the extension of the studied FD bi-directional systems to a multi-carrier setup is interesting. Nevertheless, such extension is not a trivial task for a system with FD transceivers. Note that in a traditional HD system, the design of multi-carrier transmit/receive strategies are usually coupled only due to a joint power constraint, and can be otherwise decomposed for each sub channel, e.g., see \cite{6873345,5910709}. Nevertheless, such consideration is not valid in a FD system due to the impacts of non-linear hardware impairments in the residual interference signal\footnote{For instance, a high-power transmission in one of the sub-channels will result in a higher residual self-interference in all of the sub-channels due to, e.g., higher power amplifier or quantization noise levels.}. 

\subsection{Related works on FD MC systems} \label{related_works}
In the early work by Riihonen \emph{et al.} \cite{6488955}, the performance of a combined analog/digital SIC scheme is evaluated for a FD orthogonal-frequency-division-multiplexing (OFDM) transceiver, taking into account the impact of hardware distortions, e.g., limited analog-to-digital convertor (ADC) accuracy. The problem of resource allocation and performance analysis for FD MC communication systems is then addressed in \cite{5449862,7270330,7504451,sun2016optimal,7454410,7194031,6832469}, however, assuming a single antenna transceiver.  
%
%\cite{5449862,7270330,7504451}, in the context of FD relaying, in \cite{sun2016optimal,7454410} in the context of FD cellular systems with non-orthogonal multiple access (NOMA) capability, and in \cite{6832469} for a single antenna bi-directional setup,  
In this regard, a FD MC system is studied in \cite{5449862,7270330,7504451} in the context of FD relaying, in \cite{7454410, 7194031} and \cite{sun2016optimal} in the context of FD cellular systems with non-orthogonal multiple access (NOMA) capability, and in \cite{6832469} for rate region analysis of a hybrid HD/FD link. Moreover, an MC relaying system with hybrid decode/amplify-and-forward operation is studied in \cite{ng2012dynamic}, with the goal of maximizing the system sum rate via scheduling and resource allocation. \par
%An analog SIC scheme is proposed in \cite{}, considering MIMO OFDM systems. 
In all of the aforementioned designs the behavior of the residual self-interference signal is modeled as a purely linear system. As a result, the impact of the hardware distortions leading to inter-carrier leakage, as such observed in \cite{6488955}, are neglected. Moreover, to the best of the authors knowledge, the design of a bidirectional MC MIMO system, where the communication links in opposite directions simultaneously suffer from self-interference, is still an open problem. \par 

\subsection{Contribution and paper organization}
In this paper we study a bidirectional FD MIMO OFDM system, where the impacts of hardware distortions leading to imperfect SIC and inter-subcarrier leakage are taken into account. 
%In this paper we study a worst-case weighted sum rate maximization problem for a FD and bi-directional multi-carrier system. 
Our main contributions are summarized as following:
\begin{itemize}
\item In Section~\ref{sec:model} the operation of a FD MC transceiver is modeled, taking into account the impacts of hardware impairments, following the same framework proposed in \cite{DMBS:12}. As a result, the explicit impact of hardware inaccuracies on the inter-carrier leakage is observed.
\item In Section~\ref{sec:WMMSE}, an alternating quadratic convex program (QCP), denoted as AltQCP, is proposed in order to obtain a minimum weighted MSE transceiver design. The known weighted-minimum-MSE (WMMSE) method \cite{CACC:08} is then utilized to extend the AltQCP framework for maximizing the system sum rate. For both algorithms, a monotonic performance improvement is observed at each step, leading to a necessary convergence.   

%In Section~\ref{sec:WMMSE} a weighted sum rate maximization problem is formulated in the context of a FD P2P system. Due to the intractable nature of the problem, a WMMSE-based method \cite{SRLH:11} is applied to cast the resulting problem into a separately convex problem, which facilitates a converging iterative solution. Moreover, a methodology to obtain worst-case CSI error matrices is proposed, by turning the corresponding non-convex quadratic problem into a convex problem. Analytic bounds for the arithmetic complexity of the proposed optimization method is also provided in a general case. 

\item In Section~\ref{sec:WMMSE_CSI_Error} the proposed design in Section~\ref{sec:WMMSE} is extended by also taking into account the impact of CSI error. This is done by updating the system model proposed in Section~\ref{sec:model}. Moreover, a worst-case MMSE design is proposed as an alternating semi definite program (SDP), denoted as AltSDP. Similar to the previous methods, a monotonic performance improvement is observed at each step, leading to a necessary convergence.    
%In Section~\ref{sec:extensions}, variations of the proposed design framework is given to incorporate different useful design criteria or system aspects. This includes, a robust MMSE system design, a system design with generalized power constraints, as well as a general robust sum rate maximization problem where multiple active links coexist on the same channel.  
\item In Section~\ref{sec_discussions} the computational complexity of the proposed AltSDP algorithm is analytically obtained in relation to the system dimensions. Moreover, a methodology to obtain the least favorable CSI error matrices is obtained, by transforming the resulting non-convex quadratic problem into a convex problem.

\item Finally, the proposed designs are numerically evaluated for various system parameters in Section~\ref{sec:simulations}. In particular, it is observed that the gain of utilizing a design which takes into account the impacts of inter-carrier leakage, resulting from hardware distortions, becomes significant as transceiver inaccuracy increases. The main conclusions of this paper are then summarized in Section~\ref{sec:conclusion}.
\end{itemize}

\subsection{Mathematical Notation}
Throughout this paper, column vectors and matrices are denoted as lower-case and {upper-case} bold letters, respectively. {Mathematical expectation, trace}, inverse, determinant, transpose, conjugate {and} Hermitian transpose are denoted by $ \mathbb{E}\{\cdot\}, \; {\text{tr}}(\cdot), \; (\cdot)^{-1}\; |\cdot|, \; (\cdot)^{ T},\; (\cdot)^{*}$ {and} $(\cdot)^{ H},$ respectively. The Kronecker product is denoted by $\otimes$. The identity matrix with dimension $K$ is denoted as ${\ma I}_K$ and ${\text{vec}}(\cdot)$ operator stacks the elements of a matrix into a vector. $\ma{0}_{m \times n}$ represents an all-zero matrix with size $m \times n$. $\| \cdot \|_{2}$ and $\|\cdot\|_{{F}}$ {respectively represent the Euclidean and Frobenius norms}. $\text{diag}(\cdot)$ returns a diagonal matrix by putting the off-diagonal elements to zero. $\left\lfloor \mathbf{A}_i \right \rfloor_{i=1,\ldots,K}$ denotes a tall matrix, obtained by stacking the matrices $\mathbf{A}_i,~i=1,\ldots, K$. $\mathcal{R}\{\ma{A}\}$ represents the range (column space) of the matrix $\ma{A}$. The set of real, positive real, and complex numbers are respectively denoted as $\mathbb{R}, \mathbb{R}^+ , \compl$.
 %$\ma{\Gamma}_{n}^l$ is an $n \times n$ zero matrix except for the $l$-th diagonal element equal to $1$. The Kronecker delta is denoted as $\delta_{ij}$, such that
%\begin{align}
%\delta_{ij} = \left\{ \begin{array}{cc} 1  & i=j \\ 0 & i \neq j \end{array} \right \  \nonumber 
%\end{align}  


==> acronym.tex <==
\newacronym{nnls}{NNLS}{non-negative least squares}
\newacronym{see}{SEE}{secrecy energy efficiency}
\newacronym{ee}{EE}{energy efficiency}
\newacronym{fd}{FD}{full-duplex}
\newacronym{hd}{HD}{half-duplex}
\newacronym{fdd}{FDD}{frequency division duplex}
\newacronym{tdd}{TDD}{time division duplex}
\newacronym{an}{AN}{artificial noise}
\newacronym{svd}{SVD}{singular value decomposition}
\newacronym{awgn}{AWGN}{additive white Gaussian noise}
\newacronym{sisose}{SISO-SE}{single-input, single-output, single-antenna eavesdropper}
\newacronym{mimo}{MIMO}{multiple-input multiple-output}
\newacronym{mimome}{MIMO-ME}{multiple-input, multiple-output, multiple-antenna eavesdropper}
\newacronym{dr}{DR}{dynamic range}
\newacronym{psd}{PSD}{positive semi-definite}
\newacronym{ao}{AO}{Alternating Optimisation}
\newacronym{sfp}{SFP}{Sequential Fractional Programming}
\newacronym[plural=CPUs,firstplural=Central Processing Units (CPUs)]{cpu}{CPU}{Central Processing Unit}
\newacronym{dmc}{DMC}{discrete, memoryless channel}
\newacronym{ibfd}{IBFD}{in-band full-duplex}
\newacronym{si}{SI}{self-interference}
\newacronym{ict}{ICT}{information and communications technology}
\newacronym{fp}{FP}{fractional program}
\newacronym{dc}{DC}{difference of convex}
\newacronym{scp}{SCP}{sequential convex programming}
\newacronym{giaa}{GIAA}{General Inner Approximation Algorithm}
\newacronym{kkt}{KKT}{Karush-Kuhn-Tucker}
\newacronym{qc}{QC}{quasi-concave}
\newacronym{sqc}{SQC}{strictly quasi-concave}
\newacronym{pc}{PC}{pseudo-concave}
\newacronym{spc}{SPC}{strictly pseudo-concave}
\newacronym[plural=CLFPs,firstplural=concave-linear fractional programs (CLFPs)]{clfp}{CLFP}{concave-linear fractional program}
\newacronym[plural=CCFPs,firstplural=concave-convex fractional programs (CCFPs)]{ccfp}{CCFP}{concave-convex fractional program}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{sinr}{SINR}{signal-to-interference-plus-noise ratio}
\newacronym{siso}{SISO}{single-input single-output}
\newacronym{csi}{CSI}{channel state information}
\newacronym{pdf}{PDF}{probability density function}
\newacronym{dep}{DEP}{deterministic equivalent program}
\newacronym{saa}{SAA}{sample average approximation}
\newacronym{ssum}{SSUM}{stochastic successive upper-bound minimization method}
\newacronym{gsvd}{GSVD}{generalized singular value decomposition}
\newacronym{bc}{BC}{best case}
\newacronym{wc}{WC}{worst case}
\newacronym{cdf}{CDF}{cumulative distribution function}
%\newacronym{}{}{}


==> macros.tex <==
\usepackage{bm}
%=== symbols =====================================================
%\newcommand{\ma}[1]{\bm{ #1 }}         % matrix/vector
\newcommand{\ma}[1]{\mathbf{ #1 }}         % matrix/vector

\newcommand{\ten}[1]{\ma{\mathcal #1}} % tensor
\newcommand{\set}[1]{{\mathcal #1}}    % set

\newcommand{\compl}{\mathbb{C}}        % complex-valued numbers
\newcommand{\real}{\mathbb{R}}         % real-valued numbers

%\newcommand{\eqdef}{\stackrel{.}{=}} % definition


%%%%=== functional operators ======================================
%%%\newcommand{\realof}[1]{{\rm Re}\left\{ #1 \right\}}           % real part
%%%\newcommand{\imagof}[1]{{\rm Im}\left\{ #1 \right\}}           % imaginary part
%%%\newcommand{\vecof}[1]{{\rm vec}\left\{ #1 \right\}}           % vec operator
%%%\newcommand{\unvecof}[2]{\mathop{\rm unvec}_{#2}\left\{ #1 \right\}}% unvec operator
%%%\newcommand{\diagof}[1]{{\rm diag}\left\{ #1 \right\}}         % diag operator
%%%\newcommand{\traceof}[1]{{\rm tr}\left\{ #1 \right\}}          % trace operator
%%%\newcommand{\twonorm}[1]{\left\|#1\right\|_2}                  % two-norm
%%%\newcommand{\fronorm}[1]{\left\|#1\right\|_{\rm F}}            % Frobenius norm
%%%\newcommand{\honorm}[1]{\left\|#1\right\|_{\rm H}}             % higher-order norm
%%%\newcommand{\maxof}[1]{{\rm max} \left\{ #1 \right\}}          % max
%%%\newcommand{\minof}[1]{{\rm min} \left\{ #1 \right\}}          % min
%%%\newcommand{\expvof}[1]{\mathbb{E}\left\{ #1 \right\}}         % expected value
%%%\newcommand{\expof}[1]{{\rm e}^{#1}}                           % e^{}
%%%
%%%
%%%%=== other operators ===========================================
%%%\newcommand{\argmax}{\mathop{{\arg \max}}}         % argmax
%%%
%%%%=== binary operators ===========================================
%%%\newcommand{\krp}{\diamond}  % Khatri-Rao product: A \krp B
%%%\newcommand{\kron}{\otimes}  % Kronecker product: A \kron B
%%%
%%%
%%%
%%%%=== superscripts ================================================
%%%\newcommand{\degrees}{\circ}   % e.g., 90^\degrees
%%%\newcommand{\trans}{{\rm T}}   % transpose: ^\trans
%%%\newcommand{\herm}{{\rm H}}    % hermitian: ^\herm
%%%\newcommand{\mtrans}{-{\rm T}} % inv.transpose: ^\mtrans
%%%\newcommand{\mherm}{-{\rm H}}  % inv.hermitian: ^\mherm
%%%\newcommand{\pinv}{+}          % pseudo-inverse: ^\pinv
%%%\newcommand{\conj}{*}          % complex conjugate: ^\conj
%%%
%%%
%%%
%%%%=== Tensor stuff ================================================
%%%\newcommand{\tconcat}{\mbox{\Huge \textvisiblespace \hspace{-0.2ex}} \;}
%%%\newcommand{\unf}[2]{\left[ \ten{#1} \right]_{(#2)}}
%%%\newcommand{\unfnot}[2]{\left[ #1 \right]_{(#2)}}
%%%
%%%
%%%%=== short-hand for colors =======================================
%%%%\usepackage{color}
%%%%\newcommand{\red}[1]{{\color{red} #1}}
%%%%\newcommand{\blue}[1]{{\color{blue} #1}}
%%%
%%%%=== short hand for TWR quantities ===============================
%%%\newcommand{\UT}[1]{\textsf{UT$_#1$}}
%%%\newcommand{\UTM}[2]{\textsf{UT$_#1^{(#2)}$}}
%%%\newcommand{\RS}{{\textsf{RS}}}
%%%\newcommand{\RSf}{\textsf{R}}
%%%\newcommand{\MR}{M_{\rm R}}
%%%\newcommand{\NR}{N_{\rm R}}
%%%\newcommand{\NP}{N_{\rm P}}
%%%\newcommand{\NPi}[1]{N_{\rm P,#1}}
%%%\newcommand{\PT}[1]{P_{{\rm T},#1}}
%%%\newcommand{\PN}[1]{P_{{\rm N},#1}}
%%%\newcommand{\PTR}{P_{{\rm T,R}}}
%%%\newcommand{\PNR}{P_{{\rm N,R}}}
%%%\newcommand{\PTx}{P_{{\rm T}}}
%%%\newcommand{\PNx}{P_{{\rm N}}}
%%%
%%%\newcommand{\eff}{{\rm (e)}}
%%%\newcommand{\effT}{{\rm (e)^\trans}}
%%%\newcommand{\effS}{{\rm (e)^2}}
%%%\newcommand{\eq}{{\rm (eq)}}
%%%
%%%\newcommand{\target}{{\rm (T)}}
%%%
%%%\newcommand{\forw}{{\rm (f)}}
%%%\newcommand{\forwT}{{\rm (f)^\trans}}
%%%\newcommand{\forwH}{{\rm (f)^\herm}}
%%%\newcommand{\backw}{{\rm (b)}}
%%%\newcommand{\backwT}{{\rm (b)^\trans}}
%%%\newcommand{\backwH}{{\rm (b)^\herm}}
%%%
%%%\newcommand{\forwn}{{\rm (f,0)}}
%%%\newcommand{\backwn}{{\rm (b,0)}}
%%%
%%%
%%%%=== pseudo code =================================================
%%%%\newcommand{\algorithmicinitiate}{\textbf{Initiate:}}
%%%
%%%%=== other stuff =================================================
%%%\newcommand{\note}[1]{\red{\bfseries #1}}
%%%\newcommand{\TODO}[1]{\par\red{\bfseries ***TODO: #1***}\\}


==> main06.tex <==
\chapter{Numerical Results}
\label{chap:numerical_results}
This chapter provides a numerical evaluation of all previously introduced system models and algorithms. Firstly the performance of the algorithms is evaluated. Then a reference parameter set is defined and the system performance is evaluated for this set. This result is then used as a reference point for the following performance evaluation of the impact of each system parameter on the system's performance. Furthermore, the system model extensions and the corresponding algorithms are evaluated and compared to the reference parameter set and the basic system model.

\section{Algorithm Evaluation}
\label{sec:numerical_alg_eval}
In this section the performance of the proposed algorithms are evaluated. Firstly, the performance of \ref{alg:sfp} (SFP) and \ref{alg:ao} (AO) are compared. Secondly, the proposed initialization for these algorithms is evaluated. Then the performance of \gls{ssum} and enhanced \gls{ssum} is analyzed.

In the remainder of this chapter the performance of the investigated system models is also evaluated to check if their secrecy capacity is maximized, which is usually being done in the literature. Consequently, the maximization of the \gls{see} is compared to the maximization of the secrecy capacity. A secrecy capacity maximization can also be performed with each previously introduced algorithm. Therefore, it is only necessary to ensure that the power consumption (the denominator of the \gls{see} ratio) is constantly $1$. This can simply be achieved by e.g.  setting $\alpha_i = 0$ and choosing $P_{c,i}$ accordingly.

\subsection{Performance of SFP and AO}
\label{sec:numerical_eval_SFP_AO}
In \ref{chap:mimo-me_see_maximization} two algorithms are introduced which can obtain a locally optimal solution for the problem of maximizing the \gls{see} of the introduced system model. In this section the performance of these two algorithms are evaluated. The average \gls{see}, secrecy rate and computation duration of 100 realizations over an increasing transmit power constraint is depicted in \ref{fig:numerical_sfp_ao_cmp_see}, \ref{fig:numerical_sfp_ao_cmp_cs} and \ref{fig:numerical_sfp_ao_cmp_dur}, respectively.

% Eval SFP AO performance

\begin{figure}
\centering
\subfloat[~]{\label{fig:numerical_sfp_ao_cmp_see}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				%legend entries ={FD - $\max SEE$ - SFP, FD - $\max SEE$ - AO, HD - $\max SEE$ - SFP, HD - $\max SEE$ - AO},
				xmin=-50, 
				xmax=0,
				ymin=0,
				ymax=90,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={Max. Transmit Power per Modem [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north west,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/cmp_see_sfp_ao.dat};
				\addplot table[x index=0,y index=2] {data/cmp_see_sfp_ao.dat};
				\addplot table[x index=0,y index=3] {data/cmp_see_sfp_ao.dat};
				\addplot table[x index=0,y index=4] {data/cmp_see_sfp_ao.dat};
				\addplot table[x index=0,y index=5] {data/cmp_see_sfp_ao.dat};
				\addplot table[x index=0,y index=6] {data/cmp_see_sfp_ao.dat};
				\addplot table[x index=0,y index=7] {data/cmp_see_sfp_ao.dat};
				\addplot table[x index=0,y index=8] {data/cmp_see_sfp_ao.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[~]{\label{fig:numerical_sfp_ao_cmp_cs}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				%legend entries ={FD - $\max SEE$ - SFP, FD - $\max SEE$ - AO, FD - $\max C_s$ - SFP, HD - $\max C_s$ - AO},
				xmin=-50, 
				xmax=0,
				ymin=0,
				ymax=15,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				xlabel={Max. Transmit Power per Modem [dB]},
				ylabel={$R_s$ $\left[ \text{secure bits / Hz / s} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north west,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/cmp_cs_sfp_ao.dat};
				\addplot table[x index=0,y index=2] {data/cmp_cs_sfp_ao.dat};
				\addplot table[x index=0,y index=3] {data/cmp_cs_sfp_ao.dat};
				\addplot table[x index=0,y index=4] {data/cmp_cs_sfp_ao.dat};
				\addplot table[x index=0,y index=5] {data/cmp_cs_sfp_ao.dat};
				\addplot table[x index=0,y index=6] {data/cmp_cs_sfp_ao.dat};
				\addplot table[x index=0,y index=7] {data/cmp_cs_sfp_ao.dat};
				\addplot table[x index=0,y index=8] {data/cmp_cs_sfp_ao.dat};
			\end{axis}
	\end{tikzpicture}}
	
	\subfloat[~]{\label{fig:numerical_sfp_ao_cmp_dur}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - SFP, FD - $\max SEE$ - AO, HD - $\max SEE$ - SFP, HD - $\max SEE$ - AO, FD - $\max C_s$ - SFP, FD - $\max C_s$ - AO, HD - $\max C_s$ - SFP, HD - $\max C_s$ - AO},
				xmin=-50, 
				xmax=0,
				ymin=0,
				ymax=300,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				xlabel={Max. Transmit Power per Modem [dB]},
				ylabel={Computation Duration $\left[ s \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west},
				legend style={at={(1.1,0.5)},anchor=west},
				%legend pos=outer north west,
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/cmp_dur_sfp_ao.dat};
				\addplot table[x index=0,y index=2] {data/cmp_dur_sfp_ao.dat};
				\addplot table[x index=0,y index=3] {data/cmp_dur_sfp_ao.dat};
				\addplot table[x index=0,y index=4] {data/cmp_dur_sfp_ao.dat};
				\addplot table[x index=0,y index=5] {data/cmp_dur_sfp_ao.dat};
				\addplot table[x index=0,y index=6] {data/cmp_dur_sfp_ao.dat};
				\addplot table[x index=0,y index=7] {data/cmp_dur_sfp_ao.dat};
				\addplot table[x index=0,y index=8] {data/cmp_dur_sfp_ao.dat};
			\end{axis}
	\end{tikzpicture}}
\caption{Performance comparison of \ref{alg:sfp} and \ref{alg:ao}.}
\label{fig:numerical_eval_sfp_ao}
\end{figure}

The first four curves compare the performance of the two introduced algorithms for maximizing the \gls{see} for the \gls{fd} and \gls{hd} case. The remaining four curves represent the performance for maximizing the secrecy capacity. In \ref{fig:numerical_sfp_ao_cmp_see} it can be seen  that the two algorithms achieve a similar \gls{see} performance. Furthermore it can be seen in \ref{fig:numerical_sfp_ao_cmp_cs} that \gls{sfp} achieves a slightly higher secrecy rate when maximizing for secrecy capacity in case of high transmit power constraints. As a result the \gls{see} is slightly worse. For this reason \gls{sfp} slightly outperforms \gls{hd}.

Comparing the computation duration of \gls{sfp} and \gls{ao} (see \ref{fig:numerical_sfp_ao_cmp_dur}) it can be seen that for transmit powers below \si{-30}{dB} all algorithms yield a solution very fast. However for transmit power constraints above \si{-30}{dB} the computation duration starts to deviate. For each of the two compared objectives (maximizing for \gls{see} or secrecy capacity $C_s$) and for each of the two system models (\gls{fd} and \gls{hd}) \gls{sfp} solves the problem faster than \gls{ao}. The gain of \gls{sfp} is most significant when maximizing the secrecy capacity in case of a \gls{fd} system model.

It can be concluded that both algorithms yield roughly a similar performance. Because both algorithms are independent of each other, the results are plausible. However, \gls{sfp} is significantly faster for larger transmit power constraints. For this reason the remaining evaluation is based on the \gls{sfp} algorithm.

\subsection{Evaluation of Proposed Initialization}
\label{sec:numerical_eval_init}
One of the major problems of this work is that all proposed algorithms only yield locally optimal solutions because the objective function is difficult to maximize. Therefore, it is not possible to claim global optimality with any of the proposed algorithms. The goal of this section is to evaluate the performance of the proposed algorithms in terms of optimality.

In general each of the proposed algorithms is either based on \gls{sfp} or \gls{ao}. Both approaches iteratively improve an initial solution until they converge to a stationary point of the objective function. This approach can either get stuck in a local optimum or it converges to the global optimum. Therefore, the performance of both algorithms depends heavily on the chosen initialization. In \ref{sec:initialization} a possible initialization scheme is introduced. In the remainder of this subsection the performance of this initialization is discussed.

In general the global optimum of the investigated problem can only be obtained by an exhaustive search of the set of feasible solutions, which is infeasible for large problem sizes. The following approach is proposed as a benchmark for the initialization: The initialization requires initial guesses for the three covariance matrices $\mat{Q}_{a,t}$, $\mat{Q}_{a,a}$ and $\mat{Q}_{b}$. If quantized roughly (with "1 bit"), each covariance matrix can either have a very high value (H) or a very low value (L). Because of these two quantization steps and the three variables, this results in 8 possible initializations (see \ref{tab:numerical_inits}).

\begin{table}[tb]
	\centering
	\caption{Benchmark for the initialization with uniform initialization.}
	\label{tab:numerical_inits}
	\begin{tabular}{@{}c|cccccccc@{}}
		\hline
		Initialization & 1. & 2. & 3. & 4. & 5. & 6. & 7. & 8. \\ \hline
		$\mat{Q}_{a,t}$ & L & H & L & H & L & H & L & H \\
		$\mat{Q}_{a,a}$ & L & L & H & H & L & L & H & H \\
		$\mat{Q}_{b}$ & L & L & L & L & H & H & H & H \\ \hline
	\end{tabular}
\end{table}

Now as a benchmark for each problem realization the algorithm is initialized with each of the 8 possible initializations and subsequently maximized for each of them. The benchmark performance is then obtained by taking the maximum resulting \gls{see} when maximizing \gls{see} or $C_s$ when maximizing secrecy capacity. The initializations for L are obtained by initializing the covariance matrices with $\mat{0}$. For H the covariance matrices are initialized by obtaining the structure which maximizes the energy ratio for the corresponding covariance matrix as discussed in \ref{sec:finding_a_good_structure} and then by scaling the covariance matrix such that the maximum transmit power is allocated.

% Eval init: benchmark vs proposed init
\begin{figure}
\centering
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - Bench,
					FD - $\max SEE$ - Init,
					HD - $\max SEE$ - Bench,
					HD - $\max SEE$ - Init,
					FD - $\max C_s$ - Bench,
					FD - $\max C_s$ - Init,
					HD - $\max C_s$ - Bench,
					HD - $\max C_s$ - Init},
				xmin=-50, 
				xmax=10,
				ymin=0,
				ymax=35,
				xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				xlabel={Max. Transmit Power per Modem [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west},
				legend style={at={(1.1,0.5)},anchor=west},
				%legend pos=north west,
				font=\footnotesize]
				\addplot table[x index=0,y index=2] {data/bench_data.dat};
				\addplot table[x index=0,y index=1] {data/bench_data.dat};
				\addplot table[x index=0,y index=4] {data/bench_data.dat};
				\addplot table[x index=0,y index=3] {data/bench_data.dat};
				\addplot table[x index=0,y index=6] {data/bench_data.dat};
				\addplot table[x index=0,y index=5] {data/bench_data.dat};
				\addplot table[x index=0,y index=8] {data/bench_data.dat};
				\addplot table[x index=0,y index=7] {data/bench_data.dat};
			\end{axis}
	\end{tikzpicture}
\caption{Evaluation of the performance of the proposed initialization.}
\label{fig:numerical_eval_init}
\end{figure}

\Cref{fig:numerical_eval_init} illustrates the performance of the proposed initialization (see \ref{sec:two_stage_init}) which is compared to the previously introduced benchmark initialization for 100 problem realizations over an increasing transmit power constraint. It can be seen that the performance nearly matches. The remaining offset could result from the numerical evaluation. Because of this analysis it can be assumed that the performance of the proposed initialization achieves at least a similar performance as the benchmark. Furthermore the proposed initialization requires only a single optimization instead of 8, hence reducing complexity roughly by $1/8$.

In the remainder of this chapter the numerical evaluation is only performed using the proposed initialization. A better local optimum could maybe be obtained by quantizing with a higher resolution. However, due to the increased complexity this approach is not pursuit further.

\subsection{Evaluation of SSUM for SEE Maximization}
\label{sec:numerical_eval_ssum}
In this subsection the performance of \ref{alg:stat_ssum}, which is based on \gls{ssum}, is evaluated. Because the algorithm numerically approximates the expectation operator by iteratively drawing random initialization of the gives statistics until convergence, it is interesting to compare the performance of multiple iterations of the algorithm on the same problem instance. In \ref{fig:numerical_eval_ssum} the empirical \gls{cdf} of the solutions is shown.

% Eval SSUM
\begin{figure}
\centering
\subfloat[]{\label{ig:numerical_eval_ssum01}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - SSUM, HD - $\max SEE$ - SSUM},
				%axis x discontinuity=crunch, enlargelimits=true,
				xmin=66, 
				xmax=72,
				ymin=0,
				ymax=1,
				%xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				title={Cumulative Distribution Function
},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west},
				legend style={at={(0.5,-0.3)},anchor=north},
				%legend pos=north west,
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/eval_ssum.dat};
				\addplot table[x index=2,y index=3] {data/eval_ssum.dat};
				%\addplot table[x index=4,y index=5] {data/eval_ssum.dat};
				%\addplot table[x index=6,y index=7] {data/eval_ssum.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[]{\label{ig:numerical_eval_ssum02}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max C_s$ - SSUM, HD - $\max C_s$ - SSUM},
				%axis x discontinuity=crunch, enlargelimits=true,
				xmin=20, 
				xmax=26,
				ymin=0,
				ymax=1,
				%xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				title={Cumulative Distribution Function
},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west},
				legend style={at={(0.5,-0.3)},anchor=north},
				%legend pos=north west,
				font=\footnotesize]
				%\addplot table[x index=0,y index=1] {data/eval_ssum.dat};
				%\addplot table[x index=2,y index=3] {data/eval_ssum.dat};
				\addplot table[x index=4,y index=5] {data/eval_ssum.dat};
				\addplot table[x index=6,y index=7] {data/eval_ssum.dat};
			\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of the performance of \ref{alg:stat_ssum} which is based on \gls{ssum}.}
\label{fig:numerical_eval_ssum}
\end{figure}

The results were generated by using the algorithm 100 times to solve the same problem instance. The algorithm specifications are shown in \ref{tab:numerical_ssum_stopping_criterion}, where \emph{iterations} denotes the number of algorithm evaluations, minimum average improvement denotes the minimum average improvement which is required to continue the algorithm. The moving average window size defines the size of the window over the last samples over which the average improvement is computed. Furthermore, the minimum and the maximum number of realizations represent hard thresholds on the minimum and maximum number of random realizations of the given statistical distribution which the algorithm draws. If the maximum number of realizations is reached, the algorithm terminates. This is also known as early stopping in the literature \cite{Razaviyayn2016}.

\begin{table}[tb]
	\centering
	\caption{Stopping criterion for \gls{ssum} algorithm evaluation.}
	\label{tab:numerical_ssum_stopping_criterion}
	\begin{tabular}{@{}ccccc@{}}
		\hline
		\multirow{2}{*}{Iterations} & Min. Avg. & Moving Avg. & Min. & Max. \\
		& Improvement & Window Size & Realizations & Realizations\\ \hline
		100 & $10^{-3}$ & 5 & 25 & 125\\ \hline
	\end{tabular}
\end{table}

The \gls{cdf} for maximizing for \gls{see} in case of a \gls{hd} system model as well as the \gls{cdf} for maximizing for secrecy capacity in case of a \gls{hd} system model are very narrow, which means that the algorithm will always yield a very similar solution. However for the remaining two cases the \gls{cdf} is much more broad and stretches approximately over 2 secure bits / Hz / J. This is already a significant variation. However, the accuracy of the algorithm might be increased by defining a stricter stopping criterion at the cost of increased computational complexity.

\subsection{Evaluation of Enhanced SSUM for SEE Maximization}
\label{sec:numerical_eval_essum}
Consequently the performance of the proposed extension of the \gls{ssum} algorithm, denoted as \emph{enhanced SSUM} and given by \cref{alg:stat_enhanced_ssum}, is evaluated. The algorithm parameters which are used are listed in \cref{tab:numerical_essum_stopping_criterion}. The algorithm is evaluated on 100 randomly generated problem instances. For the evaluation the mean \gls{see} and standard deviation of standard and enhanced \gls{ssum} is computed and can be found in \cref{tab:numerical_eval_essum_performance}. It can be seen that enhanced \gls{ssum} provides a small gain for the \gls{hd} system model. However for the \gls{fd} system model the gain is vanishing. A possible explanation could be that the number of \emph{negative channel realizations} is much smaller in case of \gls{fd}. This result is elaborated in \cref{sec:numeric_eval_stat_csi}.

\begin{table}[tb]
	\centering
	\caption{Stopping criterion for enhanced \gls{ssum} algorithm evaluation.}
	\label{tab:numerical_essum_stopping_criterion}
	\begin{tabular}{@{}ccccc@{}}
		\hline
		\multirow{2}{*}{Iterations} & Min. Avg. & Moving Avg. & Min. & Max. \\
		& Improvement & Window Size & Realizations & Realizations\\ \hline
		100 & $10^{-3}$ & 5 & 25 & 100\\ \hline
	\end{tabular}
\end{table}

\begin{table}[tb]
\centering
\caption{Evaluation of performance of enhanced \gls{ssum}.}
\label{tab:numerical_eval_essum_performance}
\begin{tabular}{cc|cc|cc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{}}                                                                                             & \multicolumn{2}{c|}{HD} & \multicolumn{2}{c}{FD} \\
\multicolumn{2}{c|}{}                                                                                                              & SSUM   & enhanced SSUM  & SSUM  & enhanced SSUM  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$SEE$\\ $\left[ \text{sec. bits / Hz / J} \right]$\end{tabular}} & Mean               & $20.562$ & $21.315$              & $37.299$     & $37.306$              \\
                                                                                                              & Std. dev. & $11.443$      & $11.065$              & $12.930$     & $12.914$ \\ \hline
\end{tabular}
\end{table}

\section{Reference Parameter Set}
\label{sec:numerical_reference_parameter_set}
In this section a set of reference parameters is defined. Then this reference parameter set is evaluated.

The analyzed system model mainly depends on a set of 11 parameters:
\begin{itemize}
	\item Thermal noise variance $\sigma_i^2$ of Bob ($i = b$) and Eve ($i=e$).
	\item Maximum transmit power $P_{\text{max},i}$ per modem of Alice ($i = a$) and Bob ($i = b$).
	\item Power amplifier efficiency $\alpha_i^{-1}$ of Alice ($i=a$) and Bob ($i=b$).
	\item Constant power consumption of Alice $P_{c,a}$ and Bob $P_{c,b}$.
	\item Bob's additional power consumption $P_{\text{FD}}$ due to his \gls{fd} modem.
	\item Position of Eve $pos_{\text{Eve}}$ for the case that Eve is located on the line connecting Alice and Bob. For this case it is assumed, that Alice is fixed at a position \si{0}{m} and Bob at a position \si{100}{m}.
	\item Variance of the channel coefficients of Bob's \gls{si} channel $\sigma_{SI}^2$.
	\item The transmitter noise $\kappa_i$ of Alice ($i = a$) and Bob ($i = b$) and the receiver noise $\beta_j$ of Bob ($j = b$) and Eve ($j = e$).
	\item Number of antennas of Alice $N_a$ and Bob $N_b$.
	\item Number of antennas of Eve $N_e$.
\end{itemize}
An overview of the default parameters of the system model and the range of each parameter which is evaluated can be found in \ref{tab:ref_parameters}. Note that the geometry of the reference setup places Alice, Bob and Eve on the 3 corners of an equilateral triangle. As a result all three nodes have equal distance to each other. Only for the evaluation of $pos_{\text{Eve}}$ this geometry is changed and Eve moves along the line connecting Alice and Bob. In this setup Alice and Bob are placed at a distance of \si{100}{m}.

% Table of reference parameters
\begin{table}[tb]
\centering
\caption{Set of reference parameters and range of each parameter.}
\label{tab:ref_parameters}
\begin{tabular}{c|cccccccccc}
\hline
Parameter  & \begin{tabular}[c]{@{}c@{}}$\sigma_i^2$\\ {[}dB{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$P_{max,i}$\\ {[}dB{]}\end{tabular} & $\alpha_i$ & \begin{tabular}[c]{@{}c@{}}$P_{c,i}$\\ {[}dB{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$P_{\text{FD}}$\\ {[}dB{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$pos_{\text{Eve}}$\\ {[}m{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\sigma_{SI}^2$\\ {[}dB{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\kappa_i  = \beta_j$\\ {[}dB{]}\end{tabular} & $N_a = N_b$ & $N_e$ \\ \hline
Ref. Value & -40                                                             & 0                                                              & 0.9        & -20                                                          & 0                                                                  & /                                                                    & 0                                                                  & -40                                                                      & 4           & 4     \\
Min. Value & -50                                                             & -50                                                            & 0.1        & -40                                                          & -60                                                                & 5                                                                    & -20                                                                & -60                                                                      & 2           & 2     \\
Max. Value & -10                                                             & 10                                                             & 1          & 0                                                            & 0                                                                  & 95                                                                   & 30                                                                 & 0                                                                        & 8           & 8     \\ \hline
\end{tabular}
\end{table}

In the following, four different cases will be compared in terms of \gls{see}:
\begin{enumerate}
	\item \gls{fd} Bob for maximizing the \gls{see}.
	\item \gls{hd} Bob for maximizing the \gls{see}.
	\item \gls{fd} Bob for maximizing the secrecy capacity.
	\item \gls{hd} Bob for maximizing the secrecy capacity.
\end{enumerate}

\section{Performance Evaluation for Full CSI}
\label{sec:numerical_performance_evaluation_full_csi}
In this section the performance of the previously introduced \gls{sisose} and \gls{mimome} system models for a \gls{fd} and \gls{hd} Bob is evaluated. Therefore, the impact of all system parameters on the \gls{see} is evaluated.

\subsection{Evaluation of the Impact of Thermal Noise Variance and Transmit Power}
\label{sec:numerical_eval_nvar_and_pmax}
In this subsection the impact of the thermal noise variance $\sigma_i^2$ and the maximum transmit power per modem $P_{\text{max},i}$ is evaluated. Both of them essentially change the \gls{snr} of the system, therefore the impact of both of them is studied together. The case of high thermal noise variance or low maximum transmit power is referred to as \emph{low} \gls{snr} case. Consequently, the case of low thermal noise variance or high maximum transmit power is denoted as \emph{high} \gls{snr} case.

% Eval nvar and pmax
\begin{figure}
\centering
\subfloat[SISO-SE]{\label{fig:numerical_siso_nvar}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-50, 
				xmax=-10,
				ymin=0,
				ymax=40,
				xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={Thermal Noise Variance [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north east,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/siso_nvar.dat};
				\addplot table[x index=0,y index=2] {data/siso_nvar.dat};
				\addplot table[x index=0,y index=3] {data/siso_nvar.dat};
				\addplot table[x index=0,y index=4] {data/siso_nvar.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[MIMO-ME]{\label{fig:numerical_std_nvar}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-50, 
				xmax=-10,
				ymin=0,
				ymax=250,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				xlabel={Thermal Noise Variance [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north east,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/nvar_data.dat};
				\addplot table[x index=0,y index=2] {data/nvar_data.dat};
				\addplot table[x index=0,y index=3] {data/nvar_data.dat};
				\addplot table[x index=0,y index=4] {data/nvar_data.dat};
			\end{axis}
	\end{tikzpicture}}
	
\subfloat[SISO-SE]{\label{fig:numerical_siso_pmax}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-50, 
				xmax=10,
				ymin=0,
				ymax=15,
				xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				xlabel={Max. Transmit Power per Modem [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				%legend pos=north west,
				legend style={at={(0.5,-0.3)},anchor=north},			
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/siso_pmax.dat};
				\addplot table[x index=0,y index=2] {data/siso_pmax.dat};
				\addplot table[x index=0,y index=3] {data/siso_pmax.dat};
				\addplot table[x index=0,y index=4] {data/siso_pmax.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[MIMO-ME]{\label{fig:numerical_std_pmax}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-50, 
				xmax=10,
				ymin=0,
				ymax=90,
				xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				xlabel={Max. Transmit Power per Modem [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				%legend pos=north west,
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/pmax_data.dat};
				\addplot table[x index=0,y index=2] {data/pmax_data.dat};
				\addplot table[x index=0,y index=3] {data/pmax_data.dat};
				\addplot table[x index=0,y index=4] {data/pmax_data.dat};
		\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of thermal noise variance $\sigma_i^2$ and maximum transmit power per modem $P_{\text{max},i}$ on the system's \gls{see} for the \gls{sisose} and \gls{mimome} case.}
\label{fig:eval_nvar_pmax}
\end{figure}

\Cref{fig:numerical_siso_nvar} and \ref{fig:numerical_std_nvar} characterize the \gls{see} for a varying thermal noise variance for the \gls{sisose} and \gls{mimome} case, respectively. It is assumed that the thermal noise variances at Bob and Eve are identical: $\sigma_b^2 = \sigma_e^2$. For very low $\sigma_i^2$, \gls{fd} exhibits a significant gain over \gls{hd} for maximizing the \gls{see} for both cases \gls{sisose} and \gls{mimome}. Maximizing for secrecy capacity is in general much less energy efficient. However for the \gls{mimome} case, the \gls{ee}, especially of \gls{hd}, increases for very low $\sigma_i^2$. To go on it can be seen that for $\sigma_i^2 \geq -30$ the gain of \gls{fd} over \gls{hd} is diminishing when maximizing the \gls{see}. Furthermore, for $\sigma_i^2 \rightarrow \infty$ the \gls{see} of all four schemes goes to zero.

In \ref{fig:numerical_siso_pmax} and \ref{fig:numerical_std_pmax} the \gls{see} is depicted over the maximum transmit power per modem for the \gls{sisose} and \gls{mimome} case respectively. It is assumed that Alice and Bob both have an equal maximum transmit power constraint. Note that independent and no joint transmit power constraints are assumed throughout this work.

It can be seen that the performance for the single antenna and the multiple antenna case are similar. For low transmit powers (low \gls{snr}) all four schemes perform equally. That means that maximizing for secrecy capacity is also optimal in terms of \gls{see} for low \gls{snr}. However for high transmit powers above \si{20}{dB} all four schemes start to deviate significantly: The \gls{see} of maximizing for secrecy capacity decreases significantly and approaches nearly zero. As a result maximizing for secrecy capacity is highly sub-optimal in terms of \gls{see}. Furthermore for maximizing the secrecy capacity in the \gls{mimome} case \gls{fd} performs worse than \gls{hd}. That means the increased secrecy rate of \gls{fd} enhanced physical layer security comes at high costs in terms of \gls{see}. When maximizing the \gls{see}, \gls{fd} can slightly improve the \gls{see} as compared to \gls{hd}.

To summarize: For low \gls{snr} maximizing with respect to secrecy capacity is also optimal in terms of \gls{see} and \gls{fd} can not increase the performance. In contrast for high \gls{snr} maximizing for secrecy capacity comes at a high \gls{ee} cost. Furthermore for high \gls{snr} it is possible to achieve a slight \gls{see} gain by a \gls{fd} Bob if \gls{see} maximization is applied.

\subsection{Evaluation of the Impact of the Power Consumption}
\label{sec:numeric_eval_power_consumption}
In this subsection the impact of the power amplifier efficiency $\alpha_i^{-1}$ and constant power consumption $P_{c,i}$ on the system's \gls{see} is evaluated. These two parameters are used to characterize the power consumption of Alice and Bob. It is important to evaluate the impact of these parameters because it can be expected that they have a high impact on the system's \gls{see}.

% Eval alpha and Pc
\begin{figure}
\centering
\subfloat[SISO-SE]{\label{fig:numerical_siso_alpha}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=0, 
				xmax=1,
				ymin=0,
				ymax=15,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={Power Amplifier Efficiency},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north west,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/siso_alpha.dat};
				\addplot table[x index=0,y index=2] {data/siso_alpha.dat};
				\addplot table[x index=0,y index=3] {data/siso_alpha.dat};
				\addplot table[x index=0,y index=4] {data/siso_alpha.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[MIMO-ME]{\label{fig:numerical_std_alpha}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=0, 
				xmax=1,
				ymin=0,
				ymax=100,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				xlabel={Power Amplifier Efficiency},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north west,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/alpha_data.dat};
				\addplot table[x index=0,y index=2] {data/alpha_data.dat};
				\addplot table[x index=0,y index=3] {data/alpha_data.dat};
				\addplot table[x index=0,y index=4] {data/alpha_data.dat};
			\end{axis}
	\end{tikzpicture}}
	
\subfloat[SISO-SE]{\label{fig:numerical_siso_Pc}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-40, 
				xmax=0,
				ymin=0,
				ymax=50,
				%xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				xlabel={Constant Power Consumption [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north east,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/siso_Pc.dat};
				\addplot table[x index=0,y index=2] {data/siso_Pc.dat};
				\addplot table[x index=0,y index=3] {data/siso_Pc.dat};
				\addplot table[x index=0,y index=4] {data/siso_Pc.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[MIMO-ME]{\label{fig:numerical_std_Pc}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-40, 
				xmax=0,
				ymin=0,
				ymax=600,
				%xtick={0,-40,-30,-20,-10,10,20},			
				%ytick={0,50,100,150,200},
				xlabel={Constant Power Consumption [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north east,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/Pc_data.dat};
				\addplot table[x index=0,y index=2] {data/Pc_data.dat};
				\addplot table[x index=0,y index=3] {data/Pc_data.dat};
				\addplot table[x index=0,y index=4] {data/Pc_data.dat};
		\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of power amplifier efficiency $\alpha_i$ and constant power consumption per modem $P_{c,i}$ on the system's \gls{see} for the \gls{sisose} and \gls{mimome} case.}
\label{fig:eval_alpha_Pc}
\end{figure}

The impact of the power amplifier efficiency on the system's \gls{see} is depicted in \ref{fig:numerical_siso_alpha} and \ref{fig:numerical_std_alpha}. Firstly it can be observed that the relative performance for the \gls{sisose} and \gls{mimome} case is very similar. For a low efficiency of e.g. 0.1, the performance of \gls{fd} and \gls{hd} for maximizing the \gls{see} is very similar in terms of \gls{see}. With increasing power amplifier efficiency, the \gls{see} of both systems increases. However, the rate of improvement drops for higher power amplifier efficiencies. Furthermore, \gls{fd} exhibits an increasing gain over \gls{hd} for increasing power amplifier efficiency. The maximum is obtained at a power amplifier efficiency of \si{100}{\%}.

The \gls{see} for varying constant power consumption $P_{c,i}$ is shown in \ref{fig:numerical_siso_Pc} and in \ref{fig:numerical_std_Pc}. Again the \gls{sisose} and the \gls{mimome} system model perform similarly. The \gls{see} for \gls{hd} and \gls{fd} for maximizing the secrecy capacity stays quasi constant at a very low level close to zero. In contrast, the \gls{see} increases rapidly if maximized for \gls{see} for low constant power consumptions. Furthermore there is hardly any gain of \gls{fd} over \gls{hd} for low constant power consumptions. For high constant power consumptions the \gls{see} of \gls{fd} and \gls{hd} for maximizing the \gls{see} also approaches zero. It is interesting to note that \gls{fd} exhibits the highest absolute gain over \gls{hd} if maximized for \gls{see} in the range of \si{-20}{dB} to \si{-10}{dB}.

\subsubsection{Full-Duplex Power Consumption}
\label{sec:numerical_eval_p_fd}
In this \namecref{sec:numerical_eval_p_fd} the impact of the additional power consumption $P_{\text{FD}}$ of any \gls{fd} node is evaluated. \Cref{fig:eval_p_fd} provides an overview of the results. The combined impact of $P_{\text{FD}}$ and four other parameters (thermal noise variance, power amplifier efficiency, transmitter noise / receiver distortion and strength of Bob's \gls{si} channel) is evaluated. In general it can be seen that the \gls{fd} \gls{see} approaches zero as $P_{\text{FD}} \rightarrow \infty$. In contrast the \gls{hd} performance is not effected.

% Eval P_FD
\begin{figure}
\centering
\subfloat[Thermal noise variance]{\label{fig:numerical_p_fd_nvar}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={
					FD - $\max SEE$ - $\sigma_i^2 = -50$ dB,
					HD - $\max SEE$ - $\sigma_i^2 = -50$ dB,
					FD - $\max SEE$ - $\sigma_i^2 = -40$ dB,
					HD - $\max SEE$ - $\sigma_i^2 = -40$ dB,
					FD - $\max SEE$ - $\sigma_i^2 = -30$ dB,
					HD - $\max SEE$ - $\sigma_i^2 = -30$ dB
				},
				xmin=-40, 
				xmax=0,
				ymin=0,
				ymax=250,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={FD Power Consumption $P_{\text{FD}}$ [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				%legend pos=north west,
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/nvar_pfd_data.dat};
				\addplot table[x index=0,y index=2] {data/nvar_pfd_data.dat};
				\addplot table[x index=0,y index=5] {data/nvar_pfd_data.dat};
				\addplot table[x index=0,y index=6] {data/nvar_pfd_data.dat};
				\addplot table[x index=0,y index=9] {data/nvar_pfd_data.dat};
				\addplot table[x index=0,y index=10] {data/nvar_pfd_data.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[Power amplifier efficiency]{\label{fig:numerical_p_fd_alpha}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={
					FD - $\max SEE$ - $\alpha_i^{-1} = 0.3$ dB,
					HD - $\max SEE$ - $\alpha_i^{-1} = 0.3$ dB,
					FD - $\max SEE$ - $\alpha_i^{-1} = 0.6$ dB,
					HD - $\max SEE$ - $\alpha_i^{-1} = 0.6$ dB,
					FD - $\max SEE$ - $\alpha_i^{-1} = 0.9$ dB,
					HD - $\max SEE$ - $\alpha_i^{-1} = 0.9$ dB
				},
				xmin=-40, 
				xmax=0,
				ymin=0,
				ymax=90,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={FD Power Consumption $P_{\text{FD}}$ [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				%legend pos=north west,
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/alpha_pfd_data.dat};
				\addplot table[x index=0,y index=2] {data/alpha_pfd_data.dat};
				\addplot table[x index=0,y index=5] {data/alpha_pfd_data.dat};
				\addplot table[x index=0,y index=6] {data/alpha_pfd_data.dat};
				\addplot table[x index=0,y index=9] {data/alpha_pfd_data.dat};
				\addplot table[x index=0,y index=10] {data/alpha_pfd_data.dat};
			\end{axis}
	\end{tikzpicture}}
	
\subfloat[Transmitter noise / receiver distortion]{\label{fig:numerical_p_fd_kappa_beta}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={
					FD - $\max SEE$ - $\kappa_i = \beta_j = -60$ dB,
					HD - $\max SEE$ - $\kappa_i = \beta_j = -60$ dB,
					FD - $\max SEE$ - $\kappa_i = \beta_j = -40$ dB,
					HD - $\max SEE$ - $\kappa_i = \beta_j = -40$ dB,
					FD - $\max SEE$ - $\kappa_i = \beta_j = -20$ dB,
					HD - $\max SEE$ - $\kappa_i = \beta_j = -20$ dB,
				},
				xmin=-40, 
				xmax=0,
				ymin=0,
				%ymax=15,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={FD Power Consumption $P_{\text{FD}}$ [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				%legend pos=north west,
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/kappa_beta_pfd_data.dat};
				\addplot table[x index=0,y index=2] {data/kappa_beta_pfd_data.dat};
				\addplot table[x index=0,y index=5] {data/kappa_beta_pfd_data.dat};
				\addplot table[x index=0,y index=6] {data/kappa_beta_pfd_data.dat};
				\addplot table[x index=0,y index=9] {data/kappa_beta_pfd_data.dat};
				\addplot table[x index=0,y index=10] {data/kappa_beta_pfd_data.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[Constant power consumption]{\label{fig:numerical_p_fd_Pc}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={
					FD - $\max SEE$ - $P_c = -30$ dB,
					HD - $\max SEE$ - $P_c = -30$ dB,
					FD - $\max SEE$ - $P_c = -20$ dB,
					HD - $\max SEE$ - $P_c = -20$ dB,
					FD - $\max SEE$ - $P_c = -10$ dB,
					HD - $\max SEE$ - $P_c = -10$ dB,
				},
				xmin=-40, 
				xmax=0,
				ymin=0,
				%ymax=15,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={FD Power Consumption $P_{\text{FD}}$ [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				%legend pos=north west,
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/Pc_pfd_data.dat};
				\addplot table[x index=0,y index=2] {data/Pc_pfd_data.dat};
				\addplot table[x index=0,y index=5] {data/Pc_pfd_data.dat};
				\addplot table[x index=0,y index=6] {data/Pc_pfd_data.dat};
				\addplot table[x index=0,y index=9] {data/Pc_pfd_data.dat};
				\addplot table[x index=0,y index=10] {data/Pc_pfd_data.dat};
			\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of the \gls{fd} power consumption $P_\text{FD}$ on the system's \gls{see}.}
\label{fig:eval_p_fd}
\end{figure}

The impact of the \gls{fd} power consumption on the system's \gls{see} for three different noise variances is depicted in figure \cref{fig:numerical_p_fd_nvar}. As already evaluated, the gain of \gls{fd} as compared to \gls{hd} vanishes with increasing thermal noise variance. Now comparing the amount of \gls{fd} power consumption as well, it can be seen that the maximum tolerable $P_{\text{FD}}$ decreases with increasing thermal noise variance $\sigma_i^2$. E.g. for $\sigma_i^2 = -50$ dB, \gls{fd} yields a gain for $P_{\text{FD}} < -20$ dB. However for $\sigma_i^2 = -40$ dB, \gls{fd} yields only a gain for $P_{\text{FD}} < -30$ dB.

A similar system performance for different power amplifier efficiencies is illustrated in \cref{fig:numerical_p_fd_alpha}. For lower $\alpha_i^{-1}$, \gls{fd} requires a lower $P_{\text{FD}}$ in order to yield a \gls{see} gain as compared to \gls{hd}.

To summarize: It can be seen that the \gls{see} can be significantly increased by maximizing for \gls{see} instead of secrecy capacity for any power amplifier efficiency and for constant power consumptions which are not too high. Furthermore \gls{fd} can only outperform \gls{hd} in terms of \gls{see} for a very high power amplifier efficiency and a low constant power consumption as well as a low \gls{fd} power consumption $P_{\text{FD}}$.

\subsection{Evaluation of the Impact of Self-Interference}
\label{sec:numeric_eval_si}
In this subsection the impact of the \gls{si} on the system's \gls{see} is analyzed. The \gls{si} is mainly characterized by the transmitter noise parameter $\kappa_i$, the receiver distortion paramter $\beta_i$ and the power of the \gls{si} channel. It is important to evaluate the performance of the system in dependency on these parameters because canceling the \gls{si} of \gls{fd} systems is still a challenge.

% Eval kappa_beta and si
\begin{figure}
\centering
\subfloat[SISO-SE]{\label{fig:numerical_siso_kappa_beta}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-60, 
				xmax=0,
				ymin=0,
				ymax=15,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={Transmitter Noise $\kappa_i$ / Receiver Distortion $\beta_j$ ($\kappa_i = \beta_j$) [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend style={at={(0.04,0.3)},anchor=west},				
				%legend pos=south west,
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/siso_kappa_beta.dat};
				\addplot table[x index=0,y index=2] {data/siso_kappa_beta.dat};
				\addplot table[x index=0,y index=3] {data/siso_kappa_beta.dat};
				\addplot table[x index=0,y index=4] {data/siso_kappa_beta.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[MIMO-ME]{\label{fig:numerical_std_kappa_beta}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-60, 
				xmax=0,
				ymin=0,
				ymax=90,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				xlabel={Transmitter Noise $\kappa_i$ / Receiver Distortion $\beta_j$ ($\kappa_i = \beta_j$) [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				%legend pos=south west,
				legend style={at={(0.04,0.3)},anchor=west},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/kappa_beta_data.dat};
				\addplot table[x index=0,y index=2] {data/kappa_beta_data.dat};
				\addplot table[x index=0,y index=3] {data/kappa_beta_data.dat};
				\addplot table[x index=0,y index=4] {data/kappa_beta_data.dat};
			\end{axis}
	\end{tikzpicture}}
	
\subfloat[SISO-SE]{\label{fig:numerical_siso_si}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-30, 
				xmax=30,
				ymin=0,
				ymax=15,
				%xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				xlabel={Variance of Bob's SI Channel [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				%legend pos=south east,
				legend style={at={(0.04,0.3)},anchor=west},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/siso_si.dat};
				\addplot table[x index=0,y index=2] {data/siso_si.dat};
				\addplot table[x index=0,y index=3] {data/siso_si.dat};
				\addplot table[x index=0,y index=4] {data/siso_si.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[MIMO-ME]{\label{fig:numerical_std_si}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=-20, 
				xmax=30,
				ymin=0,
				ymax=90,
				%xtick={0,-40,-30,-20,-10,10,20},			
				%ytick={0,50,100,150,200},
				xlabel={Variance of Bob's SI Channel [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend style={at={(0.04,0.3)},anchor=west},				
				%legend pos=south east,
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/si_data.dat};
				\addplot table[x index=0,y index=2] {data/si_data.dat};
				\addplot table[x index=0,y index=3] {data/si_data.dat};
				\addplot table[x index=0,y index=4] {data/si_data.dat};
		\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of transmitter noise $\kappa_i$, receiver distortion $\beta_i$ and variance of \gls{si} channel $\sigma_{SI}^2$ on the system's \gls{see} for the \gls{sisose} and \gls{mimome} case.}
\label{fig:eval_kappa_beta_si}
\end{figure}

Firstly, the effect of the transmitter noise and the receiver distortion on the \gls{see} for the \gls{sisose} and \gls{mimome} case is analyzed (see \ref{fig:numerical_siso_kappa_beta} and \ref{fig:numerical_std_kappa_beta}). The results for the \gls{sisose} case have to be interpreted cautiously because the transmitter noise and receiver distortion is only modeled at Bob in the \gls{sisose} system model of \ref{chap:siso-se}. However, in the \gls{mimome} system model these distortions are incorporated at each node. Therefore the \gls{see} approaches zero for all four settings if the distortion goes to infinity only in the \gls{mimome} case (see \ref{fig:numerical_std_kappa_beta}). However in both figures it can be seen that the gain of \gls{fd} over \gls{hd} for maximizing the \gls{see} vanishes for distortions above \si{-20}{dB}.

It is interesting to note that when maximizing the secrecy capacity for both cases, the \gls{see} increases for higher distortions before it drops to zero for very high distortions. A possible explanation for this could be that the distortion depends on the transmit power. For higher parameters $\kappa_i$ and $\beta_j$ it might be optimal to allocate less power, which in turn leads to an increased \gls{see}.

In \ref{fig:numerical_siso_si} and \ref{fig:numerical_std_si} the impact of the power of Bob's \gls{si} channel on the \gls{see} is depicted. The performance of the two \gls{hd} cases is constant since their system model does not depend on the \gls{si} channel $\mat{H}_{bb}$. However for the two \gls{fd} cases the gain over \gls{hd} diminishes for a variance of roughly \si{20}{dB} for the \gls{si} channel.

In summary it can be seen that \gls{fd} only outperforms \gls{hd} in terms of \gls{see} for low distortion parameters $\kappa_i$ and $\beta_j$ and for a low variance of the \gls{si} channel.

\subsection{Evaluation of the Impact of Eve's Position}
\label{sec:numeric_eval_pos}
In this subsection the geometry of the system models is altered. Now a system model is considered where Alice and Bob are located at a distance of \si{100}{m} and Eve is located somewhere on the line connecting Alice and Bob. In the following it is analyzed how the \gls{see} performance is affected by the position of Eve on this line-segment. 

% Eval pos
\begin{figure}
\centering
\subfloat[SISO-SE]{\label{fig:numerical_siso_pos}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=0, 
				xmax=100,
				ymin=0,
				ymax=0.7,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={Position of Eve [m] (Alice \si{0}{m}; Bob \si{100}{m})},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north west,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/siso_pos.dat};
				\addplot table[x index=0,y index=2] {data/siso_pos.dat};
				\addplot table[x index=0,y index=3] {data/siso_pos.dat};
				\addplot table[x index=0,y index=4] {data/siso_pos.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[MIMO-ME]{\label{fig:numerical_std_pos}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=0, 
				xmax=100,
				ymin=0,
				ymax=4,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				xlabel={Position of Eve [m] (Alice \si{0}{m}; Bob \si{100}{m})},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north west,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/pos_data.dat};
				\addplot table[x index=0,y index=2] {data/pos_data.dat};
				\addplot table[x index=0,y index=3] {data/pos_data.dat};
				\addplot table[x index=0,y index=4] {data/pos_data.dat};
			\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of the position of Eve $pos_{\text{Eve}}$ on the system's \gls{see} for the \gls{sisose} and \gls{mimome} case.}
\label{fig:eval_pos}
\end{figure}

The performance of the \gls{sisose} system model and the \gls{mimome} system model for a varying position of Eve is depicted in \ref{fig:numerical_std_pos} and \ref{fig:numerical_siso_pos}. Firstly, it is noted that both system models roughly have a similar relative performance. The \gls{see} is lowest for Eve being close to Alice for all compared cases and for both system models. Furthermore, the \gls{see} increases when Eve moves away from Alice and towards Bob. In general \gls{fd} and \gls{hd} have a very similar performance. For maximizing the \gls{see}, \gls{fd} is always at least as good as \gls{hd}. However once Eve is closer to Bob than to Alice, \gls{fd} yields a higher \gls{see} as compared to \gls{hd}. This gain increases when Eve moves closer to Bob and it becomes significant e.g. for a position of \si{95}{m}. Also for maximizing the secrecy capacity the \gls{see} of \gls{fd} is higher than in the \gls{hd} case if Eve is located close to Bob. This makes sense intuitively because jamming from Bob is much more efficient if Eve is located in close proximity to Bob.

In summary, \gls{fd} can yield a higher \gls{see} only if Eve is located close to Bob. This is also true if the secrecy capacity is maximized.

\subsection{Evaluation of the Impact of the Number of Antennas}
\label{sec:numeric_eval_Na_Nb_Nc}
In the following subsection the impact of the number of antennas on the system's \gls{see} is investigated. This is only possible for the \gls{mimome} system model. The results are depicted in \ref{fig:numerical_std_Na_Nb} and \ref{fig:numerical_std_Ne}.

% Eval Na Nb Ne
\begin{figure}
\centering
\subfloat[~]{\label{fig:numerical_std_Na_Nb}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=2, 
				xmax=8,
				ymin=0,
				ymax=250,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				xlabel={Number of Antennas of Alice and Bob $N_a = N_b$},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north west,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/Na_Nb_data.dat};
				\addplot table[x index=0,y index=2] {data/Na_Nb_data.dat};
				\addplot table[x index=0,y index=3] {data/Na_Nb_data.dat};
				\addplot table[x index=0,y index=4] {data/Na_Nb_data.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[~]{\label{fig:numerical_std_Ne}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$, HD - $\max SEE$, FD - $\max C_s$, HD - $\max C_s$},
				xmin=2, 
				xmax=8,
				ymin=0,
				ymax=120,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				xlabel={Number of Antennas of Eve},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend pos=north east,font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/Ne_data.dat};
				\addplot table[x index=0,y index=2] {data/Ne_data.dat};
				\addplot table[x index=0,y index=3] {data/Ne_data.dat};
				\addplot table[x index=0,y index=4] {data/Ne_data.dat};
			\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of the number of antennas of Alice, Bob and Eve on the system's \gls{see} for the \gls{mimome} case.}
\label{fig:eval_Na_Nb_Ne}
\end{figure}

In general the \gls{see} increases for an increasing number of antennas of Alice and Bob (see \ref{fig:numerical_std_Na_Nb}). Firstly, it can be seen that the gain of maximizing for \gls{see} is much higher for a larger number of antennas. Secondly, \gls{fd} exhibits a gain over \gls{hd} for low number of antennas for maximizing for \gls{see}. However, for a large number of antennas the gain vanishes, when maximizing \gls{see}. In contrast, when maximizing the secrecy capacity \gls{hd} is more efficient for a large number of antennas where as they both perform equally well for a low number of antennas.

The system performance for varying the number of antennas of Eve is somewhat reciprocal to that. The \gls{see} increases for a smaller number of antennas. For a larger number of antennas \gls{fd} yields a gain over \gls{hd} if maximized for \gls{see}. Furthermore, the gain is quite significant if Eve has 8 antennas (double as many as Alice and Bob).

In conclusion, the \gls{see} increases if Alice and Bob have more antennas than Eve. Furthermore, the gain of \gls{fd} is only significant if Eve has more antennas than Alice and Bob.

\section{Performance Evaluation for Bidirectional Communication}
\label{sec:numeric_eval_bidirectional}
In this section the \gls{see} performance of different bidirectional communication schemes, which are introduced in \ref{chap:sse_bidirectional_mimo-me}, are evaluated numerically. These are \gls{fd}, \gls{fdd} and \gls{tdd}.

% Eval bidirect communication
\begin{figure}
\centering
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandard,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={
					FD BC - $\max SEE$,
					FD WC - $\max SEE$,
					FDD. - $\max SEE$,
					TDD. - $\max SEE$,
					FD BC - $\max C_s$,
					FD WC - $\max C_s$,
					FDD. - $\max C_s$,
					TDD. - $\max C_s$
				},
				xmin=-50, 
				xmax=10,
				ymin=0,
				ymax=120,
				xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				xlabel={Max. Transmit Power per Modem [dB]},
				ylabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west},
				legend style={at={(1.1,0.5)},anchor=west},
				%legend pos=north west,
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/bidirectional_pmax_data.dat};
				\addplot table[x index=0,y index=2] {data/bidirectional_pmax_data.dat};
				\addplot table[x index=0,y index=3] {data/bidirectional_pmax_data.dat};
				\addplot table[x index=0,y index=4] {data/bidirectional_pmax_data.dat};
				\addplot table[x index=0,y index=5] {data/bidirectional_pmax_data.dat};
				\addplot table[x index=0,y index=6] {data/bidirectional_pmax_data.dat};
				\addplot table[x index=0,y index=7] {data/bidirectional_pmax_data.dat};
				\addplot table[x index=0,y index=8] {data/bidirectional_pmax_data.dat};	
			\end{axis}
	\end{tikzpicture}
\caption{Evaluation of the performance of \gls{fd}, \gls{fdd} and \gls{tdd} for bidirectional communication.}
\label{fig:numerical_eval_bidirect}
\end{figure}

\Cref{fig:numerical_eval_bidirect} depicts the performance of all four schemes for either \gls{see} or secrecy capacity maximization over an increasing transmit power constraint. The system parameters are chosen as in the previous section (see \ref{tab:ref_parameters}). For low transmit powers (low \gls{snr}) maximizing for secrecy capacity is again also optimal with respect to \gls{see}. Furthermore, \gls{fd} and \gls{fdd} perform similarly where as \gls{tdd} performs worst.

Comparing \gls{fdd} and \gls{tdd} it can be seen that \gls{fdd} yields a better performance for maximum transmit powers below \si{-20}{dB}. This could result from the lower noise power because of the reduced bandwidth of \gls{fdd}. However, for maximum transmit powers above \si{-20}{dB}, \gls{tdd} outperforms \gls{fdd}. A possible explanation could be the reduced transmit power of \gls{tdd} because only one transmitter is transmitting at each time.

For high \gls{snr} it can be observed that \gls{fd} significantly outperforms \gls{fdd} and \gls{tdd}. In case of the \glsfirst{bc} system model \gls{fd} can nearly double the \gls{see} as compared to \gls{fdd} and \gls{tdd}. The \glsfirst{wc} \gls{fd} system model performs worse but still significantly outperforms the classical schemes.

As a result it can be concluded that \gls{fd} can yield a significant \gls{see} gain in case of bidirectional communication as compared to classic approaches like \gls{fdd} and \gls{tdd}.

\section{Performance Evaluation for Statistical CSI}
\label{sec:numeric_eval_stat_csi}
In this section it is evaluated what performance the system can achieve in case of statistical \gls{csi} knowledge of the eavesdropper channels, as introduced in \ref{chap:sse_mimo-me_statistical_csi}. Therefore, the previous evaluation is extended to the statistical \gls{csi} system model of \ref{chap:sse_mimo-me_statistical_csi}. Firstly, the performance of different solutions in the reference point is compared. Then the impact of different system parameters on the system's performance is evaluated.

For the evaluation \si{10000} random channel realizations of each known channel distribution are generated. The performance of the covariance matrices, which where obtained by the different optimization algorithms, is then evaluated on this set of reference channels. It is assumed that the \si{10000} reference channels empirically catch the underlying statistical distribution.

\subsection{Evaluation for Reference Parameters}
\label{sec:numerical_stat_csi_eval_ref_parameters}
In this subsection the performance for the reference parameter set is evaluated. A simple approximation is to approximate the channel statistics with the mean of the distribution, which is denoted as $\mat{\bar{H}}$. In this case the deterministic algorithms of \ref{chap:mimo-me_see_maximization} (especially \ref{alg:sfp}) can be used to maximize either the \gls{see} or the secrecy capacity. This approach is considered as a benchmark for \ref{alg:stat_ssum}, which is denoted as \emph{Bench} for the remainder of this section.

% Eval SSUM for reference point
\begin{figure}
\centering
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - Bench,
					HD - $\max SEE$ - Bench,
					FD - $\max C_s$ - Bench,
					HD - $\max C_s$ - Bench,
					FD - $\max SEE$ - SSUM,
					HD - $\max SEE$ - SSUM,
					FD - $\max C_s$ - SSUM,
					HD - $\max C_s$ - SSUM},
				xmin=0, 
				xmax=140,
				ymin=0,
				ymax=1,
				%xtick={0,-50,-40,-30,-20,-10,10},			
				%ytick={0,50,100,150,200},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west},
				legend style={at={(1.1,0.5)},anchor=west},
				%legend pos=north west,
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_bench_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_bench_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_bench_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_bench_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_hd_m.dat};
			\end{axis}
	\end{tikzpicture}
\caption{Evaluation of the performance of SSUM.}
\label{fig:numerical_ssum_ref}
\end{figure}

A comparison of the performance in terms of \gls{see} is depicted as a \gls{cdf} in \ref{fig:numerical_ssum_ref}. Firstly, it can be observed that approximating the channel statistics by the mean value $\mat{\bar{H}}$ (\emph{Bench}) does not yield a good performance. Especially for the \gls{hd} case the result performs well only on very few channel realizations. Secondly, \gls{fd} yields a significant gain in \gls{see} and more importantly always has fewer channel realizations where the \gls{see} is zero.

To provide security in case of statistical \gls{csi} the number of channel realizations which result in a zero \gls{see} should be as small as possible. Therefore a \gls{fd} Bob can significantly enhance the security as well as the \gls{see} in case of statistical \gls{csi} because it results in significantly fewer zero \gls{see} channel realizations.

\subsection{Evaluation of the Impact of Thermal Noise Variance and Transmit Power}
\label{sec:numerical_stat_csi_eval_nvar_pmax}
In this subsection the impact of the thermal noise variance and the maximum transmit power per modem is evaluated.

% Eval statistical CSI nvar, pmax
\begin{figure}
\centering
\subfloat[Thermal noise variance]{\label{fig:numerical_stat_csi_nvar}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - $\sigma_i^2 = -50$ dB,
					HD - $\max SEE$ - $\sigma_i^2 = -50$ dB,
					%FD - $\max C_s$ - $\sigma_i^2 = -50$ dB,
					%HD - $\max C_s$ - $\sigma_i^2 = -50$ dB,
					FD - $\max SEE$ - $\sigma_i^2 = -40$ dB,
					HD - $\max SEE$ - $\sigma_i^2 = -40$ dB,
					%FD - $\max C_s$ - $\sigma_i^2 = -40$ dB,
					%HD - $\max C_s$ - $\sigma_i^2 = -40$ dB,
					FD - $\max SEE$ - $\sigma_i^2 = -30$ dB,
					HD - $\max SEE$ - $\sigma_i^2 = -30$ dB,
					%FD - $\max C_s$ - $\sigma_i^2 = -30$ dB,
					%HD - $\max C_s$ - $\sigma_i^2 = -30$ dB
					},
				xmin=0, 
				xmax=300,
				ymin=0,
				ymax=1,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_fd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_hd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_fd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_hd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_hd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_fd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_fd_h.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_nvar_hd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_fd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_nvar_hd_h.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[Max. transmit power]{\label{fig:numerical_stat_csi_pmax}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - $p_{max} = -10$ dB,
					HD - $\max SEE$ - $p_{max} = -10$ dB,
					%FD - $\max C_s$ - $p_{max} = -10$ dB,
					%HD - $\max C_s$ - $p_{max} = -10$ dB,
					FD - $\max SEE$ - $p_{max} = 0$ dB,
					HD - $\max SEE$ - $p_{max} = 0$ dB,
					%FD - $\max C_s$ - $p_{max} = 0$ dB,
					%HD - $\max C_s$ - $p_{max} = 0$ dB,
					FD - $\max SEE$ - $p_{max} = 10$ dB,
					HD - $\max SEE$ - $p_{max} = 10$ dB,
					%FD - $\max C_s$ - $p_{max} = 10$ dB,
					%HD - $\max C_s$ - $p_{max} = 10$ dB
					},
				xmin=0, 
				xmax=120,
				ymin=0,
				ymax=1,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_pmax_fd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_pmax_hd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_pmax_fd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_pmax_hd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_pmax_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_pmax_hd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_pmax_fd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_pmax_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_pmax_fd_h.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_pmax_hd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_pmax_fd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_pmax_hd_h.dat};
			\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of the thermal noise variance and the maximum transmit power per modem on the system's \gls{see} for the \gls{mimome} system model in case of statistical \gls{csi} of all eavesdropper channels.}
\label{fig:numerical_stat_csi_eval_nvar_pmax}
\end{figure}

The \gls{cdf} of \gls{fd} and \gls{hd} for maximizing the \gls{see} for three different thermal noise variance levels is depicted in \ref{fig:numerical_stat_csi_nvar}. It can be observed that with decreasing thermal noise variance the average \gls{see} increases and that the number of channel realizations with a zero \gls{see} decreases for both \gls{fd} and \gls{hd}. For this reason a low thermal noise vaiance, or a high \gls{snr}, is highly beneficial for secrecy as well as for \gls{see}. Furthermore it can be observed that the gain of \gls{fd} over \gls{hd} increases with decreasing thermal noise power. As a result in case of low \gls{snr} \gls{fd} yields no gain over \gls{hd}. These results match the results of the evaluation for full \gls{csi} as elaborated in \ref{sec:numerical_eval_nvar_and_pmax}.

Similarly the performance in terms of \gls{see} for three different maximum transmit power constraints is shown in \ref{fig:numerical_stat_csi_pmax}. It can be seen that the performance significantly increases with increasing transmit power constraint. This result matches the results from \cref{sec:numerical_eval_nvar_and_pmax}. A new result is that \gls{fd} has significantly less zero $SEE$ channel realizations for low transmit powers as compared to \gls{hd}. Therefore, \gls{fd} improves the secrecy not only in terms of average secrecy rate.

\subsection{Evaluation of the Impact of the Power Consumption}
\label{sec:numerical_stat_csi_eval_alpha_Pc}
In this subsection the impact of the power consumption, which mainly depends on the power amplifier efficiency $\alpha_i^{-1}$ and the constant power consumption per modem $P_{c,i}$, on the system's \gls{see} is evaluated.

% Eval statistical CSI alpha, Pc
\begin{figure}
\centering
\subfloat[Power amplifier efficiency]{\label{fig:numerical_stat_csi_alpha}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - $\alpha_i^{-1} = 0.3$ dB,
					HD - $\max SEE$ - $\alpha_i^{-1} = 0.3$ dB,
					%FD - $\max C_s$ - $\alpha_i^{-1} = 0.3$ dB,
					%HD - $\max C_s$ - $\alpha_i^{-1} = 0.3$ dB,
					FD - $\max SEE$ - $\alpha_i^{-1} = 0.6$ dB,
					HD - $\max SEE$ - $\alpha_i^{-1} = 0.6$ dB,
					%FD - $\max C_s$ - $\alpha_i^{-1} = 0.6$ dB,
					%HD - $\max C_s$ - $\alpha_i^{-1} = 0.6$ dB,
					FD - $\max SEE$ - $\alpha_i^{-1} = 0.9$ dB,
					HD - $\max SEE$ - $\alpha_i^{-1} = 0.9$ dB,
					%FD - $\max C_s$ - $\alpha_i^{-1} = 0.9$ dB,
					%HD - $\max C_s$ - $\alpha_i^{-1} = 0.9$ dB
					},
				xmin=0, 
				%xmax=300,
				ymin=0,
				ymax=1,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_alpha_fd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_alpha_hd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_alpha_fd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_alpha_hd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_alpha_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_alpha_hd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_alpha_fd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_alpha_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_alpha_fd_h.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_alpha_hd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_alpha_fd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_alpha_hd_h.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[Constant power consumption]{\label{fig:numerical_stat_csi_Pc}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - $P_c = -30$ dB,
					HD - $\max SEE$ - $P_c = -30$ dB,
					%FD - $\max C_s$ - $P_c = -30$ dB,
					%HD - $\max C_s$ - $P_c = -30$ dB,
					FD - $\max SEE$ - $P_c = -20$ dB,
					HD - $\max SEE$ - $P_c = -20$ dB,
					%FD - $\max C_s$ - $P_c = -20$ dB,
					%HD - $\max C_s$ - $P_c = -20$ dB,
					FD - $\max SEE$ - $P_c = -10$ dB,
					HD - $\max SEE$ - $P_c = -10$ dB,
					%FD - $\max C_s$ - $P_c = -10$ dB,
					%HD - $\max C_s$ - $P_c = -10$ dB
					},
				xmin=0, 
				%xmax=120,
				ymin=0,
				ymax=1,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_Pc_fd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_Pc_hd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_Pc_fd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_Pc_hd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_Pc_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_Pc_hd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_Pc_fd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_Pc_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_Pc_fd_h.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_Pc_hd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_Pc_fd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_Pc_hd_h.dat};
			\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of the power amplifier efficiency and the constant power consumption per modem on the system's \gls{see} for the \gls{mimome} system model in case of statistical \gls{csi} of all eavesdropper channels.}
\label{fig:numerical_stat_csi_eval_alpha_Pc}
\end{figure}

The \gls{cdf} for three different values of the power amplifier efficiency is illustrated in \ref{fig:numerical_stat_csi_alpha}. It can be observed that the \gls{see} as well as the gain of \gls{fd} over \gls{hd} grows with increasing power amplifier efficiency. This results matches the results of the \gls{sisose} and \gls{mimome} system model in case of full eavesdropper \gls{csi}.

The performance in terms of \gls{see} for three different constant power consumption values is depicted in \ref{fig:numerical_stat_csi_Pc}. The \gls{see} of both system models increases with decreasing constant power consumption. However, the gain of \gls{fd} over \gls{hd} does not change significantly. Furthermore, the number of channel realizations which result in a zero \gls{see} decreases for higher constant power consumptions. This is a new result and it means that a higher constant power consumption is beneficial for the system's security.

In conclusion the impact of the power amplifier efficiency as well as the constant power consumption on the system's \gls{see} in case of statistical \gls{csi} is very similar to the deterministic case.

\subsection{Evaluation of the Impact of Self-Interference}
\label{sec:numerical_stat_csi_eval_kappa_beta_si}
In this subsection the impact of the \gls{si}, which mainly depends on the transmitter noise, the receiver distortion and the strength of Bob's \gls{si} channel, on the system's \gls{see} is evaluated.

% Eval statistical CSI kappa_beta, si
\begin{figure}
\centering
\subfloat[Transmitter noise and receiver distortion]{\label{fig:numerical_stat_csi_kappa_beta}
	\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - $\kappa_i = \beta_j = -60$ dB,
					HD - $\max SEE$ - $\kappa_i = \beta_j = -60$ dB,
					%FD - $\max C_s$ - $\kappa_i = \beta_j = -60$ dB,
					%HD - $\max C_s$ - $\kappa_i = \beta_j = -60$ dB,
					FD - $\max SEE$ - $\kappa_i = \beta_j = -40$ dB,
					HD - $\max SEE$ - $\kappa_i = \beta_j = -40$ dB,
					%FD - $\max C_s$ - $\kappa_i = \beta_j = -40$ dB,
					%HD - $\max C_s$ - $\kappa_i = \beta_j = -40$ dB,
					FD - $\max SEE$ - $\kappa_i = \beta_j = -20$ dB,
					HD - $\max SEE$ - $\kappa_i = \beta_j = -20$ dB,
					%FD - $\max C_s$ - $\kappa_i = \beta_j = -20$ dB,
					%HD - $\max C_s$ - $\kappa_i = \beta_j = -20$ dB
					},
				xmin=0, 
				%xmax=300,
				ymin=0,
				ymax=1,
				%xtick={0,-50,-40,-30,-20,-10},			
				%ytick={0,50,100,150,200},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_kappa_beta_fd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_kappa_beta_hd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_kappa_beta_fd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_kappa_beta_hd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_kappa_beta_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_kappa_beta_hd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_kappa_beta_fd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_kappa_beta_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_kappa_beta_fd_h.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_kappa_beta_hd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_kappa_beta_fd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_kappa_beta_hd_h.dat};
			\end{axis}
	\end{tikzpicture}}
\hfill
\subfloat[Constant power consumption]{\label{fig:numerical_stat_csi_si}
		\begin{tikzpicture}[baseline,trim axis left,trim axis right]
			\begin{axis}[myStandardCDF,
				width=.39\textwidth,
				legend style={font=\tiny},
				legend style={cells={align=center}},
				legend entries ={FD - $\max SEE$ - $\sigma_{\text{SI}}^2 = -20$ dB,
					HD - $\max SEE$ - $\sigma_{\text{SI}}^2 = -20$ dB,
					%FD - $\max C_s$ - $\sigma_{\text{SI}}^2 = -20$ dB,
					%HD - $\max C_s$ - $\sigma_{\text{SI}}^2 = -20$ dB,
					FD - $\max SEE$ - $\sigma_{\text{SI}}^2 = 0$ dB,
					HD - $\max SEE$ - $\sigma_{\text{SI}}^2 = 0$ dB,
					%FD - $\max C_s$ - $\sigma_{\text{SI}}^2 = 0$ dB,
					%HD - $\max C_s$ - $\sigma_{\text{SI}}^2 = 0$ dB,
					FD - $\max SEE$ - $\sigma_{\text{SI}}^2 = 20$ dB,
					HD - $\max SEE$ - $\sigma_{\text{SI}}^2 = 20$ dB,
					%FD - $\max C_s$ - $\sigma_{\text{SI}}^2 = 20$ dB,
					%HD - $\max C_s$ - $\sigma_{\text{SI}}^2 = 20$ dB
					},
				xmin=0, 
				%xmax=120,
				ymin=0,
				ymax=1,
				%xtick={0,-60,-50,-40,-30,-20,-10},			
				%ytick={0,100,200,300,400},
				ylabel={Probability},
				xlabel={SEE $\left[ \text{secure bits / Hz / J} \right]$},
				xlabel near ticks,
				ylabel near ticks,
				/pgf/number format/1000 sep={},
				clip=false,
				legend image post style={xscale=1},
				%yticklabels={0,0.02,0.04,0.06,0.08,0.1},
				/tikz/plot label/.style={black, anchor=west}, 
				legend style={at={(0.5,-0.3)},anchor=north},
				font=\footnotesize]
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_si_fd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_si_hd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_si_fd_l.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_si_hd_l.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_si_fd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_si_hd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_si_fd_m.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_si_hd_m.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_si_fd_h.dat};
				\addplot table[x index=0,y index=1] {data/eCDF_maxsee_si_hd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_si_fd_h.dat};
				%\addplot table[x index=0,y index=1] {data/eCDF_maxcs_si_hd_h.dat};
			\end{axis}
	\end{tikzpicture}}
\caption{Evaluation of impact of the transmitter noise, receiver distortion and strength of Bob's \gls{si} channel on the system's \gls{see} for the \gls{mimome} system model in case of statistical \gls{csi} of all eavesdropper channels.}
\label{fig:numerical_stat_csi_eval_kappa_beta_si}
\end{figure}

The \gls{cdf} for three different values of $\kappa_i$ and $\beta_j$ is characterized in \ref{fig:numerical_stat_csi_kappa_beta}. As throughout this work it is assumed that both parameters are equal: $\kappa_i = \beta_j$. Two observations can be made from this evaluation: Firstly, the gain of \gls{fd} over \gls{hd} diminishes with increasing distortion, which is expected. Secondly, the number of channels which have a zero \gls{see} drops with decreasing distortions for both \gls{fd} and \gls{hd}. Therefore, from a security point of view, it is highly desirable to have low transmitter and receiver distortions. Additionally, it can be observed that the \gls{see} of \gls{hd} increases for large distortions. This is also observed for full \gls{csi}.

\Cref{fig:numerical_stat_csi_si} illustrates the \gls{cdf} for three different values of the strength of Bob's \gls{si} channel. As expected, it can be observed that the strength of the \gls{si} channel has no impact on the \gls{hd} system model. Furthermore, the performance of \gls{fd} drops with increasing \gls{si} strength. However, the performance of \gls{fd} should not drop below the \gls{hd} performance. Therefore, the gap between them for $\sigma_{\text{SI}}^2 = 20$dB should not exist and has to result from imperfections in the numerical evaluation.

==> mimoshapes.tex <==
% This file defines some new node shapes to use with tikz.
%
% The start code was taken and modified from the example in
% http://www.texample.net/tikz/examples/d-flip-flops-and-shift-register/
%
% The shapes defined here are:
% - mimoone
% - mimotwo
% - mimothree
% - mimoind
% - boxtwo
% - boxthree
%
% For the three first shapes you can epecify either the "right antennas" or
% "left antennas" option to indicate the antennas position. You can also
% change some distances by specifying the options "antenna offset",
% "antenna base height" and "antenna side" with some value.
%
% For the last two shapes you can change the appearance with the "circle
% fill color", "circle stroke color" and "circle radius" options.

\makeatletter

\newif\ifleftantennas

% The keys that the user can provide are all the keys below, except
% "leftantennas" (use the "right antennas" or "left antennas" keys instead)
\pgfkeys{
  /mimonode/leftantennas/.is if=leftantennas,
  /pgf/.cd,
  right antennas/.code={\pgfkeys{/mimonode/leftantennas=false}},
  left antennas/.code={\pgfkeys{/mimonode/leftantennas=true}},
  % minimum width/.initial=1.5cm,
  % minimum height/.initial=2cm,
  circle fill color/.initial=white,
  circle stroke color/.initial=black,
  circle radius/.initial=2mm,
  antenna offset/.initial=0.3 cm,
  antenna yshift/.initial=0. cm,
  antenna base height/.initial=0.2 cm,
  antenna side/.initial=0.4cm,
}


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx Macro definitions xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

% Macro with the common code to draw an antenna. Before calling this macro
% (inside the backgroundpath or similar) you need to set the values of
% \pgf@x and \pgf@y to point to the start of the antenna.
\def\mimoshapesdrawantenna{
  % Store the current positions in \pgf@xa and \pgf@ya
  \pgf@xa=\pgf@x 
  \pgf@ya=\pgf@y
  \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}

  \advance\pgf@xa by \antennaoffset
  \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
  \pgfpathclose
  \pgfmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}

  % \pgf@xb and \pgf@yb will have the coordinate with the starting point to
  % draw the triangle
  \pgf@xb=\pgf@xa \pgf@yb=\pgf@ya
  \advance\pgf@yb by \antennabaseheight cm
  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  
  % See section "Internals of How Point Commands Work" of the pgf manual to
  % understand pgf@process
  \pgf@process{
    \pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\pgfpointpolar{60}{\pgfkeysvalueof{/pgf/antenna side}}}
  }
  \pgf@xc=\pgf@x 
  \pgf@yc=\pgf@y
  \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
  
  
  \pgf@process{
    \pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}{\pgfpointpolar{180}{\pgfkeysvalueof{/pgf/antenna side}}}
  }
  \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
  
  \pgf@process{
    \pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\pgfpointpolar{240}{\pgfkeysvalueof{/pgf/antenna side}}}
  }
  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
}


% Macro with the common code to draw the ellipses. Before calling this
% macro (inside the backgroundpath or similar) you need to set the values
% of \pgf@x and \pgf@y to point to the center of the ellipses.
\def\drawellipses{
  % Store the current positions in \pgf@xa and \pgf@ya
  \pgf@xa=\pgf@x 
  \advance\pgf@xa by \antennaoffset
  \pgf@ya=\pgf@y
  
  % See section "Internals of How Point Commands Work" of the pgf manual to
  % understand pgf@process
  \pgf@process{\pgfpathcircle{\pgfpoint{\pgf@xa}{\pgf@ya+\antennabaseheight-1pt}}{1pt}}
  \pgf@process{\pgfpathcircle{\pgfpoint{\pgf@xa}{\pgf@ya+\antennabaseheight+2pt}}{1pt}}
  \pgf@process{\pgfpathcircle{\pgfpoint{\pgf@xa}{\pgf@ya+\antennabaseheight+5pt}}{1pt}}
}


% The code to determine the x coordinate for the anchors in the start of
% each antenna is common for all antennas. Therefore, it is better to
% define a macro with it and just call the macro when define the respective
% savedanchor.
\def\antennaStartXCoordinate{
  % x position
  \ifleftantennas
  % Anchor position when the "left antennas" key is used
  \pgf@x=-.5\wd\pgfnodeparttextbox
  % Advance by the inner xsep
  \pgfmathsetlength\pgf@xc{-\pgfkeysvalueof{/pgf/inner xsep}}
  \advance\pgf@x by \pgf@xc%
  %
  % If the resulting x coordinate is lower the value required for the
  % minimum width then the value for the minimum width will be used instead
  \setlength{\pgf@xa}{-\pgfshapeminwidth}
  \ifdim\pgf@x>.5\pgf@xa
  \pgf@x=.5\pgf@xa
  \fi
  \else
  % Anchor position when the "left antennas" key is not used or when
  % the "right antennas" key is used.
  \pgf@x=.5\wd\pgfnodeparttextbox % width of the box
  \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}
  \advance\pgf@x by \pgf@xc%
  \setlength{\pgf@xa}{\pgfshapeminwidth}
  \ifdim\pgf@x<.5\pgf@xa
  \pgf@x=.5\pgf@xa
  \fi
  \fi
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx mimoone shape declaration xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{mimoone}{

  % xxxxxxxxxx First we define some savedmacros xxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\antennaoffset{
    \ifleftantennas
      \def\antennaoffset{-\pgfkeysvalueof{/pgf/antenna offset}}
    \else
      \def\antennaoffset{\pgfkeysvalueof{/pgf/antenna offset}}
    \fi
  }

  \savedmacro\antennabaseheight{
    \def\antennabaseheight{\pgfkeysvalueof{/pgf/antenna base height}}
  }

  \savedmacro\antennayshift{
    \def\antennayshift{\pgfkeysvalueof{/pgf/antenna yshift}}
  }

  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define the savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedanchor\northeast{%
    \pgf@y=.5\ht\pgfnodeparttextbox % height of the box, ignoring the depth
    \pgf@x=.5\wd\pgfnodeparttextbox % width of the box
    %
    % -----> Take the inner sep into account
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}
    \advance\pgf@x by \pgf@xc%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}
    \advance\pgf@y by \pgf@yc%
    % -----
    % Test if the minimum width and height are respected. If not, set it as
    % the minimum width/height.
    \setlength{\pgf@xa}{\shapewidth}
    \ifdim\pgf@x<.5\pgf@xa
    \pgf@x=.5\pgf@xa
    \fi
    \setlength{\pgf@ya}{\shapeheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    %
    % -----> Take the outer sep into account
    % Now that we have the values of x and y we could stop here. However,
    % in order to take into account the "outer sep" we need to add it to
    % the anchor position(the idea is that the anchor will be outside the
    % actual node (by the outer sep ammount). The default value of the
    % outer sep is half the length of a line. Note that we are including
    % the outer sep value in the anchor definition, but it should not be
    % taken into account when drawing the background. Therefore, we need to
    % remove this when drawing the rectangle box.
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }

  \savedanchor\southwest{%
    \pgf@y=-.5\ht\pgfnodeparttextbox % height of the box, ignoring the depth
    \pgf@x=-.5\wd\pgfnodeparttextbox % width of the box
    %
    % -----> Take the inner sep into account
    \pgfmathsetlength\pgf@xc{-\pgfkeysvalueof{/pgf/inner xsep}}
    \advance\pgf@x by \pgf@xc%
    \pgfmathsetlength\pgf@yc{-\pgfkeysvalueof{/pgf/inner ysep}}
    \advance\pgf@y by \pgf@yc%
    % 
    % Test if the minimum width and height are respected. If not, set it as
    % the minimum width/height.
    \setlength{\pgf@xa}{-\shapewidth}
    \ifdim\pgf@x>.5\pgf@xa
    \pgf@x=.5\pgf@xa
    \fi
    \setlength{\pgf@ya}{-\shapeheight}
    \ifdim\pgf@y>.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    %
    % -----> Take the outer sep into account (see comment in the northeast savedanchor)
    \pgfmathsetlength\pgf@xa{-\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength\pgf@ya{-\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }

  % This anchor position will depend if the "left antennas" option was
  % passed or not.
  \savedanchor{\anchorA}{
    % -----> y position for the first antenna
    \pgf@y=.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from rectangle xxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Inherit normal anchors from rectangle xxxxxxxxxxxxxxxxxxxxxx
  % We can inherit the "usual" from rectangle. They depend on the
  % "\southwest" and "\northeast" savedanchors but this will use our
  % version instead of the rectangle's version.
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{A}{
    \pgf@process{\anchorA}
  }

  \anchor{text}
  {
    \pgf@process{\pgfpointorigin}
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }
  
  % -----> Define some more useful anchors
  \anchor{first antenna base start}{
    \pgf@process{\anchorA}
  }

  \anchor{first antenna base end}{
    \pgf@process{\anchorA}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.2cm%
  }

  \anchor{first antenna}{
    %\csname pgf@anchor@mimoone@first antenna base start\endcsname
    \pgf@process{\anchorA}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.4cm%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    % \pgfpathrectanglecorners{\southwest}{\northeast}
    \pgfpathrectanglecorners
    { % First corner of the rectangle
      \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
    }
    { % Second corner of the rectangle
      \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    }

    %%%%%%% Draw the first antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorA}
    % The mimoshapesdrawantenna command only needs that the pgf@x and pgf@y
    % variables are correctly set. This is done by calling the anchor A
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of mimoone shape declaration xxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx mimotwo shape declaration xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{mimotwo}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimoone
  \inheritsavedanchors[from=mimoone]  
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define some savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we redefine the "anchorA", since it will be different from the
  % one we inherited from the mimoone shape.
  %
  % This anchor position will depend if the "left antennas" option was
  % passed or not.
  \savedanchor{\anchorA}{
    % -----> y position for the first antenna
    \pgf@y=.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.4\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }

  % Now we define a new anchorB for the second antenna.
  % This anchor position will depend if the "left antennas" option was
  % passed or not
  \savedanchor{\anchorB}{
    % -----> y position for the first antenna
    \pgf@y=-.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{-\pgfshapeminheight}
    \ifdim\pgf@y>.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.6\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimoone xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=mimoone]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Inherit normal anchors from mimoone xxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=mimoone]{center}
  \inheritanchor[from=mimoone]{north}
  \inheritanchor[from=mimoone]{east}
  \inheritanchor[from=mimoone]{south}
  \inheritanchor[from=mimoone]{west}
  \inheritanchor[from=mimoone]{north east}
  \inheritanchor[from=mimoone]{north west}
  \inheritanchor[from=mimoone]{south west}
  \inheritanchor[from=mimoone]{south east}
  \inheritanchor[from=mimoone]{text}
  \inheritanchor[from=mimoone]{A}
  \inheritanchor[from=mimoone]{first antenna base start}
  \inheritanchor[from=mimoone]{first antenna base end}
  \inheritanchor[from=mimoone]{first antenna}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{B}{
    \pgf@process{\anchorB}
  }

  \anchor{second antenna base start}{
    \pgf@process{\anchorB}
  }

  \anchor{second antenna base end}{
    \pgf@process{\anchorB}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.2cm%
  }

  \anchor{second antenna}{
    %\csname pgf@anchor@mimotwo@second antenna base start\endcsname
    \pgf@process{\anchorB}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.4cm%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    % \pgfpathrectanglecorners{\southwest}{\northeast}
    \pgfpathrectanglecorners
    { % First corner of the rectangle
      \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
    }
    { % Second corner of the rectangle
      \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    }

    %%%%%%% Draw the first antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorA}
    % The mimoshapesdrawantenna command only needs that the pgf@x and pgf@y
    % variables are correctly set. This is done by calling the anchor A
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    %%%%% Draw the second antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorB}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of mimotwo shape declaration xxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxx Mimo Shape with three antennas xxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{mimothree}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimotwo
  \inheritsavedanchors[from=mimotwo]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define some savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we redefine "anchorA" and "anchorB", since they will be different
  % from the one we inherited from the mimotwo shape.
  %
  % This anchor position will depend if the "left antennas" option was
  % passed or not.
  \savedanchor{\anchorA}{
    \pgf@y=.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.5\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }

  \savedanchor{\anchorC}{
    % y position for the first antenna
    \pgf@y=-.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{-\pgfshapeminheight}
    \ifdim\pgf@y>.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.9\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }

  % B is in the middle of A and C
  \savedanchor{\anchorB}{
    % y position
    % First we get y position of anchor A
    \pgf@y=.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@ya=0.5\pgf@y
    % Then we get y position of anchor C
    \pgf@y=-.5\ht\pgfnodeparttextbox
    \setlength{\pgf@yc}{-\pgfshapeminheight}
    \ifdim\pgf@y>.5\pgf@yc
    \pgf@y=.5\pgf@yc
    \fi
    \pgf@yc=0.9\pgf@y
    % y position of anchor B is in the middle of anchor A and C
    \pgf@y=0.5\pgf@yc
    \advance\pgf@y by 0.5\pgf@ya
    %
    \advance\pgf@y by \antennayshift
    % 
    % x position
    \antennaStartXCoordinate
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimotwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=mimotwo]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from mimotwo xxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=mimotwo]{center}
  \inheritanchor[from=mimotwo]{north}
  \inheritanchor[from=mimotwo]{east}
  \inheritanchor[from=mimotwo]{south}
  \inheritanchor[from=mimotwo]{west}
  \inheritanchor[from=mimotwo]{north east}
  \inheritanchor[from=mimotwo]{north west}
  \inheritanchor[from=mimotwo]{south west}
  \inheritanchor[from=mimotwo]{south east}
  \inheritanchor[from=mimotwo]{text}
  \inheritanchor[from=mimotwo]{A}
  \inheritanchor[from=mimotwo]{B}
  \inheritanchor[from=mimotwo]{first antenna base start}
  \inheritanchor[from=mimotwo]{second antenna base start}
  \inheritanchor[from=mimotwo]{first antenna base end}
  \inheritanchor[from=mimotwo]{second antenna base end}
  \inheritanchor[from=mimotwo]{first antenna}
  \inheritanchor[from=mimotwo]{second antenna}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{C}{\anchorC}

  \anchor{third antenna base start}{
    \pgf@process{\anchorC}
  }
  \anchor{third antenna base end}{
    \pgf@process{\anchorC}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.2cm%
  }
  \anchor{third antenna}{
    %\csname pgf@anchor@mimothree@third antenna base start\endcsname
    \pgf@process{\anchorC}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.4cm%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners
    { % First corner of the rectangle
      \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
    }
    { % Second corner of the rectangle
      \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    }

    %%%%%%% Draw the first antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorA}
    % The mimoshapesdrawantenna command only needs that the pgf@x and pgf@y
    % variables are correctly set. This is done by calling the anchor A
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    %%%%% Draw the second antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorB}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    %%%%% Draw the third %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorC}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  }
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of mimothree shape declaration xxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxx Mimo Shape with "many" antennas xxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{mimoind}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimothree
  \inheritsavedanchors[from=mimothree]

  % There is no need to define more savedanchors, since mimothree already
  % provide us with all we need.
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimotwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=mimothree]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from mimothree xxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=mimothree]{center}
  \inheritanchor[from=mimothree]{north}
  \inheritanchor[from=mimothree]{east}
  \inheritanchor[from=mimothree]{south}
  \inheritanchor[from=mimothree]{west}
  \inheritanchor[from=mimothree]{north east}
  \inheritanchor[from=mimothree]{north west}
  \inheritanchor[from=mimothree]{south west}
  \inheritanchor[from=mimothree]{south east}
  \inheritanchor[from=mimothree]{text}
  \inheritanchor[from=mimothree]{A}
  \inheritanchor[from=mimothree]{B}
  \inheritanchor[from=mimothree]{C}
  \inheritanchor[from=mimothree]{first antenna base start}
  \inheritanchor[from=mimothree]{second antenna base start}
  \inheritanchor[from=mimothree]{third antenna base start}
  \inheritanchor[from=mimothree]{first antenna base end}
  \inheritanchor[from=mimothree]{second antenna base end}
  \inheritanchor[from=mimothree]{third antenna base end}
  \inheritanchor[from=mimothree]{first antenna}
  \inheritanchor[from=mimothree]{second antenna}
  \inheritanchor[from=mimothree]{third antenna}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners
    { % First corner of the rectangle
      \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
    }
    { % Second corner of the rectangle
      \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    }

    %%%%%%% Draw the first antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Você pode usar \pgf@anchor@SHAPE_NAME@ANCHOR_NAME para mudar o \pgf@x
    % e o \pgf@y para as coordenadas de uma âncora. Só que se você resolver
    % mudar o nome do shape depois vai ter que mudar todas as linhas que
    % contem o SHAPE_NAME. Melhor usar o csname como na linha abaixo.
    \pgf@process{\anchorA}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    %%%%% Draw the second antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\csname pgf@anchor@\pgf@sm@shape@name @second antenna base end\endcsname
    \pgf@process{\anchorB}
    %\mimoshapesdrawantenna
    \drawellipses
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    %%%%% Draw the third antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorC}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  }
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of mimoind shape declaration xxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxx Boxtwo Node xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{boxtwo}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimoone
  \inheritsavedanchors[from=mimoone]

  % There is no need to define more savedanchors, since mimoone already
  % provide us with all we need.
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimotwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=mimoone]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from mimoone xxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=mimotwo]{center}
  \inheritanchor[from=mimotwo]{north}
  \inheritanchor[from=mimotwo]{east}
  \inheritanchor[from=mimotwo]{south}
  \inheritanchor[from=mimotwo]{west}
  \inheritanchor[from=mimotwo]{north east}
  \inheritanchor[from=mimotwo]{north west}
  \inheritanchor[from=mimotwo]{south west}
  \inheritanchor[from=mimotwo]{south east}
  \inheritanchor[from=mimotwo]{text}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  % See section "Internals of How Point Commands Work" of the pgf manual to
  % understand pgf@process
  \anchor{A}{
    \pgf@process{\northeast}%
    \pgf@x=0pt
    \pgf@y=0.5\pgf@y%
  }

  \anchor{B}{
    \pgf@process{\northeast}%
    \pgf@x=0pt
    \pgf@y=-0.5\pgf@y%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    {
      \pgfpathrectanglecorners
      { % First corner of the rectangle
        \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
      }
      { % Second corner of the rectangle
        \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
      }
      \pgfusepath{stroke,fill}
    }
    
    % The two circles
    {
      \csname pgf@anchor@\pgf@sm@shape@name @A\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \csname pgf@anchor@\pgf@sm@shape@name @B\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/circle fill color}}
      \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/circle stroke color}}
      \pgfusepath{stroke,fill}
    }
  }
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of boxtwo shape declaration xxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxx Boxthree Node xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{boxthree}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimoone
  \inheritsavedanchors[from=boxtwo]

  % There is no need to define more savedanchors, since mimoone already
  % provide us with all we need.
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimotwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=boxtwo]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from boxtwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=boxtwo]{center}
  \inheritanchor[from=boxtwo]{north}
  \inheritanchor[from=boxtwo]{east}
  \inheritanchor[from=boxtwo]{south}
  \inheritanchor[from=boxtwo]{west}
  \inheritanchor[from=boxtwo]{north east}
  \inheritanchor[from=boxtwo]{north west}
  \inheritanchor[from=boxtwo]{south west}
  \inheritanchor[from=boxtwo]{south east}
  \inheritanchor[from=boxtwo]{text}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  % See section "Internals of How Point Commands Work" of the pgf manual to
  % understand pgf@process
  \anchor{A}{
    \northeast
    \pgf@x=0pt
    \pgf@y=0.6\pgf@y%
  }

  \anchor{B}{
    \pgf@x=0pt
    \pgf@y=0pt
  }

  \anchor{C}{
    \northeast
    \pgf@x=0pt
    \pgf@y=-0.6\pgf@y%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    {
      \pgfpathrectanglecorners
      { % First corner of the rectangle
        \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
      }
      { % Second corner of the rectangle
        \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
      }
      \pgfusepath{stroke,fill}
    }
    
    % The three circles
    {
      \csname pgf@anchor@\pgf@sm@shape@name @A\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \csname pgf@anchor@\pgf@sm@shape@name @B\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \csname pgf@anchor@\pgf@sm@shape@name @C\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/circle fill color}}
      \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/circle stroke color}}
      \pgfusepath{stroke,fill}
      }
  }
}

\makeatother


% The Comment below is only important for Emacs

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "testmimoshapes.tex"
%%% TeX-PDF-mode: t
%%% End: 

